Outlier-Robust Clustering of Non-Spherical Mixtures

We give the first outlier-robust efficient algorithm for clustering a mixture of $k$ statistically separated d-dimensional Gaussians (k-GMMs). Concretely, our algorithm takes input an $\epsilon$-corrupted sample from a $k$-GMM and whp in $d^{\text{poly}(k/\eta)}$ time, outputs an approximate clustering that misclassifies at most $k^{O(k)}(\epsilon+\eta)$ fraction of the points whenever every pair of mixture components are separated by $1-\exp(-\text{poly}(k/\eta)^k)$ in total variation (TV) distance. Such a result was not previously known even for $k=2$. TV separation is the statistically weakest possible notion of separation and captures important special cases such as mixed linear regression and subspace clustering. Our main conceptual contribution is to distill simple analytic properties - (certifiable) hypercontractivity and bounded variance of degree 2 polynomials and anti-concentration of linear projections - that are necessary and sufficient for mixture models to be (efficiently) clusterable. As a consequence, our results extend to clustering mixtures of arbitrary affine transforms of the uniform distribution on the $d$-dimensional unit sphere. Even the information-theoretic clusterability of separated distributions satisfying these two analytic assumptions was not known prior to our work and is likely to be of independent interest. Our algorithms build on the recent sequence of works relying on certifiable anti-concentration first introduced in the works of Karmarkar, Klivans, and Kothari and Raghavendra, and Yau in 2019. Our techniques expand the sum-of-squares toolkit to show robust certifiability of TV-separated Gaussian clusters in data. This involves giving a low-degree sum-of-squares proof of statements that relate parameter (i.e. mean and covariances) distance to total variation distance by relying only on hypercontractivity and anti-concentration.

==> content/old/LDC.tex <==
%!TEX root = ../main.tex

\section{List-Decodable Covariance Estimation}
\Pnote{some  global notation guidelines since this is  going to  get hairy.
\begin{enumerate}
\item $\tzeta$ will be our pseudo-distribution throughout.
\item $\mu,\Sigma$ whenever it is used should be used to denote means/covariances.
\item $X$ is the original uncorrupted $n$-sample. $Y$ is the sample we see (not $\cS$) and the only thing we know is that $|Y \cap X|\geq \alpha n$. And $X'$ is the sample our algorithm tries to discover - $X'$ are variables in our program, cannot treat them as constants.
\item $w$ indicates the intersection of $Y$ and $X'$. It doesn't denote the intersection of $X'$ and $X$ which is what need in the analysis. I am using $w'$ for this for now.
\item There are two constants floating around right now - the constant $C$ in certifiable hypercontractivity and the constant - also called $C$ - in certifiable anti-concentration. Need to fix this.
\item A: Since $\epsilon$ is being used as a fraction of corruption by adversary, I will use $\gamma$ to denote the closeness between emperical mean and covariance of an inlier cluster and the true parameters of the corresponding distribution.
\end{enumerate}
}

In this section, we give an efficient algorithm to list-decode mean and covariance of all distributions that arise from a \emph{nice} ``base model''.

\begin{definition}[Nice Distributions]
\label{def:nice_distribution}
An isotropic (i.e. mean $0$ and $I$-covariance) distribution $\cD$ on $\R^d$ is \emph{nice} if it satisfies the following three properties:
\begin{enumerate}
\item \emph{Subgaussianity}: $\cD$ is $1$-subgaussian.
\item \emph{Certifiable Anti-Concentration}: The distribution of $x-x'$ for $x,x' \sim \cD$, chosen independently, is $s$-certifiably $(\delta,C\delta)$ anti-concentrated with the witnessing polynomial $p_{\cD}$ of degree $r$, for some $\delta \leq 1/k$ and,
\item  \emph{Certifiable Hypercontractivity}: The distribution of $x-x'$ for $x,x' \sim \cD$, chosen independently, has $h$-certifiably $C$-hypercontractive degree $2$ polynomials.
\end{enumerate}
Observe that if $\cD$ has $h$-certifiably $C$-hypercontractive degree 2 polynomials then it is also $h$-certifiably $C$-subgaussian.
\end{definition}

The goal of this section is to prove the following theorem:
\begin{theorem}\label{thm:main-theorem-LDC}
Let $\Sigma_*$ be a PSD matrix such that $0 < \lambda_l I \preceq \Sigma_* \preceq \lambda_u I$ and let $\kappa = \lambda_u/\lambda_l$. Then, there exists an algorithm that takes a sample of size $n \geq n_0 = $ drawn according to $\cov_{\cD,\alpha}(\mu_*,\Sigma_*)$ for any nice distribution $\cD$, runs in time $n^{}$ and outputs a list $\cL$ $\{(\mu_i,\Sigma_i)\}_{i \leq r}$ of size $r = $ such that with probability at least $0.99$ over the draw of the sample, there exists a $(\mu_0,\Sigma_0)$ in $\cL$ satisfying:
\begin{enumerate}
\item \textbf{Mean Closeness :} $\Norm{\Sigma_*^{-1/2} (\mu_{0} - \mu_*)}_2^2 \leq \Paren{\frac{1}{\alpha}}^2 $,
\item \textbf{Spectral Closeness:} $\Omega\Paren{\frac{\alpha}{s}}^2 \alpha^{2/s} I \preceq  \Sigma_*^{-1/2} \hat{\Sigma} \Sigma_*^{-1/2} \preceq \Paren{\frac{\alpha}{s}}^2 \alpha^{4/s} (1-\frac{C}{\alpha^3})^{1/s} I$
\item \textbf{Relative Frobenius Closeness: } $\Norm{I - \Sigma_*^{-1/2} \Sigma_{0} \Sigma_*^{-1/2}}^2_F \leq \frac{1}{\alpha}$.
\end{enumerate}
\Anote{insert the right bounds here. This will follow from pruning. }
\end{theorem}
\FIXME{add spectral closeness statement in Theorem above.}

% In this section, we describe and analyze our algorithm for list-decodable covariance estimation. Throughout this section, we fix a known ``base model'' -  isotropic distribution $\cD$ that is certifiably anti-concentrated with witnessing polynomial $p$ and has certifiable hypercontractive degree 2 polynomial moments. Recall that our input data is obtained by an $(1-\alpha)$ corruption of an i.i.d. sample from $\cD(0,\Sigma_*)$ for some unknown $\Sigma_*$.

Our algorithm is based on rounding an SoS relaxation of a natural polynomial formulation of the problem. At a high level, the polynomial formulation attempts to find \emph{nice} distributions that are close (intersects in $\geq \alpha n$ points) to the input corrupted sample and output their means and covariances. We describe this polynomial constraint system next.



% Our algorithm is based on solving a sum-of-squares relaxation of a natural polynomial program. At a high level, the program simply tries to find a sample of $n$ points that  are 1) certifiably anti-concentrated 2) have certifiably hypercontractive degree $2$ polynomials 3) intersect the input sample in $\alpha n$ points. We start by describing how we can capture these conditions by means of polynomial constraints.

\subsection{Constraint System}
Our constraint system $\cA$ uses polynomial constraints to describe a subset $X'$ of the input points of size $\alpha n$ with mean $\mu$ and covariance $\Sigma$ and satisfy the requirements of being a nice distribution. We describe the specific formulation next. For ease of exposition, we break $\cA$ into $\cA_1 \cup \cdots \cup \cA_5$ each of which captures a natural category of constraints.

For our argument, we will need access to the square root and inverse square root of $\Sigma$.
So we introduce the constraint system $\cA_1$ with extra matrix valued indeterminates $\Theta$ and $\Pi$ that satisfy polynomial equality constraints corresponding to $\Pi$ being the square root of $\Sigma$ and $\Theta$ the inverse of $\Pi$.
\Pnote{Make notation consistent throughout this section: Input Samples = $Y = \{y_1, y_2,...,y_n\}$. The set indicated by $w$ = $X' \subseteq Y$. Inliers = $\cI$. } \Anote{done.}

\begin{equation}
\text{Covariance Constraints: $\cA_1$} = %  \cA_{w,\Pi}\colon
  \left \{
    \begin{aligned}
      &
      &\Theta, \Pi
      &\succeq 0\\
      &
      &\Theta \Pi = \Pi \Theta
      &= I\\
      &
      &\Pi^2
      &=\Sigma\\
      &
      &\Theta^2\Sigma  = \Sigma \Theta^2
      &=\Theta\Sigma\Theta =I\\
    \end{aligned}
  \right \}
\end{equation}

Next, we formulate intersection constraints that identify the subset $X'$ of size $\alpha n$.
\begin{equation}
\text{Intersection Constraints: $\cA_2$} = %  \cA_{w,\Pi}\colon
  \left \{
    \begin{aligned}
      &\forall i\in [n].
      & w_i^2
      & = w_i\\
      &&
      \textstyle\sum_{i\in[n]} w_i
      &= \alpha n\\
    \end{aligned}
  \right \}
\end{equation}

Next, we enforce that $X'$ must have $\mu$ and covariance $\Sigma$. We also enforce condition number constraints on $\Sigma$ and their implications on $\Pi$ and $\Theta$.

\begin{equation}
\text{Parameter Constraints: $\cA_3$} = %  \cA_{w,\Pi}\colon
  \left \{
    \begin{aligned}
      &
      &\frac{1}{\alpha n}\sum_{i = 1}^n w_i y_i
      &= \mu\\
      &
      &\frac{1}{\alpha n}\sum_{i = 1}^n w_i \Paren{y_i-\mu} \Paren{y_i-\mu}^{\top}
      &= \Sigma\\
      &
      &\lambda_u I - \Sigma
      &\succeq 0\\
      &
      &\Sigma-\lambda_l I
      &\succeq 0\\
      &
      &\lambda^{1/2}_u I - \Pi
      &\succeq 0\\
      &
      &\Pi-\lambda^{1/2}_l I
      &\succeq 0\\
      &
      &\lambda^{-1/2}_l I - \Theta
      &\succeq 0\\
      &
      &\Theta-\lambda_u^{-1/2} I
      &\succeq 0\\
    \end{aligned}
  \right \}
\end{equation}

% Next, we formulate intersection constraints that subset of points indicated  by $w$ intersect the input sample $Y$ in $\alpha n$ points. and that $X'$ has mean $\mu$ and covariance $\Sigma$.
% \begin{equation}
% \text{Intersection Constraints: $\cA_3$} = %  \cA_{w,\Pi}\colon
%   \left \{
%     \begin{aligned}
%       &\forall i\in [n].
%       & w_i^2
%       & = w_i\\
%       &&
%       \textstyle\sum_{i\in[n]} w_i
%       &= \alpha n\\
%       &\forall i \in [n]
%       & w_i (y_i-y_i')
%       &=0
%     \end{aligned}
%   \right \}
% \end{equation}


Next, we add constraints that enforce that the uniform distribution on $X'$ forms a \textit{nice} distribution when put in isotropic position. Observe that in ``real life'', $\Theta (y_i-\mu)$ will give us a distribution with mean $0$ and covariance $I$ since $\Theta$ is supposed to stand for the inverse square root of $\Sigma$. For our analysis, though, it turns out to be easier to "isotropize" instead by taking the distribution on ${n \choose 2}$ points produced by $\Theta \frac{(y_i -y_j)}{\sqrt{2}}$ for $i \neq j$. Observe that uniform distribution on $\Theta \frac{(y_i -y_j)}{\sqrt{2}}$, in ``real life'' has mean $0$ and covariance $I$. Thus, the first set of constraints $\cA_4$ enforce certifiable anti-concentration of the set of points $\left\{\Theta \frac{(y_i -y_j)}{\sqrt{2}}\right\}_{i,j \leq n}$. Finally, $\cA_5$ enforces the certifiable hyper-contractivity of $\left\{\Theta \frac{(y_i -y_j)}{\sqrt{2}}\right\}_{i \leq n}$.






\text{Certifiable Anti-Concentration: }
\begin{equation}
 \cA_4 =% \cA_{w,\Pi}\colon
  \left \{
    \begin{aligned}
      % &\forall i \neq j \in [n].
      % & \norm{v}_2^{2t-2} \Iprod{\Theta \frac{(y_i -y_j)}{\sqrt{2}},v}^2 +\delta^2 p_{\cD}^2 \Paren{\Iprod{\Theta \frac{(y_i -y_j)}{\sqrt{2}},v}}
      % &\geq \delta^2 \norm{v}_2^{2t}\\
      &
      &\frac{1}{\alpha^2 n^2}\sum_{i \neq j \in [n]} w_i w_j p_{\cD}^2\Paren{\Iprod{\Theta \frac{(y_i -y_j)}{\sqrt{2}},v}}
      &\leq C\delta \norm{v}_2^{2t}\\
     \end{aligned}
    \right\}
 \end{equation}

\text{Certifiable Hyper-contractivity :}
\begin{equation}
 \cA_5 = %\cA_{w,\Pi}\colon
  \left \{
    \begin{aligned}
     &
     &\frac{1}{\alpha^2 n^2} \sum_{i \neq j \in [n]} w_i w_j \Paren{ \Iprod{\Paren{\Theta \frac{(y_i -y_j)}{\sqrt{2}}}\Paren{\Theta \frac{(y_i -y_j)}{\sqrt{2}}}^{\top},Q } - \tr(Q)}^2
     &\leq 3\Norm{Q}_F^2\mper
    \end{aligned}
  \right \}
\end{equation}

\Anote{I think we can leave the $w_i, w_j$ notation here and introduce the $\expecf{w}{}$ notation in the analysis. Happy to change if you feel strongly about this.}


\subsection{Algorithm}
We are now ready to describe our algorithm for List-Decodable Covariance Estimation.

Conceptually, our algorithm can be broken down into three stages. The first stage computes a pseudo-distribution consistent with the system of constraints $\cA$. The second rounds this pseudo-distribution into a list of parameters one of which is guaranteed to be close to the true inlier parameters $\mu_*,\Sigma_*$. This list is $d^{O(s\log \kappa) \poly(1/\alpha))}$ in size. Finally, the third stage ``prunes'' this list down to the optimal size $O(1/\alpha)$.

\begin{mdframed}[nobreak=true]
  \begin{algorithm} List-Decodable Covariance Estimation
    \label[algorithm]{alg:covariance-estimation}\mbox{}
    \begin{description}
    \item[Given:]
    Sample $Y = \{y_1, y_2, \ldots y_n \}$ of size $n$ such that an $\alpha$-fraction of points are $s$-certifiably anti-concentrated and $h$-certifiably hypercontractive.
      \item[Operation:] \textrm{ }\\
      \vspace{-0.3in}
      \begin{enumerate}
        %\item Let $t =  \Delta \cdot \left(\frac{\log^5(1/\alpha)\log(r\kappa)}{\alpha^2}\right)$ for a large enough constant $\Delta >0$.
        \item Let $\Delta = O((h+s)(1+\log(\kappa)))$. Compute a $\Delta$-degree pseudo-distribution $\tzeta$ satisfying $\cA$ that minimizes $\Norm{\sum_{i = 1}^n\pE[w_i]}^2_2$.
        \item Applying the Large-List Rounding procedure (Algorithm \ref{alg:rounding_large_list}) to output a $O(1/\alpha^\Delta)$ sized list $\cL'$. %Apply Large List Rouding Algorithm .
        \item Run pruning (Algorithm \ref{alg:pruning-general}) on $\cL'$ and output the resulting list $\cL$.
      \end{enumerate}
    \item[Output:]
      A list $\cL$ of size $O(1/\alpha)$ containing $(\mu,\Sigma)$ satisfying $\Norm{\Sigma_*^{-1/2}(\mu-\mu_*)}_2^2 < $, $\Sigma_*^{-1/2} \hat{\Sigma} \Sigma_*^{-1/2} \preceq$, and $\Norm{I - \Sigma_*^{-1/2} \Sigma \Sigma_*^{-1/2}}_F^2 \leq $ \Anote{Fill these params in.}
    \end{description}
  \end{algorithm}%\label{alg:main}
\end{mdframed}


Intuitively, our large list rounding algorithm works by ``conditioning'' on a small, randomly chosen set of samples to be included in the set $X'$ computed by the algorithm and outputs the pseudo-expectations of the parameters $\mu$ and $\Sigma$ after conditioning. Our analysis shows that with a non-trivially large probability over the choice of the random set used in the conditioning, the set of parameters we obtain in the rounding are close to $\mu_*,\Sigma_*$.


\begin{mdframed}[nobreak=true]
  \begin{algorithm} Large List Rounding
    \label[algorithm]{alg:rounding_large_list}\mbox{}
    \begin{description}
    \item[Given:]
    A pseudo-distribution $\tzeta$ of degree $\Delta = O((h+s)(1+\log(\kappa)))$ satisfying $\cA$ and minimizing $\Norm{\sum_{i\leq n} \pE w_i}_2^2$ %such that $t =  \Delta \cdot \left(\frac{\log^5(1/\alpha)\log(r\kappa/\eta)}{\alpha^2}\right)$, for a large constant $\Delta$, accuracy parameter $\eta >0$.
      \item[Operation:] Repeat $\ell= O(1/\alpha^\Delta)$ times:
      \begin{enumerate}
      \item Pick multiset $S \subseteq [n]$ of size $\Delta$ with probability proportional to ${n \choose S} \pE_{\tzeta}[w_S]$.
      \item Let $\hat{\Sigma} = \frac{\pE_{\tzeta}[w_S \Sigma]}{\pE_{\tzeta}[w_S]}$  and $\hat{\mu} = \frac{\pE_{\tzeta}[w_S \mu]}{\pE_{\tzeta}[w_S]}$. %Compute the Eigenvalue Decomposition of $\tilde{\Pi} = \tilde{U}\tilde{\Lambda}\tilde{U}^{\top}$ and let $\hat{\Pi} = \tilde{U}_{r}\tilde{U}^{\top}_{r}$, where $\tilde{U}_{r}$ are the eigenvectors corresponding to the top-$r$ eigenvalues of $\tilde{\Pi}$.
      \item Add $(\hat{\mu},\hat{\Sigma})$ to the list $\cL$.
    \end{enumerate}
    \item[Output:]
      A list $\cL$ of parameters of size $O(1/\alpha^\Delta)$ containing $(\mu,\Sigma)$ satisfying $\Norm{\Sigma_*^{-1/2}(\mu-\mu_*)}_2^2 \leq O(s^{2} \alpha^{-2} \alpha^{-2/s})$, $\Omega\Paren{\frac{\alpha}{s}}^2 \alpha^{2/s} I \preceq  \Sigma_*^{-1/2} \hat{\Sigma} \Sigma_*^{-1/2}$, and $\Norm{I - \Sigma_*^{-1/2} \Sigma \Sigma_*^{-1/2}}_F^2 \leq O(h^{4} \alpha^{-4} \alpha^{-6/h}) $.
    \end{description}
  \end{algorithm}
\end{mdframed}



The goal of the pruning algorithm is to keep at most $O(1/\alpha)$ parameters from the large list above while ensuring that there's still a set of parameters close to $\mu_*,\Sigma_*$ in the resulting list. The key to this process is a test that takes a purported set of parameters, say $\hat{\mu},\hat{\Sigma}$ and finds if there's a weighting  (that serves as a certificate of goodness) of the input sample that gives a nice (certifiably hypercontractive and certifiably anti-concentrated) distribution with parameters close to $\hat{\mu},\hat{\Sigma}$. The parameters that are close to the true inliers are thus always accepted. We then run this test on pairwise separated set of parameters and show that at most $O(1/\alpha)$ of the tests accept.


\subsection{Analysis of the Algorithm}
In this section, we analyze Algorithm~\ref{alg:covariance-estimation} to prove Theorem~\ref{thm:main-theorem-LDC}.
We start with a high-level organization of the analysis.
% \begin{theorem}[List-Decodable Covariance Estimation in Strong Contamination Model]
% Let $\cD$ be an $h$-certifiably $C$-hypercontractive, $s$-certifiably $(\delta,C\delta)$-anti-concentrated isotropic distribution on $\R^d$.
% Let $Y$ be chosen according to $\cov_{\cD}(\alpha,\Sigma_*)$.
% Then, Algorithm~\ref{alg:covariance-estimation} when run on input $Y$ for $n \geq $, with probability at least $0.99$ over the choice of the sample $Y$ and the randomness of the algorithm, outputs a list of size $O(1/\alpha)$ guaranteed to contain $\hat{\Sigma}$ satisfying
% \begin{enumerate}
% \item $\Norm{\Sigma_*^{-1}\hat{\Sigma}-I}_F^2\leq 1/\alpha^{10}$.
% \item $\alpha \Sigma_* \preceq \hat{\Sigma} \preceq 1/\alpha \Sigma_*$.
% \end{enumerate}
% The algorithm runs in time $d^{??}$.
% \label{thm:main-analysis-LDC}
% \end{theorem}


% of the proof of Theorem~\ref{thm:main-analysis-LDC}.

\paragraph{Sample Inherits Population Properties.}
We first prove that with high probability over the draw of a large enough sample, the uniform distribution on $\cI$ (the inliers) is an affine transformation of a nice distribution. This implies the feasability of our constraint system, given sufficient samples.

\begin{lemma}[Sample vs Population] \label{lem:sample-vs-pop}
%\Pnote{get a precise version and prove in the appendix}\Anote{It may suffice to say that a similar proof appears in Appendix B.}
Suppose $n = \Omega\left( dk\log(k)/\eta^2+ 2^{2s} dk\log(k) + k\left( (sd\log d)^{s} + (hd)^{8h}  \right) \right) $. Then, with probability at least $0.99$ over the draw of the sample $\cI$, we have:

\begin{enumerate}
  \item Empirical mean: $\Norm{ \Sigma^{-1/2}_{*}  ( \mu  - \mu_{*})}^2_2 \leq \eta $ % \sqrt{\frac{\trace{\Sigma_{\ell}} }{m_\ell n}} + \sqrt{\frac{\|\Sigma_{\ell}\|_2d}{m_{\ell n}}}$
  \item Empirical covariance: $ \left(1 - \frac{1}{2^{2s}}\right)\Sigma_{*} \preceq  \Sigma \preceq \left(1 + \frac{1}{2^{2s}}\right) \Sigma_{*}$.
  \item Certifiable Anti-concentration:
  % \begin{enumerate}
  %   \item For all $y_i \in C_{\ell}$, \[ \forall v\in \mathbb{R}^d,
  %     \norm{v}_2^{2t-2} \iprod{y_i,v}^2 +\gamma_3^2 p^2 (\iprod{\Sigma_{\ell}^{-\frac{1}{2}} y_i,v})
  %     \geq \gamma_3^2 \norm{v}_2^{2t}
%     \]
\[
\sststile{2s}{v} \Set{
\frac{k^2}{n^2}\sum_{\substack{y_i, x_{j} \in C_{\ell} \\ i\neq j}}  p^2_{\cD}\left( \left\langle \Theta \Paren{\frac{y_i-y_j}{\sqrt{2}}},v\right\rangle \right)\leq 10\delta \|v\|^{2s}_2}
\]
  \item Certifiable Hypercontractivity:
\[
\sststile{2h}{Q} \Set{
\frac{k^2}{n^2} \sum_{\substack{y_i, x_{j} \in C_{\ell} \\ i\neq j}}  \Paren{\left\langle \Paren{ \Theta \Paren{\frac{y_i -y_j}{\sqrt{2}}}} \Paren{ \Theta  \Paren{\frac{y_i -y_j}{\sqrt{2}}}}^{\top},Q \right\rangle }^h
     \leq (Ch)^h\Norm{Q}_F^h}
  \]
\end{enumerate}


% \begin{enumerate}
% \item $\cI$ has $h$-certifiably $C$-hyper-contractive degree $2$ polynomials. % moments.
% \item $\cI$ is $s$-certifiably $(\delta, C\delta)$-anti-concentrated.
% \item $\E_{x \sim X} xx^{\top}\approx\Sigma_*$.
% \item $\E_{x \sim X} x = \mu_*$.
%  \end{enumerate}
\end{lemma}

In what follows, we will analyze the algorithm conditioned on the event that the sample $\cI$ satisfies the properties in lemma~\ref{lem:sample-vs-pop}. %Further, for the purpose of analyzing the algorithm and proving Theorem~\ref{thm:main-theorem-LDC}, we will assume that the empirical covariance of $\cI$, $\E_{x \sim X} xx^{\top} = I$. This is without loss of generality and can be ensured by simply working with a linear transformation of the input $Y$ if needed.


\paragraph{Guaranteeing High Intersection of $X'$ with $\cI$.} Observe that in our polynomial program, $\alpha = \frac{1}{n}\sum_{i=1}^n w_i$ measures the fraction of samples shared between $X'$ and $Y$. In order to guarantee that we can recover $(\hat{\mu},\hat{\Sigma})$ close to $\Sigma_*$, we need to ensure that a $\cI$ (that is unknown to the algorithm) and $X'$ share a significant fraction of samples.

% Towards this, let for each $1 \leq i \leq n$, define $w_i' = w_i \cdot \1(y_i = y_i)$. Then, as expected, $w'_i$ serves as the indicator of the samples in the intersection between $\cI$ and $X'$.

% \begin{lemma}[Intersection between $\cI$ and $X'$] \label{lem:intersection-indicator}
% For each $1 \leq  i \leq n$, let $w_i' = w_i \1(y_i = y_i)$. Then,
% \[
% \cA_2 \sststile{2}{X',w} \Set{w_i'(y_i -y_i) = 0}
% \]
% \end{lemma}
% \begin{proof}
% \[
% \cA_2  \sststile{2}{X',w} \Set{w_i'(y_i-y_i) = \1(y_i = y_i) \cdot w_i (y_i -y_i)  + \1(y_i = y_i) w_i'(y_i-y_i) = 0}\mper
% \]
% \end{proof}

If $\alpha > 1/2$, then one can simply conclude that $|\cI \cap X'| \geq \frac{1}{\alpha n} \sum_{i=1}^n w_i \geq 1-2\alpha$. This bound, however, is meaningless in our setting of $\alpha \ll 1/2$. To get around this hurdle, we rely on a result (first proven in~\cite{DBLP:journals/corr/abs-1905-05679}) that shows that given a pseudo-distribution $\tzeta$, $X'$ has an normalized intersection at least $\alpha^2$ with $\cI$ \emph{in expectation} provided that $\tzeta$ satisfies a ``max-entropy'' condition.  Let $w(\cI) = \frac{1}{\alpha n} \sum_{i \leq n}^n w_i$.

\begin{lemma}[High Intersection with Uncorrupted Sample, Lemma~4.3  in \cite{DBLP:journals/corr/abs-1905-05679}] \label{lem:high-entropy-intersection-original}
Let $\tzeta$ be a pseudo-distribution consistent with $\cA$ minimizing $\Norm{\frac{1}{\alpha n}\sum_{i\leq n} \pE_{\tzeta} w_i}_2^2$.  Then, $\pE_{\tzeta} w(\cI) \geq \alpha$.
\end{lemma}

Despite the above statement being true only ``in expectation'' over $\tzeta$, we will show that it is enough to list-decode the unknown covariance. % while pretending that the bound above holds ``pointwise''.

\paragraph{TV vs Parameter Distance Bounds.} Given the result above, our goal reduces to showing that whenever $X'$ satisfies the conditions of being (an affine transform of) a nice distribution, the distance between the covariance $\Sigma$ of $X'$ and the covariance $\Sigma_*$ of $\cI$ can be upper bounded in terms of the size of the intersection between $\cI$ and $X'$. In other words, we must relate the total variation distance between distributions (for uniform distributions on $\cI$,$X'$, this is simply the Hamming distance between $\cI$ and $X'$) to the distance between their parameters $\mu,\mu_*$ and $\Sigma, \Sigma_*$. Such results are fundamental in parametric statistics and are well-know for specific families (such as Gaussian distributions). Our job is to improve on these results on two fronts: 1) give a generalization of these results for all nice distributions instead of specific families and 2) prove them via a low-degree SoS proof. % These are simply low-degree SoS analogs of such results

Our first result bounds the spectral distance between $\Sigma$ and $\Sigma_*$ in terms of the intersection between $\cI$ and $X'$. Then, we prove:
\begin{lemma}[Spectral distance between covariances] \label{lem:spectral-distance-LDC} For every $t \in \N$,


% \[
% \cA \sststile{\Theta,w,X'}{2(t+s)} \Set{ w'(X)^{2t} \Norm{ \Theta(w)v}_2^{2s} \leq (2C\delta)^{2t} \kappa^s + 2 (s/\delta)^s \Norm{v}_2^{2s}}\mper
% \]
% \[
% \cA \sststile{\Theta,w,X'}{2(t+s)}\Set{ w'(X)^{2t} \Norm{ \Pi(w)v}_2^{2s} \leq (2C\delta)^{2t}\kappa^s + 2 (s/\delta)^s \Norm{v}_2^{2s}}\mper
% \]
% \[
% \cA \sststile{\Theta,w,X'}{2(t+s)} \Set{ w'(X)^{2} \Norm{ \Theta(w)v}_2^{2s} \leq (2C\delta)^{2} \kappa^s + 2 (s/\delta)^s \Norm{v}_2^{2s}}\mper
% \]
% \[
% \cA \sststile{\Theta,w,X'}{2(t+s)}\Set{ w'(X)^{2} \Norm{ \Pi(w)v}_2^{2s} \leq (2C\delta)^{2}\kappa^s + 2 (s/\delta)^s \Norm{v}_2^{2s}}\mper
% \]
% \begin{equation}
% \cA \sststile{2st}{v,\Theta,w} \Set{ 2 \Paren{\sum_{i = 0}^{st-1} w'(X)^{2st-2-2i} (2C\delta)^{2i}} s/\delta)^{s} \Norm{v}_2^{2s} + (2C\delta)^{2st} \norm{\Theta(w) v}_2^{2s} \geq \norm{\Theta(w) v}_2^{2s} \Paren{w'(X)^{2st}} }\mper
% \end
%\Pnote{fix degrees of SoS proofs below.}
\begin{enumerate}
  \item \textbf{Upper Bound : }
   \[
\cA \sststile{4st + 4s}{\Pi, w,v}\Set{ w(\cI)^{2st} \Norm{ \Sigma_*^{-1/2}\Pi(w)v}_2^{2s} \leq (2C\delta)^{2st}\kappa^s + 2\Paren{\sum_{i = 0}^{st-1} w(\cI)^{2st-2-2i} (2C\delta)^{2i}} (s/\delta)^s \Norm{v}_2^{2s}}\mper
\]

\item \textbf{Lower Bound: } \[
\cA \sststile{4st+4s}{\Pi,w,v} \Set{ \Norm{\Pi(w)\Sigma_*^{-1/2} v}_2^{2s} \geq \Paren{w(\cI)^2-C\delta)} \Paren{\frac{\delta}{s}}^{2s} \Norm{v}_2^{2s} }\mper
\]
\end{enumerate}
\end{lemma}
%\Pnote{the second statement here should derive the spectral approximation lemma. Perhaps write everything not requiring invertibility? Require a statement amenable to lower bounding eigenvalues. Fixed.}


Next, we bound the distance between the means $\mu_*$ and $\mu$ in terms of the intersection between $\cI$ and $X'$.
\begin{lemma}[Mean Closeness] \label{lem:mean-closeness-main}
For every $t \in \N$, and $e_t = 2\Paren{\sum_{i = 0}^{st-1} w(\cI)^{2st-2-2i} (2C\delta)^{2i}}$,

\begin{equation}
\cA \sststile{4st+4s}{w, \mu} \Biggl\{ w(\cI)^{4s+4st} \Norm{\mu_*-\mu(w)}_2^{4s} \leq  w(\cI)^{4s-2} \Paren{2Cs}^{2s} \Paren{ \Paren{w(\cI)^{2st} + (2C\delta)^{2st}}\kappa^s + e_t (s/\delta)^s}^2 \Biggr\}
\end{equation}


\end{lemma}

And finally, we bound the relative Frobenius distance between $\Sigma$ and $\Sigma_*$.

\begin{lemma}[Relative Frobenius Closeness of $\Sigma$] \label{lem:rel-frob-close-main} For every $t \in \N$, and $e_t = \Paren{\sum_{i = 0}^{ht-1} w(\cI)^{2ht-2-2i} (2C\delta)^{2i}}$,

\[
\cA \sststile{4ht + 4h}{\Sigma, w} \Biggl\{w(\cI)^{4h+4ht} \Norm{ I- \Sigma(w)}_F^{2h} \leq O(\Paren{ e_t^2 (h/\delta)^{2h} + (C\delta)^{2ht} \kappa^{2h}} h^{2h}) w(\cI)^{4h-4} \Biggr\}\mper
\]
\end{lemma}
\paragraph{Large-List Rounding.}
Our algorithm finds a pseudo-distribution $\tzeta$ consistent with $\cA$ and minimizing $\Norm{\pE_{\tzeta} w}_2^2$. We then apply a rounding algorithm to list-decode of the unknown mean and covariances.



\begin{lemma}[Analysis of Large-List Rounding] \label{lem:main-analysis-large-list-rounding}
Let $\Delta = O((h+s)(1+\log(\kappa)))$.
Let $\cL$ be the list obtained by independently repeating the sampling process above $1000 \Paren{\frac{1}{\alpha}}^\Delta$ times. Then, with probability at least $0.99$ $\cL$ contains a pair $(\mu,\Sigma)$ satisfying
\begin{enumerate}
  \item $\Norm{\Sigma_*^{-1/2} \Sigma \Sigma_*^{-1/2}-I}_F^2 \leq O(h^{4} \alpha^{-4} \alpha^{-6/h}) $
  \item  $\Omega\Paren{\frac{\alpha}{s}}^2 \alpha^{2/s} I \preceq  \Sigma_*^{-1/2} \hat{\Sigma} \Sigma_*^{-1/2}$
  \item $\Norm{\Sigma_*^{-1/2} (\mu-\mu_*)}_2^2 \leq O(s^{2} \alpha^{-2} \alpha^{-2/s})$
\end{enumerate}
\end{lemma}
\FIXME{add spectral closeness to the statement above.}\Anote{done.}



\paragraph{Pruning.} Finally, we describe a new algorithm to \textit{prune} the large list $\cL'$ from abovee down to a list of size $O(1/\alpha)$, while still maintaining a good approximation to the covariance in our list.
\Anote{Presentation task but the pruning algorithm from below can be copy pasted here.}



Theorem~\ref{thm:main-theorem-LDC} follows immediately by combining the aforementioned Lemmas.




% \subsection{Intersection Lower Bound (Lemma~\ref{lem:high-entropy-intersection-original})}

% The proof is similar to that of Lemma~4.3 in~\cite{DBLP:journals/corr/abs-1905-05679}. \Pnote{send to appendix.}
% \begin{proof}
% Let $u = \frac{1}{\alpha n}\pE[w]$. Then, $u$ is a non-negative vector satisfying $\sum_{i \sim [n]} u_i = 1$.

% Let $\wt(\cI) = \sum_{i \in \cI} u_i$ and $\wt(\cO) = \sum_{i \not \in \cI} u_i$. Then, $\wt(\cI) + \wt(\cO) = 1$.

% We will show that if $\wt(\cI) < \alpha$, then there's a pseudo-distribution $\tmu'$ that satisfies $\cA_{w,\ell}$ and has a lower value of $\|\pE[w]\|_2$. This is enough to complete the proof.

% To show this, we will ``mix'' $\tmu$ with another pseudo-distribution satisfying $\cA_{w,\ell}$. Let $\tmu^*$ be the \emph{actual} distribution supported on single $(X,w,\Sigma_*,\mu_*)$ - $X$ being the original uncorrupted sample and $w$ the indicator of intersection between $X$ and $Y$. Thus, $\pE_{\tmu^*} w_i = 1$ iff $i \in \cI$ and $0$ otherwise. $\tmu^*$ clearly satisfies $\cA$. Thus, any convex combination (mixture) of $\tmu$ and $\tmu^*$ also satisfies $\cA_{w,\ell}$.

% Let $\tmu_{\lambda} = (1-\lambda) \tmu + \lambda \tmu^*$. We will show that there is a $\lambda >0$ such that $\|\pE_{\tmu_{\lambda}}[w]\|_2 < \|\pE[w]\|_2$.

% % Let \[ \mu_C = \sum_{i \in C} u_i \text{ and  } 1-\mu_C = \sum_{i \in [m]\setminus C} u_i. \]
% We first lower bound $\|u\|_2^2$ in terms of $\wt(\cI)$ and $\wt(\cO)$. Observe that for any fixed values of $\wt(\cI)$ and $\wt(\cO)$, the minimum is attained by the vector $u$ that ensures $u_i = \frac{1}{\alpha n} \wt(\cI)$ for each $i \in \cI$ and $u_i = \frac{1}{(1-\alpha)n} \wt(\cO)$. \begin{align*}
%   \text{This gives }  \|u\|^2 &\geq \left( \frac{\wt(\cI)}{\alpha n} \right)^2 \alpha n + \left(\frac{1-\wt(\cI)}{(1-\alpha) n}\right)^2 (1-\alpha) n
%     = \frac{1}{\alpha n}\cdot \left( \wt(\cI) + (1-\wt(\cI))^2 \left(\frac{\alpha}{1-\alpha}\right) \right)\mper
% \end{align*}
% Next, we compute the the $\ell_2$ norm of $u' = \frac{1}{\alpha n} \pE_{\tmu_{\lambda}} w$ as:
% \[ \|u'\|_2^2 = (1-\lambda)^2 \|u\|^2 +  \frac{\lambda^2}{\alpha n} + 2 \lambda(1-\lambda)\frac{\wt(\cI)}{\alpha n} \mper\]
% \begin{align*}
%     \text{Thus, } \|u'\|^2 - \|u\|^2  &= (-2\lambda+\lambda^2) \|u\|^2 +  \frac{\lambda^2}{\alpha n} + 2 \lambda(1-\lambda)\frac{\wt(\cI)}{\alpha n}\\
%     &\leq \frac{-2\lambda+\lambda^2}{\alpha n}\cdot \left( \wt(\cI)^2 + (1-\wt(\cI))^2 \frac{\alpha}{1-\alpha} \right) +  \frac{\lambda^2}{\alpha n} + 2 \lambda(1-\lambda)\frac{\wt(\cI)}{\alpha n}
% \end{align*}
% \begin{align*} \text{Rearranging, }\|u\|^2 - \|u'\|^2 &\geq \frac{\lambda}{\alpha n} \left( (2-\lambda) \cdot \left( \wt(\cI)^2 + (1-\wt(\cI))^2 \left(\frac{\alpha}{1-\alpha}\right) \right) -  \lambda - 2 (1-\lambda)\wt(\cI)\right)\\
% &\geq \frac{\lambda ( 2-\lambda)}{\alpha n} \left( \wt(\cI)^2 + (1-\wt(\cI))^2 \frac{\alpha}{1-\alpha} - \wt(\cI)\right)
% \end{align*}
% Now, whenever $\wt(\cI) < \alpha$, $\wt(\cI)^2 + (1-\wt(\cI))^2 \frac{\alpha}{1-\alpha} - \wt(\cI)> 0$. Thus, we can choose a small enough $\lambda > 0$ so that $\|u\|^2 - \|u'\|^2 > 0$. % contradicting that $u$ takes minimum norm under the conditions of the problem. Hence $\mu_C > \alpha$ and $Z \geq \alpha m$.
% \end{proof}

\subsection{Spectral Distance Bound (Lemma~\ref{lem:spectral-distance-LDC})}


The spectral distance bound implies that no eigenvalue of our estimate of the covariance shrinks too much.
The key property of the inliers that we exploit here is certifiable anti-concentration of the inlier distribution. We note that such a statement was originally discovered for rank-deficient covariances in \cite{}.

\Pnote{add commentary saying this technique was invented in subspace recovery paper.}\Anote{done.}
%\Anote{added the normalization constant infront of the sum below.}
\begin{lemma} \label{lem:spectral-step-1-LDC} For $w(\cI) = \frac{1}{\alpha n} \sum_{i \in \cI} w_i$,
% \begin{equation}
% \cA \sststile{2s}{v} \Set{(s/\delta)^{2s} \Norm{v}_2^{2s} \geq \norm{\Sigma_*^{1/2} \Theta(w)  v}_2^{2s} \Paren{\frac{1}{n^2} \sum_{i \neq j \in [n]} w'_i w'_j- 2C\delta }  }\mper
% \end{equation}


\[
\cA \sststile{2s}{v} \Set{ (s/\delta)^{2s}\Norm{v}_2^{2s} \geq \norm{\Pi(w) \Sigma_{*}^{-1/2} v}_2^{2s} \Paren{w(\cI)^2- 2C\delta }  }\mper
\]

\begin{equation}
\cA \sststile{2s}{v} \Set{(s/\delta)^{2s} \Norm{\Pi(w)\Sigma_*^{-1/2} v}_2^{2s} \geq \norm{v}_2^{2s} \Paren{w(\cI)^2- 2C\delta }  }\mper
\end{equation}

\end{lemma}


\begin{proof}
From Lemma~\ref{lem:sample-vs-pop}, we know that two-point-centering of $\cI$ is $2s$-certifiably $(\delta,C\delta)$-anti-concentrated with witness polynomial $p_{\cD}$. Thus, we must have:
\begin{enumerate}
\item for every $i,j\in [n]$,
\begin{equation} \label{eq:p-of-zero-use} \cA \sststile{2s}{v} \Set{\norm{v}_2^{2s-2} \Iprod{\Paren{\frac{y_i-y_j}{\sqrt{2}}},v}^2 + \delta^2 p_{\cD}^2\Paren{\Iprod{\Paren{\frac{y_i-y_j}{\sqrt{2}}},v}} \geq \delta^2 \norm{v}_2^{2s}} \mper \end{equation}
\item \begin{equation} \label{eq:cert-anti-conc-use} \cA \sststile{2s}{v} \Set{\frac{1}{\alpha^2 n^2} \sum_{i \neq j \in \cI}  p_{\cD}^2\Paren{\Iprod{\Paren{\frac{y_i-y_j}{\sqrt{2}}},v}} \leq C\delta  \norm{v}_2^{2s}}\mper
\end{equation}
\end{enumerate}


Multiplying by $\frac{1}{\alpha^2 n^2} w_i w_j$ and summing up \eqref{eq:p-of-zero-use} over all $i \neq j \in \cI$,  yields:
\begin{multline}
\cA \sststile{2s}{v} \Biggl\{\frac{1}{\alpha^2 n^2}\sum_{i \neq j \in \cI} w_i w_j \Paren{\norm{v}_2^{2s-2} \Iprod{\Paren{\frac{y_i-y_j}{\sqrt{2}}},v}^2 + \delta^2 p_{\cD}^2\Paren{\Iprod{\Paren{\frac{y_i-y_j}{\sqrt{2}}},v}}} \\ \geq \delta^2 \norm{v}_2^{2s} \Paren{\frac{1}{\alpha^2 n^2} \sum_{i \neq j \in \cI} w_i w_j} \Biggr\}\mper
\end{multline}
We simplify notation and use $\E_{w}$ to denote the expectation over pairs $w_i , w_j$ such that $i, j \in \cI$ and $i\neq j$.


Next, we use that $\Set{{w_i}^2 = w_i} \sststile{2}{w} \Set{w_i \leq 1} \cup \Set{0 \leq w_i}$ and \eqref{eq:cert-anti-conc-use} to conclude:
\begin{equation}
\cA \sststile{2s}{v} \Biggl\{ \expecf{w}{p_{\cD}^2\Paren{\Iprod{\Paren{\frac{y_i-y_j}{\sqrt{2}}},v}}} \leq \frac{1}{\alpha^2 n^2}\sum_{i\neq j \in \cI}  p_{\cD}^2\Paren{\Iprod{\Paren{\frac{y_i-y_j}{\sqrt{2}}},v}} \leq C\delta \Norm{v}_2^{2s} \Biggr\}\mper
\end{equation}

Combining the above two observations yields:%\sststile{2t}{v} \Set{\E_{x \sim D} p^2\Paren{\Iprod{x,v} \leq C\delta \norm{v}_2^{2t}}}$, we have:
\begin{equation}
\cA \sststile{2s}{v} \Set{ \expecf{w}{\norm{v}_2^{2s-2} \Iprod{\Paren{\frac{y_i-y_j}{\sqrt{2}}},v}^2}  \geq \delta^2 \norm{v}_2^{2s} \Paren{w(\cI)^2- C\delta }}\mper \label{eq:X-spectral-LB}
\end{equation}

On the other hand, we have the following simple \emph{upper bound}:
\begin{equation}
\Set{{w_i}^2 = w_i \forall i} \sststile{}{} \Biggl\{\Norm{v}_2^2 \geq \expecf{w}{\Iprod{\Paren{\frac{y_i-y_j}{\sqrt{2}}}, v}^2}\Biggr\}\mper
\label{eq:X-spectral-UB}
\end{equation}



A similar argument utilizing the certifiable-anti-concentration constraints $\cA_4$ yields:

\begin{equation}
\cA \sststile{2s}{v} \Set{ \expecf{w}{\norm{v}_2^{2s-2} \Iprod{\Theta(w)\Paren{\frac{y_i-y_j}{\sqrt{2}}},v}^2}  \geq \delta^2 \norm{v}_2^{2s} \Paren{w(\cI)^2- C\delta }}\mper  \label{eq:Xp-spectral-LB}
\end{equation}

And an  analog of the simple upper bound  argument above yields:
\begin{equation}
\cA \sststile{2}{v} \Set{\Norm{v}_2^2 \geq  \expecf{w}{\Iprod{  \Theta(w) \Paren{\frac{y_i-y_j}{\sqrt{2}}},v}^2}}\mper \label{eq:Xp-spectral-UB}
\end{equation}

We now substitute $v \rightarrow \Sigma(w)^{-1/2} v$ in \eqref{eq:X-spectral-LB}.
\begin{multline}
\cA \sststile{2s}{v} \Biggl\{\expecf{w}{\norm{\Theta(w) v}_2^{2s-2} \Iprod{\Paren{\frac{y_i-y_j}{\sqrt{2}}},\Theta(w) v}^2 } \geq \delta^2 \norm{\Theta(w) v}_2^{2s} \Paren{ w(\cI)^2- C\delta } \Biggr\}\mper  \label{eq:X'-spectral-LB}
\end{multline}

Observing that $\Iprod{\Paren{\frac{y_i-y_j}{\sqrt{2}}}, \Theta(w) v} = \Iprod{\Theta(w) \Paren{\frac{y_i-y_j}{\sqrt{2}}},v}$ and combining with \eqref{eq:Xp-spectral-UB}
\[
\cA \sststile{2s}{v} \Set{\Norm{v}_2^2 \Norm{ \Theta(w)v}_2^{2s-2} \geq  \expecf{w}{\norm{\Theta(w) v}_2^{2s-2} \Iprod{  \Theta(w) \Paren{\frac{y_i-y_j}{\sqrt{2}}},v}^2}}\mper \label{eq:X'-spectral-UB}
\]

Combining the last two statements yields:
\begin{equation}
\cA \sststile{2s}{v} \Set{\Norm{v}_2^2 \Norm{ \Theta(w)v}_2^{2s-2} \geq \delta^2 \norm{\Theta(w) v}_2^{2s} \Paren{w(\cI)^2- C\delta }  }\mper \label{eq:X'-spectral-UB}
\end{equation}

Next, for any $\tau > 0$, $\Norm{v}_2^2 \Norm{\Theta(w)v}_2^{2s-2} = \Paren{\Norm{v}_2^2/\tau^{s-1}} \Paren{\Norm{ \Theta(w)v}_2^{2s-2} \cdot \tau^{s-1}}$.
Using the SoS AM-GM Inequality (Fact~\ref{fact:sos-am-gm}) with the setting $f_1=\Norm{v}_2^2/\tau^{s-1}$ and $f_2 = \ldots = f_{s} = \tau \Norm{\Theta(w)v}_2^2$ to obtain that:

\[
\sststile{v}{s} \Set {\Norm{v}_2^2 \Norm{ \Theta(w)v}_2^{2s-2} \leq s^{-s} \Paren{\Norm{v}_2^2/\tau^{s-1} + (s-1) \tau \Norm{\Theta(w)v}_2^2}^s}\mper
\]
Using the SoS almost triangle inequality (Fact~\ref{fact:sos-almost-triangle}),
\[
\sststile{}{} \Set {\Norm{v}_2^2 \Norm{\Theta(w)v}_2^{2s-2} \leq \Paren{\Norm{v}_2^{2s}/\tau^{s^2-s} + (s-1) \tau^s \Norm{\Theta(w)v}_2^{2s}}}\mper
\]
Let's now plug in $\tau = \Paren{\delta/s}^{1/s}$. Observing that $(s-1) \tau^s \leq \delta$. Thus, combining with the above: % and combining with \eqref{eq:X'-spectral-UB} and rearranging gives:
\begin{equation}
\cA \sststile{2s}{v} \Set{(s/\delta)^{s-1} \Norm{v}_2^{2s} \geq \norm{ \Theta(w) v}_2^{2s} \Paren{w(\cI)^2- 2C\delta }  }\mper \label{eq:X'-spectral-UB}
\end{equation}
A similar argument using \eqref{eq:Xp-spectral-LB} and \eqref{eq:Xp-spectral-UB} yields:
\[
\cA \sststile{2s}{v} \Set{ (s/\delta)^{s}  \Norm{\Pi(w)v}_2^{2s} \geq \norm{v}_2^{2s} \Paren{w(\cI)^2- 2C\delta }  }\mper \label{eq:X'-spectral-UB}
\]




\end{proof}




To finish the proof of Lemma~\ref{lem:spectral-distance-LDC}, we need the following two results. First, we use some rough upper bounds on $\Norm{\Sigma_*^{1/2} \Theta(w)v}_2^{2s}$.

\begin{lemma} \label{lem:cond-number-upper-bound}
\[
\cA_1 \sststile{4s}{\Theta,w, v} \Set{ \Norm{\Sigma_*^{1/2} \Theta(w)v}_2^{2s} \leq \kappa^s \Norm{v}_2^{2s}}\mper
\]
\[
\cA_1 \sststile{4s}{\Pi,w,v} \Set{ \Norm{ \Pi(w)\Sigma_*^{-1/2}v}_2^{2s} \leq \kappa^s \Norm{v}_2^{2s}}\mper
\]
\end{lemma}

\begin{proof}
We prove the first claim.
The proof of the second one is similar.

\begin{align*}
\cA_1 &\sststile{4s}{\Theta,w,v} \Biggl\{ \Paren{\Norm{\Sigma_*^{1/2} \Theta(w)v}_2^{2}}^s\leq \Paren{\lambda_u \Norm{\Theta(w)v}_2^2}^s = \lambda_u^s \Paren{v^{\top} \Theta(w)^2 v}^s \leq \Paren{\frac{\lambda_u}{\lambda_l}}^s \Norm{v}_2^{2s} = \kappa^s \Norm{v}_2^{2s}
\Biggr\}\mper
\end{align*}


\end{proof}

% \begin{proof}[Proof of Spectral Distance Lemma]
% We prove the first claim. The proof of the other claim is similar.
% Rearranging the first conclusion of Lemma~\ref{lem:spectral-step-1-LDC}, we have:
% \begin{equation}
% \cA \sststile{2s}{v} \Set{\Norm{v}_2^{2s}/(\delta/s)^{2s} + 2C\delta \norm{\Sigma_*^{1/2} \Theta(w)  v}_2^{2s} \geq \norm{\Sigma_*^{1/2} \Theta(w)  v}_2^{2s} \Paren{\frac{1}{n^2} \sum_{i \neq j \in [n]} w'_i w'_j}  }\mper
% \end{equation}
% Applying Lemma~\ref{lem:cond-number-upper-bound} now yields:
% \begin{equation}
% \cA \sststile{2s}{v} \Set{\norm{\Sigma_*^{1/2} \Theta(w)  v}_2^{2s} \Paren{\frac{1}{n^2} \sum_{i \neq j \in [n]} w'_i w'_j} \leq \Norm{v}_2^{2s}/(\delta/s)^{2s} + 2C\delta \kappa^s \Norm{v}_2^{2s} }\mper
% \end{equation}
% \end{proof}

And next, we will use the following general result that allows reducing error by ``powering up''.

\begin{lemma}[General Powering] \label{lem:gen-powering}
Let $A,B,C$ be indeterminates. Then, for all $\beta \geq 0$, we have:
\[
\Set{A \geq 0} \cup \Set{ (A-\beta)B \leq C} \sststile{t+1}{A,B,C} \Set{ A^t B \leq \beta^t B +  \Paren{\sum_{i = 0}^{t-1}A^{t-1-i} \beta^i} C}\mper
\]
\end{lemma}

\begin{proof}

We start with the polynomial identity: $\Paren{\sum_{i = 0}^{t-1}A^{2(t-1-i)} \beta^i} (A-\beta) = A^{2t} - \beta^t$.
Since $\beta \geq 0$,  $ \Set{A \geq 0} \sststile{t}{A} \Set{\sum_{i = 0}^{t-1}A^{2(t-1-i)} \beta^i}$ is a square polynomial in the indeterminate $A$, we have:
%\Anote{I don't think this is a square polynomial in A or $\beta$. For t = 2, this is simply $A + \beta$.}
\[
\Set{ (A-\beta)B \leq C} \sststile{2t+1}{A,B,C} \Set{ \sum_{i = 0}^{t-1}A^{2(t-1-i)} \beta^i (A-\beta) B \leq \Paren{\sum_{i = 0}^{t-1}A^{2(t-1-i)} \beta^i} C}\mper
\]
%\Anote{Maybe we can restate the sum as $\sum^{t-1}_{i=0}A^{2(t-i-1)}\beta^{i} $, since this suffices for our application.}
Rearranging gives the lemma.

% We use induction over the parameter $t$ to prove that
% \[
% \Set{1 \geq A \geq 0} \cup \Set{ (A-\beta)B \leq C} \sststile{A,B,C}{2t} \Set{ A^t B \leq \beta^t B + \Paren{\sum_{i = 0}^{t-1} \beta^{i}} C}\mper
% \]

% The base case follows from the axioms. For the inductive case, we have:
% \begin{align*}
% \Set{1 \geq A \geq 0} \cup \Set{ (A-\beta)B \leq C} &\sststile{A,B,C}{2t} \Biggl\{ A^t B = A( A^{t-1}B) \\
% &\leq A (\beta^{t-1}B+ \Paren{\sum_{i = 0}^{t-2} \beta^{i}} C)\\
% &\leq \beta^{t} B + \beta^{t-1} C  + \Paren{\sum_{i = 0}^{t-2} \beta^{i}}\\
% &=  \beta^{t}B+ \Paren{\sum_{i = 0}^{t-1} \beta^{i}}
% \Biggr\}\mper
% \end{align*}
\end{proof}


We are now ready to finish the proof of Lemma~\ref{lem:spectral-distance-LDC}.
\begin{proof}[Proof of Lemma~\ref{lem:spectral-distance-LDC}]
The second statement is the second claim in Lemma~\ref{lem:spectral-distance-LDC}. Let's prove the first statement. %The proof of the second is similar.
From Lemma~\ref{lem:spectral-step-1-LDC}, we have:
\begin{equation}
\cA \sststile{2s}{v, \Theta,w} \Set{(s/\delta)^{s} \Norm{v}_2^{2s} \geq \norm{\Theta(w) v}_2^{2s} \Paren{\frac{1}{\alpha^2 n^2} \sum_{i \neq j \in \cI} w_i w_j- 2C\delta }  }\mper
\end{equation}

Applying Lemma~\ref{lem:gen-powering} with $A = \frac{1}{\alpha^2 n^2} \sum_{i \neq j \in [n]} w_i w_j$, $B = \norm{\Theta(w) v}_2^{2s}$ and $\beta = 2C\delta \ll 1/2$, we obtain:

\begin{equation}
\cA \sststile{4st}{v,\Theta,w} \Set{ 2 \Paren{\sum_{i = 0}^{st-1} w(\cI)^{2st-2-2i} (2C\delta)^{2i}} (s/\delta)^{s} \Norm{v}_2^{2s} + (2C\delta)^{2st} \norm{\Theta(w) v}_2^{2s} \geq \norm{\Theta(w) v}_2^{2s} \Paren{w(\cI)^{2st}} }\mper
\end{equation}

Plugging in the bound from Lemma~\ref{lem:cond-number-upper-bound} on the LHS above completes the proof.






\end{proof}

\subsection{Mean Distance Bound (Lemma~\ref{lem:mean-closeness-main})}

\begin{proof}[Proof of Lemma~\ref{lem:mean-closeness-main}]
%Observe that $\cA_2 \sststile{2}{w} \Set{ \frac{1}{\alpha n} \sum_{j \in [n]} w_i y_i  = \frac{1}{n} \sum_{j \in [n]} w'_i x'_i}$.
%\Anote{Here, the notation is $w(I)$ but the original statement its $w(X)$. In weak contamination, these are equivalent but we should be consistent, lmk which one your prefer and i can fix it. }
We apply the linear transformation $z \rightarrow \Sigma_*^{-1/2} z$ and work with the transformed points in the argument below.
\begin{align*}
\cA \sststile{2st+4s}{w,\mu} &\Biggl\{ w(\cI)^{2st} \Paren{w(\cI)^{2s} \Iprod{\mu_*-\mu(w),v}^{2s}} &= w(\cI)^{2st}\Paren{ \Iprod{\mu_* -\frac{1}{\alpha  n} \sum_{j \in \cI} w_i y_i + \frac{1}{\alpha n} \sum_{j \in \cI} w_i y_i- \mu,v}^{2s}}\\
&\leq w(\cI)^{2st} 2^{2s} \Paren{ \frac{1}{\alpha n} \sum_{i \in \cI} w_i \Iprod{y_i - \mu_*, v}^{2s} \frac{1}{\alpha n} \sum_{i \in \cI} w_i \Iprod{y_i - \mu, v}^{2s}} \\
&\leq w(\cI)^{2st} 2^{2s} \Paren{ \Paren{\frac{1}{\alpha n} \sum_{j \in \cI} {w_j}^{2s}}^{2s-1} \Paren{\frac{1}{\alpha n} \sum_{j \in \cI} \Iprod{y_j-\mu_*,v}^{2s}} + \Paren{\frac{1}{\alpha n} \sum_{j \in \cI} {w_j}^{2s}}^{2s-1} \Paren{\frac{1}{\alpha n} \sum_{j \in [n]} w_i \Iprod{y_j-\mu,v}^{2s}}}\\
&\leq  w(\cI)^{2st} \Paren{2Cs}^{s}  w(\cI)^{2s-1} \Paren{ \Norm{v}_2^{2s} + \Norm{\Pi(w) v}_2^{2s}}\\
&\leq  \Paren{2Cs}^{s}  (w(\cI)^{2st+2s-1} + w(\cI)^{2s-1} (2C\delta)^s \kappa^s + e_t w(\cI)^{2s-1} (s/\delta)^{s})  \Norm{v}_2^{2s}
\Biggr\}\mper
%&\leq \Paren{2C\sqrt{t}}^{2t}  \Paren{\frac{k}{n} \sum_{j \in C_r} w_j}^{2t-1} \Paren{ \Paren{v^{\top} \Paren{\Sigma(r)+\Sigma(w)} v}^{t}}
%\mper
\end{align*}

where we used the bound from Lemma~\ref{lem:spectral-distance-LDC} in the last inequality and $e_t = 2\Paren{\sum_{i = 0}^{st-1} w(\cI)^{2st-2-2i} (2C\delta)^{2i}}$.% and $\cA \sststile{}{} \Set{w'(X) \leq 1}$ in the final inequality.
% Multiplying both sides by $w'(X)^{2t}$ (note that $\cA \sststile{2t}{w} \Set{w'(X)^{2t} \geq 0}$), yields:
% \begin{multline}
% \cA \sststile{}{} \Biggl\{\Paren{w'(X)^{2s+2t} \Iprod{\mu_*-\mu(w),v}^{2s}} \leq  w'(X)^{2t} \Paren{ 2C\sqrt{s}}^{2s}  w'(X)^{2s-1} \Paren{ \Norm{v}_2^{2s} + \Norm{\Theta(w) v}_2^{2s}}\\ \leq \Paren{ 2C\sqrt{s}}^{2s}  w'(X)^{2s-1} \Norm{v}_2^{2s}  \Paren{ 1 + (s/\delta)^{2s} + (2C\delta)^{2t} \kappa^s }  \Biggr\}
% \end{multline}
Plugging in $v = (\mu_*-\mu)$ and using Lemma~\ref{lem:cancellation-sos} yields:
\begin{multline}
\cA \sststile{4st+4s}{w,\mu} \Biggl\{\Paren{w(\cI)^{4s + 4st} \Norm{\mu_*-\mu(w)}_2^{4s}} \\\leq  w(\cI)^{4s-2} \Paren{2Cs}^{2s} \Paren{(w(\cI)^{4st}+ (2C\delta)^{st} \kappa^s + 2\Paren{\sum_{i = 0}^{st-1} w(\cI)^{2st-2-2i} (2C\delta)^{2i}} (s/\delta)^s }^2 \Biggr\}
\end{multline}



\end{proof}


\subsection{Relative Frobenius Distance Bound (Lemma~\ref{lem:rel-frob-close-main})}

We will use the following results that follow from certifiable hypercontractivity of $\cI$ and $\cA_5$ for $\I$.
\begin{lemma} [Frobenius Distance of Subsamples] \label{lem:frob-dist-subsample-LDC}

\[
\cA \sststile{4ht + 4h}{w}\\ \Set{ \Norm{\frac{1}{\alpha^2 n^2} \sum_{i \neq j \in \cI}^n w_iw_j \Paren{\frac{y_i-y_j}{\sqrt{2}}} \Paren{\frac{y_i-y_j}{\sqrt{2}}}^{\top}- w(\cI)^2 I}_F^{2ht} \leq (Ch)^{2th} w(\cI)^{4ht-4h} }  \mper
\]

\[
\cA \sststile{4ht+4h}{w, \Pi}\\ \Set{ \Norm{\frac{1}{\alpha n^2} \sum_{i \neq j \in \cI}^n w_iw_j \Theta \Paren{\frac{y_i-y_j}{\sqrt{2}}} \Paren{\frac{y_i-y_j}{\sqrt{2}}}^{\top} \Theta^{\top}- w(\cI)^2 I}_F^{2ht} \leq (Ch)^{2th} w(\cI)^{4ht-4h} }  \mper
\]

\end{lemma}
\begin{proof}
We prove the first claim above - the proof of the other is similar.
Let $P$ be a $d \times d$ matrix-valued indeterminate. Let $\E_{w}$ denote the expectation over pairs indicated by $w_i, w_j$ such that $i,j \in \cI$ and $i \neq j$.  By an application of the SoS Hölder's inequality followed by certifiable hypercontractivity of $\cI$, we have:
\begin{align*}
\cA &\sststile{4ht+4h}{w,P} \Biggl\{ \Paren{\expecf{w}{\Iprod{\Paren{\frac{y_i-y_j}{\sqrt{2}}} \Paren{\frac{y_i-y_j}{\sqrt{2}}}^{\top},P}}- \expecf{w}{\Iprod{P,I}}}^{ht} \\
&= \Paren{ \expecf{w}{\Iprod{\Paren{\frac{y_i-y_j}{\sqrt{2}}} \Paren{\frac{y_i-y_j}{\sqrt{2}}}^{\top} -\II ,P}}}^{ht} \\
&= \Paren{\frac{1}{\alpha^2 n^2} \sum_{i \neq j\in \cI} {w_i}^{ht-1} {w_j}^{ht-1} \Iprod{\Paren{\frac{y_i-y_j}{\sqrt{2}}} \Paren{\frac{y_i-y_j}{\sqrt{2}}}^{\top}-\II,P}}^{ht}\\
&\leq \Paren{\frac{1}{\alpha^2 n^2} \sum_{i \neq j\in \cI} {w_i}^{ht} {w_j}^{ht}}^{ht-1} \Paren{\frac{1}{\alpha^2 n^2} \sum_{i \neq j\in \cI} \Iprod{\Paren{\frac{y_i-y_j}{\sqrt{2}}} \Paren{\frac{y_i-y_j}{\sqrt{2}}}^{\top}-\II,P}^{ht}}\\
&\leq  \Paren{ w(\cI)^2}^{ht-1}  \cdot (Ch)^{ht} \Norm{P}_F^{ht}\\
&=  \Paren{ w(\cI)^2}^{ht-1} \cdot (Ch)^{ht} \Norm{P}_F^{ht} \Biggr\}  \mper
\end{align*}

Here, the first inequality follows from Fact~\ref{fact:sos-holder} and the second one by the certifiable hypercontractivity of $\cI$.
Substituting $P = \expecf{w}{\Paren{\frac{y_i-y_j}{\sqrt{2}}} \Paren{\frac{y_i-y_j}{\sqrt{2}}}^{\top} } - w(\cI)^2I$ and applying SoS Cancellation (Lemma~\ref{lem:cancellation-sos}) completes the proof.
\end{proof}


\begin{proof}[Proof of Lemma~\ref{lem:rel-frob-close-main}]

Recall that $w(\cI) = \frac{1}{\alpha n} \sum_{i \in \cI} w_i$. By the SoS almost triangle inequality (Fact~\ref{fact:sos-almost-triangle}), we have:
\begin{multline}
\sststile{4ht+4h}{w,\Sigma} \Biggl\{ \Norm{w(\cI)^2 I- w(\cI)^2\Sigma(w)}_F^{2ht} \\\leq 2^{2ht} \Norm{w(\cI)^2 I-  \expecf{w}{\Paren{\frac{y_i-y_j}{\sqrt{2}}}\Paren{\frac{y_i-y_j}{\sqrt{2}}}^{\top}} }_F^{2ht}\\
+ 2^{2ht} \Norm{ \expecf{w}{\Paren{\frac{y_i-y_j}{\sqrt{2}}}\Paren{\frac{y_i-y_j}{\sqrt{2}}}^{\top}}- w(\cI)^2\Sigma(w)}_F^{2ht}\Biggr\}\mper \label{eq:main-split-frob-LDC}
\end{multline}
By Lemma~\ref{lem:frob-dist-subsample-LDC}, the first term is upper bounded by:
\[
2^{2ht}(Ch)^{2ht} w(\cI)^{4ht-4h}\leq (2Ch)^{2ht} w(\cI)^{4ht-4h}  \mper
\]

Let's analyze the second term and put it in a form that is pliable.
By noting that $\cA_1 \sststile{2}{\Pi,\Theta,\Sigma} \Set{\Pi \Theta = I} \cup \Set{ \Pi^2 = \Sigma(w)}$, we have: \Anote{editing here.}
\begin{multline}
w(\cI)^{4ht} \Norm{ \expecf{w}{\Paren{\frac{y_i-y_j}{\sqrt{2}}}\Paren{\frac{y_i-y_j}{\sqrt{2}}}^{\top}}- w(\cI)^2\Sigma(w) }_F^{2ht} \\= w(\cI)^{4tt}\Norm{ \expecf{w}{\Paren{\Pi \Theta \frac{y_i-y_j}{\sqrt{2}}}\Paren{\Pi \Theta \frac{y_i-y_j}{\sqrt{2}}}^{\top}}-w(\cI)^2\Pi^2(w)}_F^{2ht}
\end{multline}
%\Anote{changing the above from $w^{2s}$ to $w^{4st}$}
And, the RHS above can be rewritten as:
\begin{multline}
w(\cI)^{4ht} \Norm{\Pi \Paren{ \expecf{w}{\Paren{\Theta \frac{y_i-y_j}{\sqrt{2}}}\Paren{\Theta \frac{y_i-y_j}{\sqrt{2}}}^{\top}}-w(\cI)^2I}\Pi}_F^{2ht}
\end{multline}

From Lemma~\ref{lem:spectral-distance-LDC}, we know that:
\[
\cA \sststile{4ht + 4h}{\Pi, \Theta , w} \Set { w(\cI)^{2st} \Norm{\Pi(w)v}_2^{2s} \leq \Paren{ e_t (s/\delta)^{s} + (C\delta)^{st} \kappa^s} \Norm{v}_2^{2s}}\mper
\]
where $e_t = 2\Paren{\sum_{i = 0}^{st-1} w(\cI)^{2st-2-2i} (C\delta)^{i}}$.


We now apply Lemma~\ref{lem:contraction-property} with $AA^{\top} = w(\cI)^{2ht} \Pi(w)\Pi(w)^{\top}$ and $B = \Paren{ \expecf{w}{\Paren{ \Theta \frac{y_i-y_j}{\sqrt{2}}}\Paren{\Theta \frac{y_i-y_j}{\sqrt{2}}}^{\top}}-w(\cI)^2I}\Pi$  to get an upper bound on the  second  term above of:

\[
\cA \sststile{4ht+4h}{w, \Theta, \Pi} \Biggl\{ w(\cI)^{2ht}\Paren{ e_t (h)^{h} + (C\delta)^{ht} \kappa^h} h^h \Norm{\Paren{ \expecf{w}{\Paren{\Theta \frac{y_i-y_j}{\sqrt{2}}}\Paren{\Theta \frac{y_i-y_j}{\sqrt{2}}}^{\top}}-w(\cI)^2I}\Pi}_F^{2ht}\Biggr\}\mper
\]

Another application of Lemma~\ref{lem:contraction-property} now yields:

\begin{multline}
\cA \sststile{4ht+4h}{w, \Theta, \Pi}w(\cI)^{2ht} \Norm{\Pi \Paren{\expecf{w}{\Paren{\Theta \frac{y_i-y_j}{\sqrt{2}}}\Paren{\Theta \frac{y_i-y_j}{\sqrt{2}}}^{\top}}-w(\cI)^2 I}\Pi}_F^{2ht} \\\leq  \Paren{ e_t (h)^{ht} + (C\delta)^{ht} \kappa^h}^2 h^{2h} \Norm{w(\I)^2 I- \expecf{w}{\Paren{\Theta \frac{y_i-y_j}{\sqrt{2}}}\Paren{\Theta \frac{y_i-y_j}{\sqrt{2}}^{\top}} }}_F^{2ht}\mper
\end{multline}

Finally, using Lemma~\ref{lem:frob-dist-subsample-LDC} again yields:
\[
\cA \sststile{4ht+4h}{w, \Theta, \Pi} \Set{\Norm{w(\cI)^2 I- \expecf{w}{\Paren{\Theta \frac{y_i-y_j}{\sqrt{2}}}\Paren{\Theta \frac{y_i-y_j}{\sqrt{2}}^{\top}} }}_F^{2ht} \leq \Paren{ e_t (h)^{ht} + (C\delta)^{ht} \kappa^{h}}^2 s^{2ht} (Ch)^{2ht} w(\cI)^{4ht-4h}}\mper
\]

Combining the above bounds on the two terms on the RHS of \eqref{eq:main-split-frob-LDC} and using that $\cA \sststile{}{} \Set{w(\cI) \leq 1}$ yields:

\[
\cA \sststile{4ht + 4s}{w, \Sigma } \Biggl\{w(\cI)^{4ht} \Norm{w(\cI)^2 I- w(\cI)^2\Sigma(w)}_F^{2ht} \leq \Paren{ e^h_t (h)^{ht} + (C\delta)^{ht} \kappa^h}^2 h^{2ht} (2Ch)^{2ht} \Biggr\}\mper
\]

\end{proof}

\subsection{Analysis of Large List Rounding}
\Pnote{Powers of $\alpha$ and $1/\alpha$ in this section might be off at various places. Great to go over those carefully.}\Anote{done.}

We start by analyzing ``idealized'' version of the rounding procedure that modifies the first step in our rounding algorithm by sampling the multiset $S$ of size $t$ conditioned on it  lying inside $\cI$. The algorithm is (of course) not aware of $\cI$ so this rounding  is not implementable. Nonetheless, it  paves the way to analyze our actual large  list  rounding  algorithm.

\begin{enumerate}
\item Pick $S \in {[\cI] \choose t}$ with probability proportional to ${n \choose S}\pE_{\tzeta}[ \Pi_{i \in S} w_i]$.
\item Reweight $\tzeta$ by the polynomial $\Pi_{i \in S} w_i$ to obtain $\tzeta'$.
\item Output $\pE_{\tzeta'}[ \mu(w)], \pE_{\tzeta'}[ \Sigma(w)]$.
\end{enumerate}

For the remainder of the section it suffices to set the parameters as follows: $\delta = \alpha^2/2C$, $t = \log \kappa$.
The following lemma implies that the conditioned on an event that occurs with probability at least $\alpha^{-t}$, the first step of our rounding procedure produces a sample distributed according to the distribution used in the above idealized rounding procedure.


\begin{lemma}\label{lem:high-entropy-sample-in-intersection}
Let $\tzeta$ be a pseudo-distribution consistent with $\cA$ and minimizing $\Norm{\pE_{\tzeta} w}_2^2$. Then, $\pE_{\tzeta} w(\cI)^{4st+4s} \geq \alpha^{4st+4s}$ and consequently, with probability at least $\alpha^{-4st-4s}$, $S$ chosen according to our actual sampling procedure satisfies $S \subseteq \{i \mid y_i= y_i\}$.
\end{lemma}

\begin{proof}
Since $\tzeta$ minimizes $\Norm{\pE_{\tzeta} w}_2^2$, from Lemma~\ref{lem:high-entropy-intersection-original}, we know that $\pE_{\tzeta} w(\cI) \geq \alpha$. By Hölder's inequality for pseudo-expectations, $\pE_{\tzeta} w(\cI)^{4st+4s} \geq \alpha^{4st+4s}$. %This   Finally, observe that $\alpha^{4st+4s} \leq \pE_{\tzeta} \Paren{\frac{1}{\alpha n}  w_i}^{4st+4s} = \pE_{\tzeta} \Paren{\frac{1}{\alpha n}  w_i \1(S\subseteq \{i \mid y_i = y_i\})}^3 = \frac{1}{\alpha n}^3 \sum_{S \subseteq [n]} {n \choose S} \1(S \subseteq \{ i \mid y_i = y_i\}) \pE_{\tzeta} \Pi_{i \in S} w_i = \sum_{S \subseteq [n]} \Pr_{S \text{ is chosen }}  \1(S \subseteq \{ i \mid y_i = y_i\})$. This completes the proof.
\end{proof}

We now analyze this idealized rounding procedure.

\begin{lemma}[Mean Closeness of the Rounded Parameters] \label{lem:analysis-mean-rounding}
With probability at least $0.999$ over the draw of $S$ in the procedure above, $\hat{\mu} = \pE_{\tzeta'}[ \mu(w)]$ satisfies:

\[
\Norm{\hat{\mu}-\mu_*}_2^{2} \leq O(s^{2} \alpha^{-2} \alpha^{-2/s})\mper
\]
\end{lemma}

\begin{proof}
In order to simplify notation, we assume that $\Sigma_*^{-1/2} = I$ in the argument below, which holds w.l.o.g.
Since $\tzeta$ is consistent with $\cA$, applying Lemma~\ref{lem:mean-closeness-main} and taking pseudo-expectation with respect to $\tzeta$ yields:
\begin{equation}
\label{eqn:rhs_mean_closeness}
\pE_{\tzeta} w(\cI)^{4st+4s} \Norm{\mu_*-\mu(w)}_2^{4s} \leq \pE[w(\cI)^{2st+4s-2} \Paren{2Cs}^{2s} \Paren{(w(\cI)^{2st} + (2C\delta)^{2st}\kappa^s + e_t (s/\delta)^s}^2] \mper
\end{equation}

Dividing both sides by $\pE[w(\cI)^{4st+4s}]$ gives:
\begin{multline}
\frac{1}{\pE[w(\cI)^{4st+4s}]} \pE_{\tzeta} w(\cI)^{4st+4s} \Norm{\mu_*-\mu(w)}_2^{4s} \\\leq \frac{1}{\pE[w(\cI)^{4st+4s}]}  \pE[w(\cI)^{2st+4s-2} \Paren{2Cs}^{2s} \Paren{(w(\cI)^{2st} + (2C\delta)^{2st}\kappa^{2s} + e_t^2 (s/\delta)^{2s}}] \mper
\end{multline}

Let's analyze the RHS of the above inequality.
By applying Hölder's inequality for pseudo-distributions on $\pE[w(\cI)] \geq \alpha$ (from Lemma~\ref{lem:high-entropy-intersection-original}),  $\pE[w(\cI)^{q}] \geq \alpha^{q}$ for every $q$.  Combining with $\delta = \alpha/2$, $\pE[e_t^2 w(\cI)^{2st+4s-2}] \leq 2 \pE[w(\cI)^{4st-4}]$. Thus, the third term on the RHS is upper bounded by $O(1) \cdot \frac{1}{\pE[w(\cI)^{4st+4s}]} \cdot (s^{2}/\delta)^{2s} \pE[w(\cI)^{4st-4}]$. And the second term by $O(1) \cdot  \frac{1}{\pE[w(\cI)^{4st+4s}]} (C\delta)^{2st} \kappa^{2s} s^{2s} \pE[w(\cI)^{2st+4s-2}]$. Finally, the first term is upper bounded by $O(1) \cdot \frac{1}{\pE[w(\cI)^{4st+4s}]} s^{2s} \pE[w(\cI)^{4st+4s-2}]$.

By Hölder's inequality for pseudo-distributions, we can bound each term above as follows:
\[\pE[w(\cI)^{2st}]\leq \pE[w(\cI)^{4st+4s}]^{2st/(4st+4s)}\]
and
\[\pE[w(\cI)^{2st+4s-2}] \leq \pE[w(\cI)^{4st+4s}]^{(2st+4s-2)/(4st+4s)}
\]
and \[
\pE[w(\cI)^{4st+4s-4}] \leq  \pE[w(\cI)^{4st+4s}]^{(4st+4s-4)/(4st+4s)}
\]
Combined with $\pE[w(\cI)^{4st+4s}] \geq \alpha^{4st+4s}$ and using that $\delta < \alpha^2/2C$ yields that the RHS of \eqref{eqn:rhs_mean_closeness} is bounded above by $O(1) s^{2s} \alpha^{-4s} \alpha^{-4} + s^{2s} (C\delta/\alpha^2)^{2st} \kappa^s \alpha^{-2} + O(1) s^{2s} \alpha^{-2}  \leq O(s^{2s}) 2^{-2st}  \kappa^s \alpha^{-4s}$.
Using that $t > \log \kappa$ yields an upper bound of $O(s^{4s} \alpha^{-4s})$ on the RHS above yielding:
\begin{equation}
\frac{1}{\pE[w(\cI)^{4st+4s}]} \pE_{\tzeta} w(\cI)^{4st+4s} \Norm{\mu_*-\mu(w)}_2^{4s} \leq O(s^{4s} \alpha^{-4s-4}) \mper
\end{equation}
Expanding out $w(\cI)^{4st+4s}$, noting that $\cA \sststile{6}{w} \Set{{w}_S^2 = w_S}$ for every $S$ and using Cauchy-Schwarz inequality for pseudo-distributions yields:
\begin{equation}
\frac{1}{\pE[w(\cI)^{4st+4s}]}  \pE_{\tzeta} \sum_{S \subseteq [n], |S| = 4st+4s} {n \choose S}  \Norm{\pE_{\tzeta} w_S \mu_*-\pE_{\tzeta'}w_S\mu(w)}_2^{4s} \leq O(s^{4s} \alpha^{-4s-4})
\end{equation}
% Noting that $\pE_{\tzeta'} \mu = \frac{\pE_{\tzeta} [w_S \mu]}{\pE_{\tzeta}[w_S]}$ gives:
% \begin{equation}
% \pE_{\tzeta} \frac{1}{\pE[w'(X)^{3}]} \sum_{S \subseteq [n], |S| = 3} {n \choose S} \pE_{\tzeta}[w'_S] \Norm{\pE_{\tzeta'}\mu-\mu_*}_2^{2} \leq \frac{1}{\pE[w'(X)^{3}]} \Paren{2Cs} O( 2C\delta \kappa + 2(s/\delta)) \Biggr\}
% %  \leq \Paren{ 2C\sqrt{s}}^{4s}  w'(X)^{4s}  \Paren{ 1 + (s/\delta)^{2s} + (2C\delta)^{2t} \kappa^s }^2\Biggr\}
% \end{equation}
% \begin{equation}
% \frac{1}{\pE[w'(X)^{4st+4s}]}  \pE_{\tzeta} \sum_{S \subseteq [n], |S| = 4st+4s} {n \choose S}  \pE_{\tzeta} w'_S \Norm{ \mu_*-\hat{\mu}}_2^{4s} \leq O(s^{4s} \alpha^{-8}) \Biggr\}
% \end{equation}
The LHS above is the expectation of the distance of the rounded mean to the true mean over the draw of a random $S$ according to the distribution in the first step of the idealized rounding procedure above. %Further, from Lemma~\ref{lem:high-entropy-sample-in-intersection} and Hölder's inequality for pseudo-distributions, $\pE[w(\cI)^{3}] \geq\pE[w(\cI)]^3 \geq \frac{1}{\alpha^3}$.
Thus, we have:
\[
\E_{S} \Norm{\pE_{\tzeta'}\mu-\mu_*}_2^{4s} \leq O(s^{4s} \alpha^{-4s-4}) \mcom
\]
where the expectation on the LHS is with respect to the random draw of set $S$ in the idealized rounding procedure above.
By Markov's inequality, with probability at least $0.999$ over the draw of the set $S$ in the idealized rounding procedure above,
\[
\Norm{\pE_{\tzeta'}\mu-\mu_*}_2^{4s} \leq O(s^{4s} \alpha^{-4s-4})\mper
\]
Taking $2s$-th roots on both sides yields:
\[
\Norm{\pE_{\tzeta'}\mu-\mu_*}_2^{2} \leq O(s^{2} \alpha^{-2} \alpha^{-2/s})\mper
\]
\end{proof}



Next, we analyze $\Sigma$ of the idealized rounding procedure above and prove that it is close to $\Sigma_*$ in spectral distance $\Sigma_*$.

\begin{lemma}[Spectral Closeness of Rounded Parameters] \label{lem:analysis-spectral-large-list-rounding}
With probability at least $0.99$ over the draw of $S$ from the idealized sampling procedure, $\hat{\Sigma} = \pE_{\tzeta'}[ \Sigma(w)]$ satisfies:
\[
\Sigma_*^{-1/2} \hat{\Sigma} \Sigma_*^{-1/2} \succeq \Omega\Paren{\frac{\alpha}{s}}^2 \alpha^{2/s} I \mper
\]
\end{lemma}

\begin{proof}

 We start with the following conclusion of the spectral distance bound (Lemma~\ref{lem:spectral-distance-LDC}):
\[
\cA \sststile{4st}{\Pi,w} \Set{ \Norm{\Pi(w)\Sigma_*^{-1/2} v}_2^{2s} \geq \Paren{w(\cI)^2-C\delta)} \Paren{\frac{\delta}{s}}^{2s} \Norm{v}_2^{2s} }\mper
\]

Multiplying by $w(\cI)^{4st+4s}$ on both sides yields:
\[
\cA \sststile{4st}{\Pi,w} \Set{ w(\cI)^{4st+4s} \Norm{\Pi(w)\Sigma_*^{-1/2} v}_2^{2s} \geq w(\cI)^{4st+4s} \Paren{w(\cI)^2-C\delta)} \Paren{\frac{\delta}{s}}^{2s} \Norm{v}_2^{2s} }\mper
\]

Taking pseudo-expectations and dividing by $\pE[w(\cI)^{4st+4s}]$ on both sides yields:

\[
 \frac{1}{\pE[ w(\cI)^{4st+4s}]}\pE\left[ w(\cI)^{4st+4s} \Norm{\Pi(w)\Sigma_*^{-1/2} v}_2^{2s}\right] \geq \frac{1}{\pE[ w(\cI)^{4st+4s}]} \pE\left[w(\cI)^{4st+4s+2}-C\delta w(\cI)^{4st+4s}\right] \Paren{\frac{\delta}{s}}^{2s} \Norm{v}_2^{2s} \mper
\]

Applying Hölder's inequality for pseudo-expectations and invoking Lemma~\ref{lem:high-entropy-intersection-original} as in the proof of Lemma~\ref{lem:analysis-mean-rounding} yields:

\[
\frac{1}{\pE[ w(\cI)^{4st+4s}]}\pE\left[ w(\cI)^{4st+4s} \Norm{\Pi(w)\Sigma_*^{-1/2} v}_2^{2s}\right] \geq \alpha^{2}\left(1-C\delta\right) \Paren{\frac{\delta}{s}}^{2s} \Norm{v}_2^{2s} \mper
\]
Reasoning as in the proof of Lemma~\ref{lem:analysis-mean-rounding}, this yields:
\[
\E_{S} \Norm{ \Sigma_*^{-1/2} \pE_{\tzeta'}[\Sigma(w)]\Sigma_*^{-1/2} v}_2^{s}] \geq \alpha^{2}\left(1-C\delta\right) \Paren{\frac{\delta}{s}}^{2s} \Norm{v}_2^{2s} \mper
\]
Using Jensen's inequality for expectations, this implies:
\[
\E_{S}  v^{\top} \Sigma_*^{-1/2} \pE_{\tzeta'} [\Sigma(w)]\Sigma_*^{-1/2} v \geq \Paren{\frac{\delta}{s}}^2 \alpha^{2/s}\left(1-C\delta\right)^{1/s} \Norm{v}_2^{2} \mper
\]
The lemma now follows from an application of Markov's inequality as in the proof of Lemma~\ref{lem:analysis-mean-rounding}.

% Employing an argument similar to the one in the proof of Lemma~\ref{lem:analysis-mean-rounding} yields

\end{proof}

\begin{lemma}[Relative Frobenius Closeness of Rounded Parameters] \label{lem:analysis-frobenius-large-list-rounding}
With probability at least $0.99$ over the draw of $S$ from the idealized sampling procedure, $\hat{\Sigma} = \pE_{\tzeta'}[ \Sigma(w)]$ satisfies:
\[
\Norm{\Sigma_*^{-1/2}\hat{\Sigma}\Sigma_*^{-1/2}-I}_F^{2} \leq O(h^{4} \alpha^{-4} \alpha^{-6/h}) \mper
\]
\end{lemma}

\begin{proof}
For ease of notation, we will assume that $\Sigma_* = I$ in the analysis below.
Since $\tzeta$ is consistent with $\cA$, applying Lemma~\ref{lem:rel-frob-close-main} and taking pseudo-expectation with respect to $\tzeta$ yields:
\begin{equation}
\pE_{\tzeta} [w(\cI)^{4ht+4h} \Norm{ I- \Sigma(w)}_F^{2ht}] \leq O(1) \pE[\Paren{ e_t^2 (h)^{2h} + (C\delta)^{2ht} \kappa^{2h}} h^{2ht}) w(\cI)^{4ht-4h}] \mcom
\end{equation}
where $e_t = \Paren{\sum_{i = 0}^{ht-1} w(\cI)^{2ht-2-2i} (2C\delta)^{2i}}$.
Dividing throughout by $\pE[w(\cI)^{4ht+4h}]$ to obtain:
\begin{multline}
 \frac{1}{\pE[w(\cI)^{4ht+4h}]} \pE_{\tzeta} [w(\cI)^{4ht+4h} \Norm{ I- \Sigma(w)}_F^{2h}] \\\leq O(1) \cdot \frac{1}{\pE[w(\cI)^{4ht+4h}]} \pE[\Paren{ e_t^2 (h/\delta)^{2ht} + (C\delta)^{2ht} \kappa^{2h}} h^{2h} w(\cI)^{4ht-4h}] \mcom \label{eq:main-eq-rel-frob-rounding}
\end{multline}

Invoking Lemma~\ref{lem:high-entropy-intersection-original}, $\pE[w(\cI)] \geq \alpha$. By Hölder's inequality for pseudo-distributions, $\pE[w(\cI)^{q}] \geq \alpha^{q}$ for every $q>1$. Combining with $\delta = \alpha/2$, $\pE[e_t^2 w(\cI)^{4ht-4h}] \leq 2 \pE[w(\cI)^{4ht-6}]$. Thus, the first term on the RHS is upper bounded by $O(1) \cdot \frac{1}{\pE[w(\cI)^{4ht+4h}]} \cdot (s^{2}/\delta)^{2h} \pE[w(\cI)^{4ht+4h-6}]$. And the second term by $O(1) \cdot \frac{1}{\pE[w(\cI)^{4ht+4h}]} (C\delta)^{2ht} \kappa^{2h} s^{2ht} \pE[w(\cI)^{4ht-4h}]$.

By Hölder's inequality for pseudo-distributions, $\pE[w(\cI)^{4h-4}]\leq \pE[w(\cI)^{4ht}]^{4h-4/4ht}$ and $\pE[w(\cI)^{4ht-6}] \leq \pE[w(\cI)^{4ht}]^{4ht-6/4ht}$. Combined with $\pE[w(\cI)^{4ht}] \geq \alpha^{4ht}$ and using that $\delta < \alpha/2C$ yields that the RHS of \eqref{eq:main-eq-rel-frob-rounding} is bounded above by $O(1) h^{4h} \alpha^{-4h} \alpha^{-6} + s^{2h} (C\delta/\alpha)^{2ht} \kappa^s \alpha^{-4} \leq O(h^{2h}) 2^{-2ht}  \kappa^s \alpha^{-4h-6}$.
Finally, using that $t > \log \kappa$ simplifies the above expression to be at most: $O(h^{4h} \alpha^{-4h} \alpha^{-6})$.
Thus, we have shown:

\begin{equation}
 \frac{1}{\pE[w(\cI)^{4ht+4h}]} \pE_{\tzeta} [w(\cI)^{4ht+4h} \Norm{ I- \Sigma(w)}_F^{2h}] \leq O(h^{4h} \alpha^{-4h} \alpha^{-6}) \mper \label{eq:main-eq-rel-frob-rounding-simplified}
\end{equation}




% Applying Hölder's inequality for pseudo-distributions, taking $1/s$-th powers on both sides yields and noting that $\pE[w'(X)$
% \begin{equation}
% \pE_{\tzeta} w'(X)^{4t+4} \Norm{ I- \Sigma(w)}_F^{2} \leq O(s^4 \alpha^{-4} \alpha^{-12/s})\mper
% \end{equation}

Expanding out $w(\cI)^{4ht+4h}$, noting that $\cA \sststile{2}{w} \Set{{w}_S^2 = w_S}$ for every $S$ and using Cauchy-Schwarz innequality for pseudo-distributions yields:

\begin{equation}
\frac{1}{\pE[w(\cI)^{4ht+4h}]} \pE_{\tzeta} \sum_{S \subseteq [n], |S| = 4ht+4h} {n \choose S}  \Norm{\pE_{\tzeta}[w_S \Sigma]-\pE_{\tzeta}[w_S] I}_F^{2h} \leq  O(h^{4h} \alpha^{-4h} \alpha^{-12})\mper
%  \leq \Paren{ 2C\sqrt{s}}^{4s}  w'(X)^{4s}  \Paren{ 1 + (s/\delta)^{2s} + (2C\delta)^{2t} \kappa^s }^2\Biggr\}
\end{equation}


% Dividing both sides by $\pE[w'(X)^{3}]$ and rearrangig yields:
% \begin{equation}
% \pE_{\tzeta} \frac{1}{\pE[w'(X)^{3}]} \sum_{S \subseteq [n], |S| = 3} {n \choose S} \pE_{\tzeta}[w'_S] \Norm{\frac{\pE_{\tzeta} [w'_S \Sigma]}{\pE_{\tzeta} w'_S]}-I}_2^{2} \leq  \frac{1}{\pE[w'(X)^{3}]} O(s^3/\delta + s^2 \delta \kappa)\mper
% \end{equation}

Noting that $\pE_{\tzeta'} \Sigma = \frac{\pE_{\tzeta} [w_S \Sigma]}{\pE_{\tzeta} w_S]}$ gives:
\begin{equation}
\frac{1}{\pE[w(X)^{4ht+4h}]} \pE_{\tzeta} \sum_{S \subseteq [n], |S| = 4ht+4h} {n \choose S} \Norm{\pE_{\tzeta'} \Sigma-I}_F^{2h} \leq O(h^{4h} \alpha^{-4h} \alpha^{-6}) \Biggr\}
%  \leq \Paren{ 2C\sqrt{s}}^{4s}  w'(X)^{4s}  \Paren{ 1 + (s/\delta)^{2s} + (2C\delta)^{2t} \kappa^s }^2\Biggr\}
\end{equation}

The LHS above is the expectation of the relative Frobenius distance of the rounded covariance to the covariance mean over the draw of a random $S$ according to the distribution in the first step of the idealized rounding procedure above. %Further, from Lemma~\ref{lem:high-entropy-sample-in-intersection} and Hölder's inequality for pseudo-distributions, $\pE[w'(X)^{4st+4s}] \geq\pE[w'(X)]^{4st+4s} \geq \frac{1}{\alpha^6}$.

Thus, we have:
\[
\E_{S} \Norm{\pE_{\tzeta'}\Sigma-I}_F^{2h} \leq O(h^{4h} \alpha^{-4h} \alpha^{-6}) \mcom
\]
where the expectation on the LHS is with respect to the random draw of set $S$ in the idealized rounding procedure above.

By Markov's inequality, with probability at least $0.999$ over the draw of the set $S$ in the idealized rounding procedure above,
\[
\Norm{\pE_{\tzeta'}\Sigma-I}_F^{2h} \leq O(h^{4h} \alpha^{-4h} \alpha^{-12}) \mper
\]
Taking $h$-th roots on both sides:
\[
\Norm{\pE_{\tzeta'}\Sigma-I}_F^{2} \leq O(h^{4} \alpha^{-4} \alpha^{-6/h}) \mper
\]
\end{proof}

\begin{proof}[Proof of Lemma~\ref{lem:main-analysis-large-list-rounding}]
The Lemma follows immediately by combining the three results above.
\end{proof}

\input{content/pruning}


==> content/old/TVvsParam.tex <==
%!TEX root = ../main.tex
\section{TV Distance vs Parameter Distance: Real Life Version}
\Pnote{This section serves a dual purpose. It should give a "real life" version of the SoS proof that follows. The proof should mirror the SoS proof as much  as possible in order  to aid make the SoS proof comprehensible. It will also give us our pruning algorithm later.}

\begin{definition}[TV Distance]
Let $D,D'$ be two distributions on $\R^d$. The total variation (TV) distance between $D,D'$ is defined as $\frac{1}{2} \int_{-\infty}^{\infty} |D(x)-D'(x)| dx$. 
\end{definition}


% \begin{lemma}[Intersection vs TV Distance]
% Let $D,D'$ be distributions on $\R^d$ such that $\int_{-\infty}^{\infty} D(x)D'(x) dx  \geq \epsilon$. Then, $\Norm{D-D'}^2_{TV} \leq 1-\epsilon$.
% \end{lemma}

% \begin{proof}
% Note that $1 \geq \int_{-\infty}^{\infty} D(x)^2 dx,\int_{-\infty}^{\infty} D'(x)^2 dx$. 
% We have:
% \begin{align*}
% \int_{-\infty}^{\infty} \Paren{D(x)-D'(x)}^2dx \leq \Paren{\int_{-\infty}^{\infty} \Abs{D(x)-D'(x)}dx}^2\\
% &\leq 4\Norm{D-D'}_{TV}^2\mper
% \end{align*}
% Now, $\int_{-\infty}^{\infty} \Paren{D(x)-D'(x)}^2dx = \int_{-\infty}^{\infty} D(x)^2 dx +\int_{-\infty}^{\infty} D'(x)^2 dx - 2 \int_{-\infty}^{\infty} D(x)D'(x)dx$. 
% Thus,  

% By Cauchy-Schwarz inequality, 
% \[
% \Paren{\frac{1}{2} \int_{\infty}^{\infty} |D(x)-D(x')| dx}^2 \leq \frac{1}{4} \int_{\infty}^{\infty} |D(x)-D(x')|^2 dx \leq 1/2-\frac{1}{2}\int_{-\infty}^{\infty} D(x) D'(x) \leq \frac{1}{2}-\alpha/2 \mper
% \]

% \end{proof}

\begin{theorem}[TV Distance vs Parameter Distance]
Let $D,D'$ be two distributions on $\R^d$ with means $\mu_1,\Sigma_1$ and $\mu_2,\Sigma_2$ satisfying $\Norm{D-D'}_{TV}\leq 1-\epsilon$. Suppose both $D,D'$ are $4$-certifiably $C$-subgaussian and $\delta$-anti-concentrated.  Then, $\Norm{\Sigma_1^{-1/2} \mu_1 - \Sigma_2^{-1/2} \mu_2}_2 +\Norm{\Sigma_1^{-1/2}\Sigma_2\Sigma_1^{-1/2}-I}_F +\Norm{\Sigma_2^{-1/2}\Sigma_1\Sigma_2^{-1/2}-I}_F \leq \poly(1/\epsilon)$. \label{thm:real-life-TV-to-parameter}
\end{theorem}

\begin{theorem}[Tightness of Theorem~\ref{thm:real-life-TV-to-parameter}]
There exist $4$-certifiably $C$-subgaussian and $\delta$-anti-concentrated $D,D'$ with means $\mu_1,\Sigma_1$ and $\mu_2,\Sigma_2$ respectively such that $\Norm{\Sigma_1^{-1/2} \mu_1 - \Sigma_2^{-1/2} \mu_2}_2 +\Norm{\Sigma_1^{-1/2}\Sigma_2\Sigma_1^{-1/2}-I}_F +\Norm{\Sigma_2^{-1/2}\Sigma_1\Sigma_2^{-1/2}-I}_F = \Omega(1/\epsilon)$.
\end{theorem}





==> content/old/TVvsParamapp.tex <==
%!TEX root = ../main.tex

\section{Total Variation vs Parameter Distance for Gaussian Distributions} \label{Sec:tv-vs-param-gaussian}
\begin{lemma}[Parameter Closeness Implies TV Closeness for Gaussian Base Model] \label{lem:tv-vs-param-for-gaussians}
Fix $\eta > 0$ and let $\mu,\mu'$ and $\Sigma, \Sigma' \succ 0$ satisfy:
\begin{enumerate}
\item \textbf{Mean Closeness: } $\Norm{\Sigma^{-1/2} \Paren{\mu - \mu'}}^2_2 \leq 1/\eta$.
\item \textbf{Spectral Closeness: } $\Norm{\Sigma^{-1/2} \Sigma' \Sigma^{-1/2}}_2, \Norm{{\Sigma'}^{-1/2} \Sigma {\Sigma'}^{-1/2}}_2 \leq \frac{1}{\eta}$. %and $  v^{\top} {\Sigma'}^{-1/2} \Sigma {\Sigma'}^{-1/2}v \leq \frac{ \Delta}{\eta} \norm{v}_2^2 $.
\item \textbf{Relative Frobenius Closeness: } $\Norm{ \Sigma^{-1/2} \Sigma' \Sigma^{-1/2} -I}_F^2 \leq \frac{1}{\eta} \cdot \Norm{ \Sigma^{-1/2} \Sigma'^{1/2}}^2_2$.
\end{enumerate}
Then, $\dtv(\cN(\mu,\Sigma), \cN(0,\Sigma')) \leq 1- \exp(-O(1/\eta^2 \log 1/\eta))$.
\end{lemma}


\begin{proof}[Proof of Lemma~\ref{lem:tv-vs-param-for-gaussians}] 

We will work with the distributions after applying the transformation $x \rightarrow \Sigma^{-1/2}x$ to the associated random variables. Since $\dtv$ is invariant under affine transformations, this is WLOG. The transformation produces distributions $\cN(\mu_1, I)$ and $\cN(\Sigma^{-1/2} \mu', \Sigma^{-1/2} \Sigma' \Sigma^{-1/2})$ for $\mu_1 = \Sigma^{-1/2} \mu$, $\mu_2 =\Sigma^{-1/2} \mu' $ and $\Sigma_2 = \Sigma^{-1/2} \Sigma' \Sigma^{-1/2}$.

We will first bound the Hellinger distance between the two distributions above. Recall that $h= h(\cN(\Sigma^{-1/2} \mu, I),\cN(\Sigma^{-1/2} \mu', \Sigma^{-1/2} \Sigma' \Sigma^{-1/2}))$ satisfies:
\[
h(\cN(\mu_1,I), \cN(\mu_2,\Sigma_2))^2 =1 - \frac{\det(\Sigma_2)^{1/4}}{\det\left( \frac{I+\Sigma_2}{2}\right)^{\frac{1}{2}}} \exp\left(-\frac{1}{8} (\mu_1 - \mu_2)^{\top}\Paren{\frac{I + \Sigma_2}{2}}^{-1} (\mu_1 - \mu_2) \right)\mper
\]
We will estimate the RHS of the expression above to bound the Hellinger distance.

From the mean closeness condition, we have:

\[
\iprod{\mu_1-\mu_2,v}= \langle \mu - \mu', \Sigma^{-1/2} v \rangle \leq \sqrt{\log 1/\eta} \sqrt{ v^{\top} (I + \Sigma_2) v } \mper
\]

Plugging in $v = \Paren{\frac{I + \Sigma_2}{2}}^{-1} (\mu_1 - \mu_2)$ gives:
\[
\iprod{\mu_1-\mu_2,\frac{I + \Sigma_2}{2}^{-1} (\mu_1 - \mu_2)} \leq  2/\eta \sqrt{ v^{\top} \Paren{\frac{I + \Sigma_2}{2}}^{-1} v } \mcom
\]
or, \[ \iprod{\mu_1-\mu_2,\Paren{\frac{I + \Sigma_2}{2}}^{-1} (\mu_1 - \mu_2)} \leq 4 1/\eta^2  \mper\]

And thus,
\[
\exp\left(-\frac{1}{8} (\mu_1 - \mu_2)^{\top} \Paren{ \frac{I + \Sigma_2}{2}}^{-1} (\mu_1 - \mu_2) \right) \geq \exp{\Paren{-1/2\eta^2}}\mper
\]

Thus, we have:
\[
h \leq 1- \frac{\det(\Sigma_2)^{\frac{1}{4}}}{\det \Paren{ \frac{\II+ \Sigma_2}{2} }^{1/2}} \exp{\Paren{-1/2\eta^2}}\mper
\]

Let $\lambda_1 \geq \lambda_2 \geq \cdots \lambda_d$ be eigenvalues of $\Sigma_2$.
From the spectral closeness condition, observe that each $\frac{1}{\eta} \geq \lambda_1 \geq \cdots \lambda_d \geq \eta$.

Then,
\[
\frac{\det(\Sigma_2)^{\frac{1}{4}}}{\det \Paren{ \frac{\II+ \Sigma_2}{2} }^{1/2}} = \frac{\Pi_{i \leq d} \lambda_i^{1/4}} { \Pi_{i \leq d} \Paren{\frac{1+\lambda_i}{2}}^{1/2}}\mper
\]
Thus,
\begin{equation}
\log(1/(1-h)) \leq \frac{1}{2} \log (1/\eta) + \frac{1}{2} \sum_{i\in [d]}\log\left(\frac{1+\lambda_i}{2\sqrt{\lambda_i}}\right)\mper \label{eq:hellinger-bound}
\end{equation}

We break the second term in the RHS above based on the magnitude of the eigenvalues $\lambda_i$s.
Let's first bound the contribution to this term coming from eigenvalues $\lambda_i \geq 1.5$ - let's call these the \emph{large} eigenvalues of $\Sigma_2$.

Next, observe that the Relative Frobenius Closeness condition gives us that $\|\II - \Sigma_2 \|^2_F \leq (1/\eta^2)$. Thus, $\sum_{i \in [d]}(1- \lambda_i)^2 = \|\II - \Sigma_2 \|^2_F \leq (1/\eta^2)$, the number of large eigenvalues is at most $4/\eta^2$. Further, for every large eigenvalue $\lambda_i$, $1+\lambda_i \leq 2\lambda_i$. Thus,

\begin{equation*}
\sum_{i: \lambda_i \text{ is large }} \log\left(\frac{1+\lambda_i}{2\sqrt{\lambda_i}}\right) \leq \sum_{i\in \cE} \log\left(\sqrt{\lambda_i} \right) \leq \frac{2}{\eta}\cdot \log(1/\eta)
\end{equation*}
where the last step uses that $\lambda_i \leq 1/\eta$.

Let's now consider all the remaining \emph{small} eigenvalues that satisfy $\eta \leq\lambda_i < 1.5$. Then, we can write $\lambda_i = 1+\beta_i$ such that $-(1-\eta)\leq \beta_i \leq 0.5$. Then, we have
\begin{equation*}
\begin{split}
\sum_{i:\lambda_i \leq 1.5} \log\left(\frac{1+\lambda_i}{2}\right) + \frac{1}{2}\log\left(\frac{1}{\lambda_i}\right) &= \sum_{i \in \cE'} \log\left(1+\frac{\beta_i}{2}\right) - \frac{1}{2}\log\left(1+\beta_i\right) \\
&\leq \sum_{i:\lambda_i \leq 1.5} \frac{\beta_i}{2} - \frac{\beta_i}{2} + \frac{\beta_i^2}{4}\\
& = \sum_{i:\lambda_i \leq 1.5} \frac{(1-\lambda_i)^2}{4} \leq \frac{1}{4\eta^2}
\end{split}
\end{equation*}
using the bound $\sum_{i} (1-\lambda_i)^2 \leq \frac{1}{\eta^2}$ in the last inequality.
Plugging this estimate back in \eqref{eq:hellinger-bound} yields $h \geq 1- \exp (-O(1/\eta^2 \log (1/\eta))$.

To finish the proof, we observe that $\dtv(p,q) \leq h(p,q) \sqrt{2-h(p,q)} \leq  1-\exp (-O(1/\eta^2 \log (1/\eta))$.

% Therefore, we can conclude $\sum_{i\in [d]}\log\left(\frac{1+\lambda_i}{2\sqrt{\lambda_i}}\right) \leq O(\frac{\log(1/\eta)}{\eta})$, and thus $\frac{\det( \Sigma_2)^{\frac{1}{2}}}{\det\left( (\II+ \Sigma_2)/2\right)} \geq \exp(-c\log(1/\eta)/\eta)$, for a fixed constant $c$.
\end{proof}



\section{Typical Samples are Good with High Probability}
\label{sec:feasibility}

\begin{proof}[Proof of Lemma~\ref{lem:typical-samples-good}] 
We begin with the empirical mean condition. 
For any fixed $\ell$, $C_{\ell}$ contains samples from a $1$-Sub-gaussian distributions and thus it follows from Fact \ref{fact:empirical_mean} that with probability at least $1-(1/\delta)$, 
\begin{equation*}
\Norm{\Sigma^{-1/2}_{\ell} ( \hat{\mu}_{\ell}  - \mu_{\ell})}_2 \leq \Norm{\Sigma^{-1/2}_{\ell} } \left( \sqrt{\frac{ k \trace{\Sigma_{\ell}} }{n}} + \sqrt{\frac{\|\Sigma_{\ell}\|_2 \log(1/\delta) k}{n}} \right) \leq \sqrt{\frac{kd}{n}} + \sqrt{\frac{k \log(1/\delta)}{n}}
\end{equation*}
%\Anote{It actually does not follow from the Hsu et al paper. This is result is somehow hard to find. I can prove it for Sub-Gaussians using Hoeffding and union bound on each coordinate. I stated it as a fact for now.}
Since $n_0= \Omega( (k\log(k) + kd)/\eta^2 )$, we can union bound over failure events for all  $\ell \in [k]$ and thus with probability at least $1-1/\poly(k)$, for all $\ell \in [k]$, $\Norm{\Sigma^{-1/2}_{\ell} ( \hat{\mu}_{\ell}  - \mu_{\ell}) }_2 \leq \eta$.

Similarly,
%\Pnote{please include a statement of the result you are using and then cite it - it's not desirable to use random results from other papers by direct references - it's also not clear what you are using and which distributions is it supposed to hold for} using standard results from Random Matrix Theory (see Proposition \cite{MR2827856-Rudelson10}), 
using Fact \ref{fact:empirical_cov} for i.i.d. samples from a $1$-Sub-gaussian distribution, it follows that for a fixed $\ell \in [k]$, with probability at least $1-1/d^{10}$,
\[
\left(1- c\sqrt{\frac{dk\log(k)}{n}}\right)\Sigma_{\ell} \preceq \hat{\Sigma}_{\ell} \preceq \left(1+c\sqrt{\frac{dk\log(k)}{n}}\right) \Sigma_{\ell}\] 
for fixed constants $c$. Union bounding over $\ell \in [k]$, and observing that $n_0 = \Omega(dk\log(k)/2^{1/s})$ with probability at least $1-1/d^{8}$ for all $\ell \in [k]$, 
\begin{equation}
\label{eqn:sample_complexity_cov}
\left(1-\frac{1}{2^{2s}}\right)\Sigma_{\ell} \preceq \hat{\Sigma}_{\ell} \preceq \left(1+\frac{1}{2^{2s}}\right) \Sigma_{\ell}
\end{equation}
for any $s>2$, 
which concludes the empirical covariance condition.
%\Pnote{I am not sure of this argument. Are you claiming the "difference of two samples is certifibaly anti-concentrated"? I don't know a  proof of this and I don't understand what your proof is here.} 
\noindent By definition of a ``nice'' distribution, we know that the points in $C_{\ell}$ are drawn i.i.d. from a $s$-certifiably $(C,\delta)$-anti-concentrated distribution denoted by $\cD(\mu_\ell, \Sigma_{\ell})$ and thus:
\begin{equation*}
\sststile{2s}{v} \Set{\E_{ x \sim \cD(\mu_\ell, \Sigma_{\ell})} \left[p^2_{\cD}\Paren{ \left\langle\Sigma^{-1/2}_{\ell} x,v \right\rangle}\right] \leq C\delta \norm{v}_2^{2s}} 
\end{equation*} 
Since $p_{\cD}$ is a degree-$s$ even polynomial, $p^2_{\cD}(z) = \sum_{i\in[s]}c_{i}z^{2i}$ and thus using the substitution rule, 

\begin{equation}
\label{eqn:cert_anit_conc_dist}
\sststile{2s}{v} \Set{\sum_{j \in [s]} c_i \left\langle \E_{ x \sim \cD(\mu_\ell, \Sigma_{\ell})} (\Sigma_{\ell}^{-1/2} x)^{\otimes 2j} , v^{\otimes 2j} \right\rangle \leq C\delta \norm{v}_2^{2s}} 
\end{equation} 
Further, observe that $(\hat{\Sigma}_{\ell}^{-1/2} x)^{\otimes 2j} = (\hat{\Sigma}_{\ell}^{-1/2} \Sigma_{\ell}^{1/2} \Sigma_{\ell}^{-1/2} x)^{\otimes 2j} \preceq \|\hat{\Sigma}_{\ell}^{-1/2} \Sigma_{\ell}^{1/2} \|^{2j}_2 (\Sigma_{\ell}^{-1/2} x)^{\otimes 2j} \preceq \left(2\right)^{j/s} (\Sigma_{\ell}^{-1/2} x)^{\otimes 2j}$, where the last inequality follows from \eqref{eqn:sample_complexity_cov}. Thus, we have

\begin{equation}
\begin{split}
\sststile{2s}{v} \Bigg\{   \E_{ x \sim \cD(\mu_\ell, \Sigma_{\ell})} \left[p^2_{\cD}\Paren{ \left\langle\hat{\Sigma}^{-1/2}_{\ell} x,v \right\rangle}\right] & =  \sum_{j \in [s]} c_i \left\langle \E_{ x \sim \cD(\mu_\ell, \Sigma_{\ell})} (\hat{\Sigma}^{-1/2}_{\ell} \Sigma_{\ell}^{1/2} \Sigma_{\ell}^{-1/2} x)^{\otimes 2j} , v^{\otimes 2j} \right\rangle  \\
& \leq  \sum_{j \in [s]} c_i \left(2\right)^{j/s}  \left\langle \E_{ x \sim \cD(\mu_\ell, \Sigma_{\ell})} (\Sigma_{\ell}^{-1/2} x)^{\otimes 2j} , v^{\otimes 2j} \right\rangle \\
& \leq 2 C \delta \|v\|^{2s}_2  \Bigg\}
\end{split}
\end{equation}
Therefore, it suffices to bound the operator norm above. 


Consider a permutation $\pi:[n/k]\to [n/k]$ that induces a pairing $x_i, x_{\pi[i]}$ of the samples from $\CC_{\ell}$. Then, observe if $i \neq \pi[i]$, $x_{i,\pi[i]} = \frac{x_i - x_{\pi[i]}}{\sqrt{2}}$ has mean $0$ covariance $\Sigma_{\ell}$. By the definition of a ``nice'' distribution we know that $x_{i,\pi[i]} $ is a $s$-certifiably $(C,\delta)$-anti-concentrated random variable. Let $\cU(0,\Sigma_{\ell})$ be the uniform distribution over the samples $x_{i,\pi[i]}$, for all $i\in[n/k]$. Since $n = \Omega( k(sd\log(d))^{s})$, it follows from Lemma \ref{lem:cert_anti_conc_sampling} that with probability at least $1-1/n^{10}$, 
\begin{equation}
\label{eqn:anti_conc_pairs}
\sststile{2s}{v} \Set{ \frac{k}{n}\sum_{i \neq \pi[i]} p^2_{\cD}\Paren{\left\langle\hat{\Sigma}^{-1/2}_{\ell} x_{i,\pi[i]},v\right\rangle} \leq C\delta \norm{v}_2^{2s}} 
\end{equation}
Repeating the aforementioned argument for $n/k$ cyclic shifts of $\pi$, and union bounding over the failure probability for each one, with probabillity at least $1- 1/n^{8}$, 

\begin{equation}
\label{eqn:anti_conc_sum}
\sststile{2s}{v} \Set{ \frac{k}{n}\sum_{x_i, x_j \in C_{\ell}: i\neq j} p^2_{\cD}\Paren{\left\langle\hat{\Sigma}^{-1/2}_{\ell} \left(\frac{x_i - x_j}{\sqrt{2}}\right) ,v\right\rangle} \leq \frac{C\delta n}{k} \norm{v}_2^{2s}} 
\end{equation}
Rearranging \eqref{eqn:anti_conc_sum} yields the claim.

Since for all $\ell \in [k]$, $\cD(\mu_\ell, \Sigma_{\ell})$ is also $h$-certifiably $C$-hypercontractive, 
\begin{equation}
\label{eqn:cert_hyper_contractivity_dist}
\sststile{2h}{Q} \Set{ \E_{x \sim \cD(\mu_\ell, \Sigma_{\ell})} \left[ \left( \left\langle\Sigma^{-1/2}_{\ell}x (\Sigma^{-1/2}_{\ell}x)^{\top},Q \right\rangle -\Tr[Q] \right)^{h} \right] \leq (Ch)^h \|Q\|^h_F }
\end{equation}
Observe,
\begin{equation*}
\begin{split}
\E_{x \sim \cD(\mu_\ell, \Sigma_{\ell})} \left[ \left( \left\langle (\hat{\Sigma}^{-1/2}x)^{\otimes 2} - \II ,Q \right\rangle  \right)^{h} \right] = \left\langle \E_{x \sim \cD(\mu_\ell, \Sigma_{\ell})}\left[\left( (\hat{\Sigma}^{-1/2}\Sigma^{1/2} \Sigma^{-1/2} x)^{\otimes 2} - \II \right)^{\otimes h}\right], Q^{\otimes h} \right\rangle
\end{split}
\end{equation*}
and $(\hat{\Sigma}^{-1/2}\Sigma^{1/2} \Sigma^{-1/2} x)^{\otimes 2} \preceq \|\hat{\Sigma}^{-1/2}\Sigma^{1/2}\|^2_2 (\Sigma^{-1/2} x)^{\otimes 2} \preceq \frac{3}{2} (\Sigma^{-1/2} x)^{\otimes 2}$, where the last inequality follows from \eqref{eqn:sample_complexity_cov}. Combining the above equation with \eqref{eqn:cert_hyper_contractivity_dist}, we have 
\begin{equation*}
\sststile{2h}{Q} \Set{ \E_{x \sim \cD(\mu_\ell, \Sigma_{\ell})} \left[ \left( \left\langle \hat{\Sigma}^{-1/2}_{\ell}x (\hat{\Sigma}^{-1/2}_{\ell}x)^{\top},Q \right\rangle -\Tr[Q] \right)^{h} \right] \leq (2Ch)^h \|Q\|^h_F }
\end{equation*}


Following the approach for anti-concentration, we can pair up the points from cluster $C_{\ell}$ using $\pi:[n/k]\to [n/k]$ and observe that it follows from the assumption that $\cD$ is ``nice'' that if $x_{i,\pi[i]} = \frac{x_i - x_{\pi[i]}}{\sqrt{2}}$ and $i \neq \pi[i]$, $\hat{\Sigma}_{\ell}^{-1/2}x_{i,\pi[i]}$ is drawn from a $h$-certifiable $2c$-hypercontractive distirbution. 
By Lemma \ref{lem:cert_hyper_sampling}, the uniform distribution on  $n = \Omega(k(hd)^{8h})$  such i.i.d. samples certifiably hypercontractive and thus with probability at least $1-1/n^{10}$,
\begin{equation}
\label{eqn:cert_hypercontractivity_pairs}
\sststile{2h}{Q} \Set{ \frac{k}{n} \sum_{i\neq \pi[i]} \left( \left\langle (\hat{\Sigma}^{-1/2}x_{i,\pi[i]}) (\hat{\Sigma}^{-1/2}x_{i, \pi[i]} )^{\top},Q \right\rangle -\Tr[Q] \right)^{h}  \leq (Ch)^h \|Q\|^h_F }
\end{equation}
Repeating the proof of \eqref{eqn:cert_hypercontractivity_pairs} for $n/k$ cyclic shifts of $\pi$, and union bounding over the failure probability for each one, with probabillity at least $1- 1/n^{8}$, 
\[
\sststile{2h}{Q} \Set{
\frac{k^2}{n^2} \sum_{x_i,x_j \in C_{\ell}}  \Paren{\left\langle \Paren{\hat{\Sigma}_{\ell}^{-\frac{1}{2}} \Paren{\frac{x_i -x_j}{\sqrt{2}}}} \Paren{ \hat{\Sigma}_{\ell}^{-\frac{1}{2}} \Paren{\frac{x_i -x_j}{\sqrt{2}}}}^{\top},Q \right\rangle - \Tr[Q]}^h
     \leq (Ch)^h\Norm{Q}_F^h}
  \]
This concludes the proof. 
\end{proof}

==> content/old/TechnicalLemmas.tex <==
%!TEX root = ../main.tex

\section{Key Technical Lemmas}

\subsection{Upper Bounds on Moments of Subsamples via Subgaussianity}

\begin{lemma}[Spectral Upper Bound on Subsamples]
Let $x_1, x_2, \ldots, x_n$ be $k$-certifiably $C$-subgaussian. Then, 
\[
\Set{w_i^2 = w_i \mid 1 \leq i \leq n} \sststile{}{} \Set{ \Paren{\frac{1}{n} \sum_{i = 1}^n w_i \iprod{x_i,v}^2}^{2t} \leq \Paren{\frac{1}{n} \sum_{i = 1}^n w_i}^{2t-2} \Paren{\frac{1}{n} \sum_{i = 1}^n \iprod{x_i,v}^2}^{2t}}\mper
\]
\end{lemma}

\begin{proof}
First, we have:
\[
\Set{w_i^2 = w_i \mid 1 \leq i \leq n} \sststile{}{} \Set{ \frac{1}{n} \sum_{i = 1}^n w_i \iprod{x_i,v}^2 = \frac{1}{n} \sum_{i = 1}^n w_i^{2t-2} \iprod{x_i,v}^2}\mper
\]
By Fact~\ref{fact:sos-holder} (sum-of-squares Hölder's inequality) %\FIXME{add statement to prelims},  
\[
\sststile{}{} \Set{ \Paren{\frac{1}{n} \sum_{i = 1}^n w_i^{2t-2} \iprod{x_i,v}^2}^{2t} \leq \Paren{\frac{1}{n} \sum_{i = 1}^n w_i^{2t}}^{2t-2} \Paren{ \frac{1}{n} \sum_{i = 1}^n \iprod{x_i,v}^{4t}}}\mper
\]
Using certifiable subgaussianity of $x_1,x_2, \ldots, x_n$, we have:
\[
\sststile{}{} \Set{ \frac{1}{n} \sum_{i = 1}^n \iprod{x_i,v}^{4t} \leq \paren{Ct}^t \Paren{\sum_{i = 1}^n \iprod{x_i,v}^{2}}^{2t}}\mper
\]
Combining the above results, we thus have:
\[
\Set{w_i^2 = w_i \mid 1 \leq i \leq n} \sststile{}{} \Set{ \Paren{\frac{1}{n} \sum_{i = 1}^n w_i \iprod{x_i,v}^2}^{2t} \leq \Paren{\frac{1}{n} \sum_{i = 1}^n w_i}^{2t-2} \Paren{\frac{1}{n} \sum_{i = 1}^n \iprod{x_i,v}^2}^{2t}}\mper\]

\end{proof}

\begin{lemma}[Frobenius Upper Bound on Subsamples]
Let $X' = x'_1, x'_2, \ldots, x'_n$ be $d$-dimensional vector valued indeterminates satisfying $\cA_4$
Let $\cA = \Set{ \frac{1}{n} \sum_{i = 1}^n x_i x_i^{\top} = I} \cup \Set{ \frac{1}{n} \sum_{i = 1}^n \iprod{x_i x_i^{\top} - I, P}^2  \leq C\Norm{P}_F^2}$.  
Then, 
% \begin{multline}
% \Set{w_i^2 = w_i \mid 1 \leq i \leq n} \cup \cA \sststile{6}{x_1,x_2,\ldots,x_n,w}\\ \Set{ \Norm{\frac{1}{n} \sum_{i = 1}^n w_i x_ix_i^{\top}- \Paren{\frac{1}{n} \sum_{i =1}^n w_i} I}_F^{4} \leq C \Paren{\frac{1}{n}\sum_{i = 1}^n w_i} \Norm{\frac{1}{n} \sum_{i = 1}^n w_i x_ix_i^{\top}- \Paren{\frac{1}{n} \sum_{i =1}^n w_i} I}_F^{2}}  \mper 
\[
\Set{w_i^2 = w_i \forall i}\cup \cA \sststile{6}{x_1,x_2,\ldots,x_n,w} \Set{ \Norm{\frac{1}{n} \sum_{i = 1}^n w_i x_ix_i^{\top}- \Paren{\frac{1}{n} \sum_{i =1}^n w_i} I}_F^{4} \leq C^2\Paren{\frac{1}{n} \sum_{i = 1}^n w_i}^2}\mper
\]
% \end{multline}
\label{lem:frob-upper-bound}
\end{lemma}

\begin{proof}

By sum-of-squares Hölder's inequality (Fact~\ref{fact:sos-holder}),  
\[
\sststile{6}{x_1,x_2,\ldots,x_n,w} \Set{ \Paren{\frac{1}{n} \sum_{i = 1}^n w_i \iprod{x_ix_i^{\top}-I,P}}^{2t} \leq \Paren{\frac{1}{n} \sum_{i = 1}^n w_i}^{2t-1} \Paren{ \frac{1}{n} \sum_{i = 1}^n \iprod{x_ix_i^{\top}-I,P}^{2t}}}\mper
\]
Next, 
\[
\Set{w_i^2 = w_i \forall i}\sststile{2}{w} \Set{ \frac{1}{n} \sum_{i =1}^n w_i^2 = \frac{1}{n} \sum_{i =1}^n w_i }\mper
\]
Applying certifiable hypercontractivity
\[
\cA \sststile{6}{x_1,x_2,\ldots,x_n} \Set{ \Paren{ \frac{1}{n} \sum_{i = 1}^n \Iprod{x_ix_i^{\top}-I,P}^{2}} \leq C\Norm{P}_F^2}\mcom
\]
and substituting $P = \frac{1}{n} \sum_{i = 1}^n w_i x_ix_i^{\top}- \Paren{\frac{1}{n} \sum_{i =1}^n w_i} I$ yields, 
\[
\Set{w_i^2 = w_i \forall i} \cup \cA \sststile{6}{x_1,x_2,\ldots,x_n,w} \Set{ \Norm{\frac{1}{n} \sum_{i = 1}^n w_i x_ix_i^{\top}- \Paren{\frac{1}{n} \sum_{i =1}^n w_i} I}_F^{4} \leq C\Paren{\frac{1}{n} \sum_{i = 1}^n w_i}\Norm{\frac{1}{n} \sum_{i = 1}^n w_i x_ix_i^{\top}- \Paren{\frac{1}{n} \sum_{i =1}^n w_i} I}_F^{2}}\mper
\]
Applying Lemma~\ref{lem:cancellation-sos} to the indeterminates $\Norm{\frac{1}{n} \sum_{i = 1}^n w_i x_ix_i^{\top}- \Paren{\frac{1}{n} \sum_{i =1}^n w_i} I}_F^{2}$ and $C\Paren{\frac{1}{n} \sum_{i = 1}^n w_i}$ respectively, we obtain:
\[
\Set{w_i^2 = w_i \forall i}\cup \cA \sststile{6}{x_1,x_2,\ldots,x_n,w} \Set{ \Norm{\frac{1}{n} \sum_{i = 1}^n w_i x_ix_i^{\top}- \Paren{\frac{1}{n} \sum_{i =1}^n w_i} I}_F^{4} \leq C^2\Paren{\frac{1}{n} \sum_{i = 1}^n w_i}^2}\mper
\]



\end{proof}

\subsection{Lower Bounds on Moments of Subsamples via Anti-Concentration}
\begin{lemma}[Spectral Lower Bound on Subsamples of Anti-Concentrated Distributions]
Let $X= \Set{x_1, x_2, \ldots, x_n} \subseteq \R^d$ be $2t$-certifiably $(\delta,C\delta)$-anti-concentrated with mean $0$ and covariance $I$.  
Then, 
\[
\Set{w_i^2 = w_i \forall i} \sststile{2t}{w,v} \Set{\frac{1}{n} \sum_{i = 1}^n w_i \norm{v}_2^{2t-2} \iprod{x_i,v}^2 \geq \delta^2 \norm{v}_2^{2t}  \Paren{\frac{1}{n} \sum_{i = 1}^n w_i - C\delta} }\mper
\] \label{lem:spectral-LB-constantx}
\end{lemma}

\begin{proof}
Since $X$ is $2t$-cerfiably $(\delta,C\delta)$-anti-concentrated, there is a univariate polynomial $p$ of degree $2t$ satisfying
\begin{enumerate}
\item $\sststile{2t}{v} \Set{\norm{v}_2^{2t-2} \iprod{x,v}^2 + \delta^2 p^2\paren{\iprod{x,v}} \geq \delta^2 \norm{v}_2^{2t}}$. 
\item $\sststile{2t}{v} \Set{\E_{x \sim D} p^2\paren{\iprod{x,v}} \leq C\delta  \norm{v}_2^{2t}}$.
\end{enumerate}

For every $1 \leq i \leq n$,  we have:
\begin{equation}
\Set{w_i^2 = w_i \forall i} \sststile{2t}{v} \Set{\norm{v}_2^{2t-2} \iprod{x_i,v}^2 + \delta^2 p^2\paren{\iprod{x_i,v}} \geq \delta^2 \norm{v}_2^{2t}}\mper
\end{equation}

Thus, 
\begin{equation}
\Set{w_i^2 = w_i \forall i} \sststile{2t}{v} \Set{\frac{1}{n}\sum_{i = 1}^n w_i \Paren{\norm{v}_2^{2t-2} \iprod{x,v}^2 + \delta^2 p^2\paren{\iprod{x,v}}} \geq \delta^2 \norm{v}_2^{2t} \Paren{\frac{1}{n} \sum_{i = 1}^n w_i}}\mper
\end{equation}

Rearranging yields:
\begin{equation}
\Set{w_i^2 = w_i \forall i} \sststile{2t}{v} \Set{\frac{1}{n}\sum_{i = 1}^n w_i \Paren{\norm{v}_2^{2t-2} \iprod{x,v}^2  \geq - \delta^2 \frac{1}{n}\sum_{i = 1}^n w_i p^2\paren{\iprod{x_i,v}}} + \delta^2 \norm{v}_2^{2t} \Paren{\frac{1}{n} \sum_{i = 1}^n w_i}}\mper
\end{equation}

Next, we use that $\Set{w_i^2 = w_i} \sststile{2}{w} \Set{w_i \leq 1} \cup \Set{0 \leq w_i}$ to conclude: 
\begin{equation}
\Set{w_i^2 = w_i \forall i} \sststile{2t}{v} \Set{\frac{1}{n}\sum_{i = 1}^n w_i  \delta^2 p^2\paren{\iprod{x_i,v}} \geq \delta^2 \frac{1}{n}\sum_{i = 1}^n  p^2\paren{\iprod{x_i,v}}}\mper
\end{equation}

Combining the above two observations with $\sststile{2t}{v} \Set{\E_{x \sim D} p^2\paren{\iprod{x,v} \leq C\delta \norm{v}_2^{2t}}}$, we have:
\begin{equation}
\Set{w_i^2 = w_i \forall i} \sststile{2t}{v} \Set{\frac{1}{n}\sum_{i = 1}^n w_i \norm{v}_2^{2t-2} \iprod{x,v}^2  \geq - C\delta^3 \norm{v}_2^{2t} + \delta^2 \norm{v}_2^{2t} \Paren{\frac{1}{n} \sum_{i = 1}^n w_i}}\mper
\end{equation}

This completes the proof.

\end{proof}

\subsection{Spectral Distance From TV Distance}

\begin{lemma}
Let $p$ be a univariate polynomial of degree $2t$ and let $\cA$ be the following set of polynomial constraints in the set of $d$-dimensional vector valued indeterminates $X = \Set{x_1,x_2, \ldots,x_n}$ and $d$ dimensional vector valued indeterminate $v$:
\begin{enumerate}
\item $ \Set{  \Paren{\frac{1}{n} \sum_{i = 1}^n \iprod{x_i,v}^2}^{t-1} \iprod{x_i,v}^2 + \delta^2 p^2\paren{\iprod{x_i,v}} \geq \delta^2 \Paren{\frac{1}{n} \sum_{i = 1}^n \iprod{x_i,v}^2}^{t}}$. 
\item $\Set{\frac{1}{n}\sum_{i =1}^n p^2\paren{\iprod{x_i,v}} \leq C\delta \norm{v}_2^{2t}}$.
\item $\Set{ \frac{1}{n} \sum_{i = 1}^n x_i x_i^{\top} = I}$.% \cup \Set{\frac{1}{n} \sum_{i=1}^n x_i = 0}$.
\end{enumerate}
% Let $\cB$ be the following set of polynomial constraints in a $d \times d$ matrix valued indeterminate $P$.
% \[
% \sststile{2}{P} \Set{\frac{1}{n} \Iprod{\Paren{x_ix_i^{\top} - I},P}^{2} \leq 4 \Norm{P}_{F}^{2}} \mper
% \]
Then, 
\[
\cA \cup \Set{w_i^2 = w_i \forall i\leq n} \sststile{2t}{x_1,x_2,\ldots,x_n,w} \Set{ I^{\otimes \paren{t-1}} \otimes \Paren{\frac{1}{n} \sum_{i = 1}^n w_i x_i x_i^{\top}} \succeq \delta^2 \Paren{\frac{1}{n} \sum_{i = 1}^n w_i - C\delta} I^{\otimes t}}
\]
\label{lem:spectral-vs-tv-general}
\end{lemma}

\begin{proof}
By definition of matrix SoS inequalities, the conclusion we desire is equivalent to:
\[
\cA \cup \Set{w_i^2 = w_i \forall i\leq n} \sststile{2t}{x_1,x_2,\ldots,x_n,w,v} \Set{ \norm{v}_2^{2t-2} \otimes \Paren{\frac{1}{n} \sum_{i = 1}^n w_i \iprod{x_i,v}^2} \succeq \delta^2 \Paren{\frac{1}{n} \sum_{i = 1}^n w_i - C\delta} \norm{v}_2^{2t}}\mper
\]
From here on, the proof is syntactically same as that of Lemma~\ref{lem:spectral-LB-constantx} except for the difference that $x_1,x_2,\ldots,x_n$ are indeterminates (as opposed to constants in the Lemma~\ref{lem:spectral-LB-constantx}) in this version so we rely on the constraint system $\cA$ to give us the constraints we need on $x_i$s rather than certifiable anti-concentration of $x_i$s. 

\subsection{Main Lemma: TV Distance vs Parameter Distance}

\Pnote{Split into multiple lemmas}

\begin{lemma}[Relative Frobenius Distance from TV Distance]
Let $X = \Set{x_1, x_2, \ldots, x_n} \subseteq \R^d$ be $2t$-certifiably $(\delta,C\delta)$-anti-concentrated (witnessed by a degree $2t$ polynomial $p$), $\frac{1}{n} \sum_{i = 1}^n x_i x_i^{\top} = I$ and $\frac{1}{n} \sum_{i = 1}^n \Paren{x'_i x_i^{\top} - I}\Paren{x'_i x_i^{\top} - I}^{\top} \preceq C I$ for some constant $C >0$.
Let $\cA$ be a set of polynomial constraints with indeterminates:
\begin{enumerate}
\item $w_1,w_2,\ldots,w_n$ - scalar valued indeterminates. 
\item $X' = \Set{x'_1,x'_2,\ldots,x_n'}$ - $d$-dimensional vector-valued indetermininates.
\item $d\times d$ matrix valued indeterminates $\Sigma, \Pi, \Theta$.
\end{enumerate}
and polynomial inequalities:
\begin{enumerate}
\item $w_i^2 = w_i$ for every $i$.
\item $w_i (x_i-x_i') = 0$ for every $i$. 
\item $\frac{1}{n} \sum_{i =1}^n x_i' x_i'^{\top} = \Sigma$.
\item $0 \preceq \Theta, \Pi$.
\item $\Pi \Theta = \Theta \Pi = I$.
\item $\Pi^2 = \Sigma$, $\Theta^2 \Sigma = \Sigma \Theta^2 = \Theta \Sigma \Theta = I$.
\item $ \frac{1}{n} \sum_{i = 1}^n \Paren{\paren{\Theta x'_i} \paren{\Theta x'_i}^{\top} - I} \Paren{\paren{\Theta x'_i} \paren{\Theta x'_i}^{\top} - I}^{\top} \preceq C I$.
\item For every $i$, $\norm{v}_2^{2t-2} \iprod{x_i,v}^2 + \delta^2 p^2\Paren{\iprod{\Theta x_i,v}} \geq \delta^2 \norm{v}_2^{2t}$.
\item $\frac{1}{n} \sum_{i = 1}^n p^2\Paren{\iprod{\Theta x_i,v}} \leq C\delta \norm{v}_2^{2t}$.
\end{enumerate}

Then, 
\begin{enumerate}
  \item \textbf{Spectral Closeness of Subsample:}
\begin{equation}
\cA \sststile{}{} \Set{\Paren{\frac{1}{n} \sum_{i \leq n} w_i - C \delta} I^{\otimes \paren{t-1}}\otimes \Sigma \preceq I^{\otimes \paren{t-1}} \otimes \frac{1}{n} \sum_{i \leq n} w_i \Paren{x_i} \Paren{x_i}^{\top} \preceq I^{\otimes t} }\mper \label{eq:spectral-LB-usage}
\end{equation}

\item \textbf{Frobenius Closeness of Isotropized Subsample according to True Covariance:} \[
\cA \sststile{6}{w}\\ \Set{ \Norm{\frac{1}{n} \sum_{i = 1}^n w_i x_i x_i^{\top}- \Paren{\frac{1}{n} \sum_{i =1}^n w_i} I}_F^{4} \leq C^2 \Paren{\frac{1}{n} \sum_{i \in n} w_i}^2 }  \mper 
\]
 \item \textbf{Frobenius Closeness of Isotropized Subsample according to Solution Covariance:} 
 \[
\cA \sststile{6}{x'_1,x'_2,\ldots,x'_n,w}\\ \Set{ \Norm{\frac{1}{n} \sum_{i = 1}^n w_i \Theta x'_i \Paren{\Theta x'_i}^{\top}- \Paren{\frac{1}{n} \sum_{i =1}^n w_i} I}_F^{4} \leq C^2 \Paren{\frac{1}{n} \sum_{i \in n} w_i}^2 }  \mper 
\]
 \item \textbf{Frobenius Closeness of Subsample to True Covariance:}
  \begin{equation}
\cA \sststile{}{} \Biggl\{\Paren{\frac{1}{n} \sum_{i \leq n} w_i - C \delta}^2 \Norm{ \frac{1}{n} \sum_{i =1}^n w_i \Sigma -\frac{1}{n} \sum_{i = 1}^n w_i x_i x_i^{\top} }_F^4 \leq C^2 \Paren{\frac{1}{n} \sum_{i \in n} w_i}^2\Biggr\}
\end{equation}



\item \textbf{Closeness between True and Solution Covariances:}

\begin{multline} \label{eq:final}
\cA \sststile{}{} \Biggl\{   \Paren{\frac{1}{n} \sum_{i \leq n} w_i - C \delta}^4\Paren{\frac{1}{n} \sum_{i \leq n } w_i}\Norm{\Sigma-I}_F^4 \leq 4 \Paren{\frac{1}{n} \sum_{i \leq n} w_i - C \delta}^2 C^2 \paren{\sum_{i \leq n} w_i}^2\\ + 4  \Paren{\frac{1}{n} \sum_{i \leq n} w_i - C \delta}^4 C^2 \paren{\sum_{i \leq n} w_i}^2 \Biggr\}\mper
\end{multline}
% \[
% \cA \sststile{}{} \Set{\Paren{\frac{1}{n} \sum_{i =  1}^n w_i }^4 \Norm{\Sigma -  I}_F^4 \leq 2\Paren{\frac{1}{n} \sum_{i =  1}^n w_i }^3 \Norm{\Sigma - I}_F^2} \mper
% \]
\end{enumerate}
\label{lem:major-lemma}
\end{lemma}
\begin{proof}
Let's start by proving the first claim.
Applying Lemma ~\ref{lem:spectral-vs-tv-general} to indeterminates $w$ and $(\Theta x'_i)$, we have:
\[
\Paren{\frac{1}{n} \sum_{i \leq n} w_i - C \delta} I^{\otimes t} \preceq I^{\otimes \paren{t-1}} \otimes \frac{1}{n} w_i \sum_{i \leq n} \Paren{\Theta x'_i} \Paren{\Theta x'_i}^{\top} \mper
\]
Observing that 
\[
\cA \sststile{}{} \Set{w_i x_i' x_i'^{\top} = w_i x_i x_i^{\top}} \mcom
\]
we thus obtain:
\[
\cA \sststile{}{} \Set{\Paren{\frac{1}{n} \sum_{i \leq n} w_i - C \delta} I^{\otimes t} \preceq I^{\otimes \paren{t-1}} \otimes \frac{1}{n} \sum_{i \leq n} w_i \Paren{\Theta x_i} \Paren{\Theta x_i}^{\top}}\mper
\]
Multiplying on left and right by $I^{\otimes t-1} \otimes \Pi$, noting that $ \cA \sststile{}{} \Set{\frac{1}{n}  \sum_{i \leq n}w_i x_i x_i^{\top} \preceq \frac{1}{n}  \sum_{i \leq n}x_i x_i^{\top} = I} \cup \Set{ \Pi^2 = \Sigma}$ yields:
\begin{equation}
\cA \sststile{}{} \Set{\Paren{\frac{1}{n} \sum_{i \leq n} w_i - C \delta} I^{\otimes \paren{t-1}}\otimes \Sigma \preceq I^{\otimes \paren{t-1}} \otimes \frac{1}{n} \sum_{i \leq n} w_i \Paren{x_i} \Paren{x_i}^{\top} \preceq I^{\otimes t} }\mper \label{eq:spectral-LB-usage}
\end{equation}
This completes the proof of the first claim.


Let's now prove the second claim. 

The hypothesis yields that $\frac{1}{n} \sum_{i \leq n} x_ix_i^{\top} = I$ and that $\sststile{}{P,w} \Set{\Iprod{\frac{1}{n} \sum_{i \leq n} x_i x_i^{\top}- I, P }^2 \leq C^2 \Norm{P}_F^2}$. Thus, applying Lemma~\ref{lem:frob-upper-bound} to constants $\{x_i\}_{i \leq n}$ and indeterminate $w$ gives:
\[
\cA \sststile{6}{w}\\ \Set{ \Norm{\frac{1}{n} \sum_{i = 1}^n w_i x_i x_i^{\top}- \Paren{\frac{1}{n} \sum_{i =1}^n w_i} I}_F^{4} \leq C^2 \Paren{\frac{1}{n} \sum_{i \in n} w_i}^2 }  \mper 
\]

The proof of the third claim is similar:

Next, consider $\{x_i'\}_{i \leq n}$. Then, 
\[
\cA \sststile{}{\Theta,P,x_1',\ldots,x_n'} \Set{\frac{1}{n} \sum_{i \leq n} (\Theta x_i') (\Theta x_i')^{\top} = I} \cup \Set{\Iprod{\frac{1}{n} x_i x_i^{\top} - I, P }^2 \leq C^2 \Norm{P}_F^2}
\] 
Thus, applying Lemma~\ref{lem:frob-upper-bound} to indeterminates $\{\Theta x_i'\}_{i \leq n}$ and $w$ gives:
\[
\cA \sststile{6}{x'_1,x'_2,\ldots,x'_n,w}\\ \Set{ \Norm{\frac{1}{n} \sum_{i = 1}^n w_i \Theta x'_i \Paren{\Theta x'_i}^{\top}- \Paren{\frac{1}{n} \sum_{i =1}^n w_i} I}_F^{4} \leq C^2 \Paren{\frac{1}{n} \sum_{i \in n} w_i}^2 }  \mper 
\]
Finally, observing that 
\[
\cA \sststile{}{} \Set{w_i x_i' x_i'^{\top} = w_i x_i x_i^{\top}} \mcom
\]
allows us to conclude:
\[
\cA \sststile{6}{x'_1,x'_2,\ldots,x'_n,w}\\ \Set{ \Norm{\frac{1}{n} \sum_{i = 1}^n w_i \Theta x_i \Paren{\Theta x_i}^{\top}- \Paren{\frac{1}{n} \sum_{i =1}^n w_i} I}_F^{4} \leq C^2 \Paren{\frac{1}{n} \sum_{i \in n} w_i}^2 }  \mper 
\]


Let's now prove the fourth claim. We have:
\begin{multline}
\cA \sststile{}{} \Biggl\{ \Paren{\frac{1}{n} \sum_{i \leq n} w_i - C \delta}^2\Norm{\Paren{\frac{1}{n} \sum_{i = 1}^n w_i}\Sigma - \frac{1}{n} \sum_{i = 1}^n w_i x_i x_i^{\top}}_F^4\\ = \Paren{\frac{1}{n} \sum_{i \leq n} w_i - C \delta}^2\Norm{ \Paren{\frac{1}{n} \sum_{i = 1}^n w_i}\Pi^2 - \Pi \Theta \frac{1}{n} \sum_{i = 1}^n w_i x_i x_i^{\top} \Theta \Pi}_F^4\\
= \Paren{\frac{1}{n} \sum_{i \leq n} w_i - C \delta}^2\Norm{ \Pi \Paren{\paren{\frac{1}{n} \sum_{i = 1}^n w_i}I- \frac{1}{n} \sum_{i = 1}^n w_i \paren{\Theta x_i} \paren{\Theta x_i}^{\top} } \Pi}_F^4 \Biggr\} \mper
\end{multline}

Next, using Lemma~\ref{fact:mixed-product-property} and the fact that $\Norm{I^{\otimes \paren{t-1}}}_F^2 = d^{t-1}$, we have:
\begin{multline}
\sststile{}{} \Biggl\{\Paren{\frac{1}{n} \sum_{i \leq n} w_i - C \delta}^2\Norm{\Pi \Paren{\paren{\frac{1}{n} \sum_{i = 1}^n w_i}-  \frac{1}{n} \sum_{i = 1}^n w_i \paren{\Theta x_i}\paren{\Theta x_i}^{\top} } \Pi}_F^4 \\= \Paren{\frac{1}{n} \sum_{i \leq n} w_i - C \delta}^2 d^{-2t+2} \Norm{ I^{\otimes \paren{t-1}} \otimes \Paren{\Pi \Paren{\paren{\frac{1}{n} \sum_{i = 1}^n w_i}- \frac{1}{n} \sum_{i = 1}^n w_i \paren{\Theta x_i}\paren{\Theta x_i}^{\top} } \Pi}}_F^4\\
=\Paren{\frac{1}{n} \sum_{i \leq n} w_i - C \delta}^2 d^{-2t+2} \Norm{ \Paren{I^{\otimes \paren{t-1}} \otimes \Pi} \Paren{I^{\otimes t-1} \otimes \Paren{\paren{\frac{1}{n} \sum_{i = 1}^n w_i}- \frac{1}{n} \sum_{i = 1}^n w_i \paren{\Theta x_i}\paren{\Theta x_i}^{\top} }} I^{\otimes t-1}\otimes \Pi}_F^4\Biggr\}
\end{multline}


Using that $\cA \sststile{}{} \Set{\Pi \Theta = \Theta \Pi = \Sigma}$, we have:
\[
\cA \sststile{}{} \Biggl\{4\Paren{\frac{1}{n} \sum_{i = 1}^n w_i}\Sigma - \frac{1}{n} \sum_{i = 1}^n w_i x_i x_i^{\top} = \Pi \Paren{  \frac{1}{n} w_i I - \frac{1}{n} w_i \Paren{\Theta x_i} \Paren{\Theta x_i}^{\top}} \Pi\Biggr\}\mper
\]





% Next, consider $\{x'_i\}_{i \leq n}$. Then, we know that $\frac{1}{n} (\Thetax_i x_i^{\top} = I$ and $\sststile{4}{w,P} \Set{\Iprod{\frac{1}{n} x_i x_i^{\top} - I, P }^2 \leq C^2 \Norm{P}_F^2}$. Thus, applying Lemma~\ref{lem:frob-upper-bound} to indeterminates $\{x_i\}_{i \in \cI}$ and $w$, yields:
% \[
% \cA \sststile{6}{x_1,x_2,\ldots,x_n,w}\\ \Set{ \Norm{\frac{1}{n} \sum_{i = 1}^n w_i x_ix_i^{\top}- \Paren{\frac{1}{n} \sum_{i =1}^n w_i} I}_F^{4} \leq C^2 \paren{\frac{1}{n} \sum_{i \in n} w_i}^2 }  \mper 
% \]



Now, $\paren{I^{\otimes t-1}\otimes \Pi}^2 = I^{\otimes t-1} \otimes \Sigma$. Using the result from part 1  with Lemma~\ref{lem:contraction-property}, the fact that $\cA \sststile{}{} \Set{\Pi^2 = \Sigma}$ and Fact~\ref{fact:mixed-product-property} again, we have:
\begin{multline}
\cA \sststile{}{} \Biggl\{d^{-2t+2} \Paren{\frac{1}{n} \sum_{i \leq n} w_i - C \delta}^2 \Norm{ \Paren{I^{\otimes \paren{t-1}} \otimes \Pi} \Paren{\paren{\frac{1}{n} \sum_{i = 1}^n w_i} I^{\otimes t} -  I^{\otimes t-1} \otimes  \frac{1}{n} \sum_{i = 1}^n w_i \Paren{\Theta x_i}\Paren{\Theta x_i}^{\top} } \Paren{I^{\otimes \paren{t-1}} \otimes \Pi} \ }_F^4\\ \leq d^{-2t+2} \Norm{I^{\otimes \paren{t-1}} \otimes \Paren{ \paren{\frac{1}{n} \sum_{i = 1}^n w_i} I-  \frac{1}{n} \sum_{i = 1}^n w_i \Paren{\Theta x_i}\Paren{\Theta x_i}^{\top} }}_F^4\\
=\Norm{\paren{\frac{1}{n} \sum_{i = 1}^n w_i} I-  \frac{1}{n} \sum_{i = 1}^n w_i \Paren{\Theta x_i}\Paren{\Theta x_i}^{\top} }_F^4\Biggr\}
\end{multline}


Combining the above arguments allows us to finally conclude:
\begin{multline}
\cA \sststile{}{} \Biggl\{\Paren{\frac{1}{n} \sum_{i \leq n} w_i - C \delta}^2 \Norm{ \frac{1}{n} \sum_{i =1}^n w_i \Sigma -\frac{1}{n} \sum_{i = 1}^n w_i x_i x_i^{\top} }_F^4 \leq \Norm{\Paren{ \paren{\frac{1}{n} \sum_{i = 1}^n w_i} I- \Theta \frac{1}{n} \sum_{i = 1}^n w_i x_i x_i^{\top} \Theta}}_F^4\Biggr\}
\end{multline}
Applying the result from part 3 then gives us the claim.


% \[
% \cA \sststile{}{} \Set{\Norm{\Sigma-I}_F^4 \leq 4\Norm{\Paren{\frac{1}{n} \sum_{i = 1}^n w_i}\Sigma - \frac{1}{n} \sum_{i = 1}^n w_i x_i x_i^{\top}}_F^4 +4 \Norm{\frac{1}{n} \sum_{i = 1}^n w_i x_i x_i^{\top} -\Paren{\frac{1}{n} \sum_{i = 1}^n w_i} I}_F^4 }\mper
% \]


We are now ready to prove the final claim.

% \[
% \cA \sststile{}{} \Set{ \Norm{\Paren{\frac{1}{n} \sum_{i = 1}^n w_i}\Sigma - \frac{1}{n} \sum_{i = 1}^n w_i x_i x_i^{\top}}_F^4 = \Norm{\Paren{\frac{1}{n} \sum_{i = 1}^n w_i}\Pi^2 - \Pi \Theta \frac{1}{n} \sum_{i = 1}^n w_i x_i x_i^{\top} \Theta \Pi}_F^4} \mper
% \]
% And thus,
% \[
% \cA \sststile{}{} \Set{ \Norm{\Paren{\frac{1}{n} \sum_{i = 1}^n w_i}\Sigma - \frac{1}{n} \sum_{i = 1}^n w_i x_i x_i^{\top}}_F^4 = \Norm{\Pi \Paren{\Paren{ \frac{1}{n} \sum_{i = 1}^n w_i}I - \Theta \frac{1}{n} \sum_{i = 1}^n w_i x_i x_i^{\top} \Theta} \Pi}_F^4} \mper
% \]
% Next, using Fact~\ref{fact:frob-of-I-tensor}, 
% \[
% \sststile{}{} \Set{ \Norm{I^{\otimes \paren{t-1}} \otimes \Paren{\Paren{\frac{1}{n} \sum_{i = 1}^n w_i}\Sigma - \frac{1}{n} \sum_{i = 1}^n w_i x_i x_i^{\top}}}_F^4 = d^{2t-2}\Norm{\Paren{\frac{1}{n} \sum_{i = 1}^n w_i}\Sigma - \frac{1}{n} \sum_{i = 1}^n w_i x_i x_i^{\top}}_F^4} 
% \]

% Now, using Fact~\ref{fact:mixed-product-property} repeatedly, 
% \[
% \cA \sststile{}{} \Set{ \Norm{I^{\otimes \paren{t-1}} \otimes \Paren{\Paren{\frac{1}{n} \sum_{i = 1}^n w_i}\Sigma - \frac{1}{n} \sum_{i = 1}^n w_i x_i x_i^{\top}}}_F^4 = \Norm{I^{\otimes \paren{t-1}}\otimes\Pi \Paren{\Paren{ \frac{1}{n} \sum_{i = 1}^n w_i}I - \Theta \frac{1}{n} \sum_{i = 1}^n w_i x_i x_i^{\top} \Theta} \Pi}_F^4} \mper
% \]

% Using Lemma~\ref{lem:contraction-property} along with Lemma~\ref{lem:spectral-vs-tv-general}, 

% \begin{multline}
% \cA \sststile{}{} \Biggl\{\Norm{I^{\otimes \paren{t-1}}\otimes\Pi \Paren{\Paren{ \frac{1}{n} \sum_{i = 1}^n w_i}I - \Theta \frac{1}{n} \sum_{i = 1}^n w_i x_i x_i^{\top} \Theta} \Pi}_F^4 \\ 
% = \Norm{\Paren{I^{\otimes \paren{t-1}}\otimes\Pi} I^{\otimes \paren{t-1}}\otimes \Paren{\Paren{ \frac{1}{n} \sum_{i = 1}^n w_i}I - \Theta \frac{1}{n} \sum_{i = 1}^n w_i x_i x_i^{\top} \Theta} \Paren{I^{\otimes \paren{t-1}}\otimes \Pi}}_F^4\Biggr\} \mper
% \end{multline}
% Applying Lemma~\ref{lem:contraction-property}, we obtain:
% \begin{multline}
% \cA \sststile{}{} \Biggl\{\Norm{I^{\otimes \paren{t-1}} \otimes \Paren{\Paren{\frac{1}{n} \sum_{i = 1}^n w_i}\Sigma - \frac{1}{n} \sum_{i = 1}^n w_i x_i x_i^{\top}}}_F^4  \leq \\
% \Norm{\Paren{I^{\otimes \paren{t-1}}\otimes\Pi} I^{\otimes \paren{t-1}}\otimes \Paren{\Paren{ \frac{1}{n} \sum_{i = 1}^n w_i}I - \Theta \frac{1}{n} \sum_{i = 1}^n w_i x_i x_i^{\top} \Theta} \Paren{I^{\otimes \paren{t-1}}\otimes \Pi}}_F^4\Biggr\} \mper
% \end{multline}

\[
\cA \sststile{}{} \Set{ \Paren{\frac{1}{n} \sum_{i \leq n } w_i}\Paren{\Sigma-I} = \Paren{\frac{1}{n} \sum_{i \leq n } w_i} \Sigma - \frac{1}{n} \sum_{i = 1}^n w_i x_i x_i^{\top} + \frac{1}{n} \sum_{i = 1}^n w_i x_i x_i^{\top} -\Paren{\frac{1}{n} \sum_{i \leq n } w_i} I  }
\]
Applying $\sststile{4}{a,b} \Set{ (a+b)^4 \leq 4a^4 + 4b^4}$ for each entry of the above matrix valued indeterminates,
\begin{multline} \label{eq:first-triangle}
\cA \sststile{}{} \Biggl\{   \Paren{\frac{1}{n} \sum_{i \leq n} w_i - C \delta}^4\Paren{\frac{1}{n} \sum_{i \leq n } w_i}\Norm{\Sigma-I}_F^4 \\\leq 4 \Paren{\frac{1}{n} \sum_{i \leq n} w_i - C \delta}^4\Norm{\Paren{\frac{1}{n} \sum_{i = 1}^n w_i}\Sigma - \frac{1}{n} \sum_{i = 1}^n w_i x_i x_i^{\top}}_F^4\\ +4 \Paren{\frac{1}{n} \sum_{i \leq n} w_i - C \delta}^4 \Norm{\frac{1}{n} \sum_{i = 1}^n w_i x_i x_i^{\top} -\Paren{\frac{1}{n} \sum_{i = 1}^n w_i} I}_F^4 \Biggr\}\mper
\end{multline}

We now apply the result from part 4 to bound the first term on the RHS and the result from part 2 to bound the second terms on the RHS. This allows us to conclude:

\begin{multline} \label{eq:final}
\cA \sststile{}{} \Biggl\{   \Paren{\frac{1}{n} \sum_{i \leq n} w_i - C \delta}^4\Paren{\frac{1}{n} \sum_{i \leq n } w_i}\Norm{\Sigma-I}_F^4 \leq 4 \Paren{\frac{1}{n} \sum_{i \leq n} w_i - C \delta}^2 C^2 \paren{\sum_{i \leq n} w_i}^2\\ + 4  \Paren{\frac{1}{n} \sum_{i \leq n} w_i - C \delta}^4 C^2 \paren{\sum_{i \leq n} w_i}^2 \Biggr\}\mper
\end{multline}





\end{proof}


==> content/old/analyzingconstraints.tex <==
%!TEX root = ../main.tex


\input{content/analyzingconstraints}
\subsection{Analyzing $\cA_{w,\Sigma^*}$: Proof of Lemma ~\ref{lem:main-sosized-fact}}


We prove Lemma~\ref{lem:main-sosized-fact} using the following three results.
\begin{lemma}[SoSized Anticoncentration]
Anti-concentration...using polynomial..
\end{lemma}

\begin{lemma}
Relating trace powers of projectors to frobenius error.
\end{lemma}
\FIXME{add proof for this lemma here.}

\begin{lemma}[Technical SoS fact about Powering]

\end{lemma}\FIXME{add proof for this lemma in appendix.}

\begin{proof}[Proof of Lemma \ref{lem:main-sosized-fact}]

\end{proof}

==> content/old/content-old.tex <==
%!TEX root = ../main.tex

\section{Partitions and Distributions}
\begin{definition}(Coarse Soluble Partition): A partition of the samples of $\sub_{\cN}{\alpha, \PI^*}$, into sets $\XX_1, \XX_2, \ldots \XX_s$ is a coarse soluble partition if for all $i\in [s]$, $|\XX_i| \geq \alpha n$ and rank$(\XX_i\XX_i^T) =k$.
\end{definition}
\noindent Note, such a partition need not exist in general. However, if we can find such a partition, we have certificate that the partition (a short list) contains the optimal solution. 
\begin{lemma}
\label{lem:basic_anti_conc}
Let $\XX_{in}$ be $\alpha$-anti-concentrated. Let $\XX_1, \XX_2, \ldots \XX_s$ be a coarse soluble partition of the rows of $\XX$. Then, there exists $i\in [s]$ such that colspan$(\XX_i) = \PI^*$. 
\end{lemma}
\begin{proof}
Since $|\XX_i| \geq \alpha n$, $s \leq \frac{1}{\alpha}$. Therefore, there exists $i \in [s]$ such that $|\XX_{in} \cap \XX_i| \geq \alpha^2 n$. Let $v$ be a vector in ker$(\XX_{in} \cap \XX_i)$. Then, 
\[
\prob{x_i \sim \XX_i}{<x_i, v> = 0} \geq \alpha
\]
which contradicts $\alpha$-anti-concentration unless ker$(\XX_{in} \cap \XX_i) = \phi$ and thus colspan$(\XX_{in}) =$ colspan$(\XX_i)$. 
\end{proof}

\noindent For an arbitrary subset of rows of $\XX$, denoted by $\mathcal{S}$, 
let $W_{i}(\mu) = \expec{\mathcal{S} \sim \mu}{ \mathbf{1}(\XX_{i,*} \in S) }$ 
be the frequency that row $\XX_{i,*}$ is chosen to be in the set $\mathcal{S}$. The uniform distribution sets $W_i = \frac{1}{k}$ for all $i \in [n]$. Define 
$\sum_{i \in [n]} W^2_i(\mu)$ to be the distance from uniformity. Minimizing 
$\sum_{i \in [n]} W^2_i(\mu)$ gives us a 'maximally-uniform' distribution among all possible distributions over rows of $\XX$. Observe, this distribution can 
be computed using convex programming. \textcolor{red}{what is the convex 
program for this? the description is large since $|S| \geq \alpha n$. }

\begin{lemma}
\label{lem:max_uni_dist}
For a maximally uniform distribution on $\alpha n$ sized soluble partition, $\mathcal{S}$, of rows of $\XX$, $\sum_{i \in \XX_{in}} \expec{\mathcal{S} \sim \mu}{\mathbf{1}(\XX_{i,*} \in S)} \geq \alpha^2 n$.
\end{lemma}
\begin{proof}

\end{proof}

\begin{lemma}(Identifiability):
Let $\XX$ be a $n \times d$ matrix sampled from $\sub_{\mathcal{N}}(\alpha, \PI^*)$ such that $\XX_{in}$ is $\delta$-anit-concentration for $\delta < \alpha$. Then, there exists an algorithm that outputs a list $\mathcal{L}$ of size $O(\frac{1}{\alpha-\delta})$ such that $\PI^* \in \mathcal{L}$, with probability at least $99/100$. 
\end{lemma}
\begin{proof}
The proof is very similar to [KKK'19] and follows from combining Lemma \ref{lem:max_uni_dist} and Lemma \ref{lem:basic_anti_conc}. Algorithmically, we sample $\ell = \frac{c}{\alpha - \delta}$ sets iid from $\mu$. Let these sets be denoted by $\SS_1, \SS_2, \ldots \SS_\ell$. For each $\SS_j$ output colspan$(\SS_j)$.   \textcolor{red}{why is it the case that picking $t$ samples from $\mu$ results in a unique $k$ dim subspace spanning each subset? This is also unclear for regression, why does such a sample from such a set have a consistent labelling?} By Lemma \ref{lem:max_uni_dist} we know 
$$ \expecf{}{|\SS_j \cap \XX_{in}| } = \sum_{x \in \XX_{in} } \Pr\left[ x \in \SS_j \right]  \geq \alpha |\XX_{in}| $$
By Markov's we have $$\Pr\left[ |\SS_j \cap \XX_{in}| \geq \frac{\alpha + \delta}{2} |\XX_{in}| \right] \geq \frac{\alpha - \delta}{2}$$
For all $j \in [\ell]$ let $\zeta_j$ be the indicator random variable for the event $|\SS_j \cap \X_{in}| \geq \frac{\alpha + \delta}{2} |\XX_{in}|$. Let $\zeta = \sum_{j \in [\ell] }\zeta_{\ell}$. Then, 
$$\Pr[\zeta \geq 1] = 1- \Pr[\zeta =0] = 1 - \left( 1- \frac{\alpha-\delta}{2} \right)^{\frac{c}{\alpha-\delta}} \geq \frac{99}{100}$$
Then, with probability at least $99/100$, there exists a $j \in [\ell]$ such that $|\SS_j \cap \X_{in}| \geq \frac{\alpha + \delta}{2} |\XX_{in}|$. The claim follows from the same argument presented in Lemma \ref{lem:basic_anti_conc}. 
\end{proof}



\section{Certifying Lower Bounds on Covariance}

\begin{lemma}[Certifying Lower Bounds on Covariance]
Let $x_1, x_2,  \ldots, x_n \sim \cN(0,I_d)$. Then, for all $n \geq n_0 = \Omega(d^{1/\alpha^4})$, with probability at least $0.99$ over the draw of the $x_i$s,  
\[
\Set{w_i^2 = w_i \forall 1 \leq i \leq n, \text{ } \sum_{i =1 }^n w_i = \alpha n} \sststile{t}{v} \frac{1}{\alpha n} \sum_{i  = 1}^n w_i \iprod{x_i,v}^2 \geq \alpha^2 \frac{1}{n}\sum_{i= 1}^n \iprod{x_i,v}^2\mcom
\]
for $t = O(1/\alpha^4)$.


\end{lemma}
\begin{proof}

\end{proof}

==> content/old/graveryard.tex <==
\section{Graveyard}
\begin{lemma}(Convergence of Higher Moments.)
\label{lem:conv_of_p}
Let $\X = \{x_1, x_2, \ldots x_n\} \in \mathbb{R}^d$  be a set of points such that, for $n = \Omega( (kd\log(d))^{O(k)})$, with probability at least $1-1/d$,  the $k$-th empirical moment of $\X$
is close to that of $\N(0, \Sig)$, i.e.
\begin{equation*}
	\Big\| \frac{1}{n}\sum_{i \in [n]} x_i^{\otimes k}  - \expecf{x \sim \N(0, \Sig)}{x^{\otimes k}}\Big\|^2_F \leq \eta
\end{equation*} 
Then, assuming a $(1, \delta)$-Indicator Polynomial $p$ exists and has degree $k$, for all $v$, *make this a fact*
\begin{equation*}
    \frac{1}{n}\sum_{i \in [n]} p^2(\iprod{x_i v}) \leq 4 \expecf{x\sim \cN(0,\Sig)}{p^2(\iprod{x, v})}
\end{equation*}
\end{lemma}
\begin{proof}
This follows from Lemma 5.5 in \cite{}. For a complete proof refer to the Appendix. 
\end{proof}


\begin{proof}
Proof idea for prop \ref{prop:relaxed_moment_matching}: if it is not the case, mix with a distribution that assigns higher weight to the inliers. Let $u = 1/\alpha n \expecf{\cD'}{w}$ be discrete distribution over $w$ such that $\sum_{i\in [n]} u_i = 1$. Let $wt(\I) = \sum_{i \in \I} u_i $ and $wt(\O) = \sum_{i \notin \I} u_i$. If $wt(\I) < \beta$, we show there exists a distribution $\widehat{\cD}$ over $w$ such that $\|\expecf{\widehat{\cD}}{ w}\|^2_2 < \|\expecf{\cD}{w} \|^2_2$. We construct the distribution $\widehat{\cD}$ by mixing $\cD$ with the ideal distribution, where $w_i = 1$ for $i \in \I$, denoted by $\cD^*$. Since $\cD^*$ satisfies all the constrains, any conic combination of $\cD^*$ and $\cD$ satisfies all constraints. We then show that there exists a $\lambda >0 $, such that if $\widehat{D} = \lambda \cD + (1-\lambda) \cD^*$ then $\|\expecf{\widehat{\cD}}{ w}\|^2_2 < \|\expecf{\cD}{w} \|^2_2$. \FIXME{finish this proof.} 
\end{proof}
\section{Certifying Lower Bounds on Covariance}
\begin{lemma}[Certifying Lower Bounds on Covariance]
Let $x_1, x_2,  \ldots, x_n \sim \cN(0,\Sig^*)$. Then, for all $n \geq n_0 = \Omega(d\log(d)^{1/\alpha^2})$, with probability at least $0.99$ over the draw of the $x_i$s,
\[
\Set{w_i^2 = w_i \forall 1 \leq i \leq n, \text{ } \sum_{i =1 }^n w_i = \alpha n} \sststile{t}{v} \frac{1}{\alpha n} \sum_{i  = 1}^n w_i \iprod{x_i,v}^2 \geq \alpha^2 \frac{1}{n}\sum_{i= 1}^n \iprod{x_i,v}^2\mcom
\]
for $t = O(1/\alpha^2)$.


\end{lemma}
\begin{proof}

\end{proof}

We use the following fact: 

\begin{fact}[Sub-gaussian Convergence, Prop 2.1 \cite{}]
\label{fact:sub_gaussian_conv}
Let $x_1, x_2, \ldots x_n \in \mathbb{R}^{d}$ be i.i.d samples from $\cN(0, \Sig)$. Then, for $n\geq d$, for any $\delta > 0$ with probability at least $1-\eta$,
\begin{equation}
\Big\| \frac{1}{n}\sum_{i \in [n]} x_i x_i^{\top} - \Sig  \Big\|_2 \leq c_{\eta} \sqrt{\frac{d}{n}}
\end{equation}
where $c_{\eta}$ is a fixed constant dependent on $\eta$.
\end{fact}



\begin{lemma}
\label{lem:moment_matching_proximity}
Let $0<\delta < \beta/8 < \alpha$. 
Let $\{x_1, x_2, \ldots x_n\}$ be samples from $\sub_{\cN}(\alpha, \Sig^*)$ such that $n \geq n_0$ where $n_0 = \Omega\left( ( d\log(d)/\beta^2)^{O(1/\beta^2)}/\alpha \right)$.
Suppose  $w \in \mathbb{R}^n$  such that for all $i\in[n]$, $w_i= w_i^2$, $\sum_{i\in[n]} w_i \geq \alpha n$, $\sum_{i \in \I} w_i \geq \beta | \I |$. Let $S$ be a subset of $\alpha n$ points such that the corresponding $w_i=1$ and $S$ is $( 1/\delta^2, \Sig)$-Near-Gaussian
for some fixed $\Sig$.
Then, with probability at least $1-1/d$, 
$$(1-\delta)\Sig^* \preceq \frac{1}{\alpha n} \sum_{i\in [n]} w_i x_i x_i^{\top} \preceq (1+\delta) \Sig^* $$
\end{lemma}
\begin{proof}
Let $\Y$ be the set of $x_i$ corresponding to $w_i=1$. By assumption, we know that he empirical  moments of $\Y$ are close to that of $\cN(0, \Sig^*)$. Let $\X_1$ be the subset of the inliers $\I$ such that $w_i =1$. Then, $| \X_1| \geq \beta |\I|$. For large enough $n \geq n_0$, it follows from  Lemma \ref{lem:projective_proximity}, that $\Sig = \Sig^*$. 

Now, observe for any $v$ such that $ v^{\top}\Sig^* v=0$, it also holds that  $ \sum_{i \in[n]} \iprod{w_i x_i, v}^2 =0$. Therefore, the kernel of $\Sig^*$ is preserved perfectly. Next, by Fact \ref{fact:sub_gaussian_conv}, it holds that with probability at least $1-1/d$,
\begin{equation*}
    \Big\| \frac{1}{\alpha n}\sum_{i \in [n]} w_i x_i x_i^{\top} - \Sig \Big\|^2_2 \leq \delta
\end{equation*}
Combined with the fact that $\Sig= \Sig^*$, for all unit vectors $v$ such that $v^{\top} \Sig v \neq 0$,
\begin{equation*}
    \frac{1}{\alpha n}\sum_{i\in [n]} w_i\iprod{x_i, v}^2 = (1\pm \delta) v^{\top} \Sig^* v
\end{equation*}
and the claim follows.
\end{proof}


\subsection{Useless stuff}
\begin{lemma}[When is a mixture model clusterable?]
Given $\alpha>0$ and two multivariate normal distributions $\cN(\mu_1, \Sigma_1), \cN(\mu_2, \Sigma_2)$ such that for all $v$, $\langle \mu_i - \mu_j, v \rangle^2 \leq \Delta_1 \log(1/\alpha) v^{\top} (\Sigma_1 + \Sigma_2) v$, $\Norm{\Sigma_1^{-1} \Sigma_2}_2 \leq \Delta_2 1/\alpha$,  $\Norm{\Sigma_2^{-1} \Sigma_1}_2 \geq \Delta_2 \alpha$ and $\Norm{ \Sigma_1^{-1/2} \Sigma_2 \Sigma_1^{-1/2}-I}_F \leq \Delta_3 1/\alpha$, then, $\dtv\left(\cN(\mu_1, \Sigma_1), \cN(\mu_2, \Sigma_2) \right)^2 \leq 1 -\exp(-c\log(1/\alpha)/\alpha)$, for a fixed constant $c$ depending on $\Delta_1, \Delta_2$ and $\Delta_3$.
\end{lemma}

\begin{proof}

By definition of Hellinger distance, we have 
\begin{equation*}
\dtv\left(\cN(\mu_1, \Sigma_1), \cN(\mu_2, \Sigma_2) \right)^2  \leq h^2\left(\cN(\mu_1, \Sigma_1), \cN(\mu_2, \Sigma_2) \right)\left(2-h^2 \left(\cN(\mu_1, \Sigma_1), \cN(\mu_2, \Sigma_2) \right)\right)
\end{equation*}

Observe, it suffices to lower bound $\frac{\det(\Sigma_1 \Sigma_2)^{\frac{1}{2}}}{\det\left( (\Sigma_1+ \Sigma_2)/2\right)} \exp\left(- (\mu_1 - \mu_2)^{\top}(\Sigma_1 + \Sigma_2)^{-1} (\mu_1 - \mu_2)/4 \right)$. Alternatively, it suffices to upper bound
\begin{equation}
\label{eqn:split}
\log\left( \frac{\det(\Sigma_1 + \Sigma_2)}{2\det\left( \Sigma_1\Sigma_2\right)^{1/2}} \right) + \log\left(\exp\left(- \frac{(\mu_1 - \mu_2)^{\top}(\Sigma_1 + \Sigma_2)^{-1} (\mu_1 - \mu_2)}{4} \right) \right)
\end{equation}
We bound these terms separately. For the first term, we consider the Linear Transformation that maps $\Sigma_1$ to $\II$ and $\Sigma_2$ to $\Sigma= \Sigma_1^{-1/2}\Sigma_2 \Sigma_1^{-1/2}$. Observe, $\Norm{ \Sigma_1^{-1/2} \Sigma_2 \Sigma_1^{-1/2}-I}_F = \Norm{ \Sigma-I}_F  \leq \Delta_3 1/\alpha$ still holds by definition. Since $\Sigma^{-1}_1\Sigma_2$ and $\Sigma^{-1/2}_1\Sigma_2\Sigma^{-1/2}$ are similar matrices, they have the same eigenvalues. Therefore, $\Norm{\Sigma}_2 \leq \Delta_2 1/\alpha$ and $\Norm{\Sigma}_2 \geq \Delta_2 \alpha$.
Thus, to upper bound the first term in \eqref{eqn:split}, it suffices to bound
\begin{equation*}
\log\left( \frac{\det(\II + \Sigma)}{2\det\left( \Sigma^{1/2}\right)} \right) =  \sum_{i\in [d]}\log\left(\frac{1+\lambda_i}{2\sqrt{\lambda_i}}\right)
\end{equation*}

Let $\lambda_1, \lambda_2, \ldots \lambda_n$ be eigenvalues of $\Sigma$.
Consider the subset of eigenvalues $\cE$ such that for all $i\in\cE$, $\lambda_i \geq 1.5$. Since $\sum_{i \in \cE}(1- \lambda_i)^2 \leq\sum_{i \in [d]}(1- \lambda_i)^2 = \|\II - \Sigma \|^2_F \leq \Delta_3 (1/\alpha)$ and $\sum_{i \in \cE}(1- \lambda_i)^2 \geq |\cE|/4$, we can conclude $|\cE| \leq 4/\alpha$.
Note, for all $i\in \cE$,  $1+\lambda_i \leq 2\lambda_i$. Therefore,
\begin{equation*}
\sum_{i: \lambda_i \text{ is large }} \log\left(\frac{1+\lambda_i}{2\sqrt{\lambda_i}}\right) \leq \sum_{i\in \cE} \log\left(\sqrt{\lambda_i} \right) \leq \frac{2 \Delta }{\eta}\cdot \log(1/\eta)
\end{equation*}
where the last step uses that $\lambda_i \leq \Delta/\eta$.

Let's now consider all the remaining \emph{small} eigenvalues that satisfy $\eta/\Delta \leq\lambda_i < 1.5$. Then, we can write $\lambda_i = 1+\beta_i$ such that $-(1-\eta/\Delta)\leq \beta_i \leq 0.5$. Then, we have
\begin{equation*}
\begin{split}
\sum_{i:\lambda_i \leq 1.5} \log\left(\frac{1+\lambda_i}{2}\right) + \frac{1}{2}\log\left(\frac{1}{\lambda_i}\right) &= \sum_{i \in \cE'} \log\left(1+\frac{\beta_i}{2}\right) - \frac{1}{2}\log\left(1+\beta_i\right) \\
&\leq \sum_{i:\lambda_i \leq 1.5} \frac{\beta_i}{2} - \frac{\beta_i}{2} + \frac{\beta_i^2}{4}\\
& = \sum_{i:\lambda_i \leq 1.5} \frac{(1-\lambda_i)^2}{4} \leq \frac{\Delta}{4\eta}
\end{split}
\end{equation*}
where the last inequality follows from $\sum_{i \in \cE'} (1-\lambda_i)^2 \leq \| \II - \Sigma\|^2_F\leq \frac{\Delta_3}{\alpha}$. Therefore, we can conclude $\sum_{i\in [d]}\log\left(\frac{1+\lambda_i}{2\sqrt{\lambda_i}}\right) \leq O\left(\frac{\log(1/\alpha)}{\alpha}\right)$.

Next, we bound $(\mu_1 - \mu_2)^{\top}(\Sigma_1+ \Sigma_2)^{-1} (\mu_1 - \mu_2)$. Setting $v= (\Sigma_1+ \Sigma_2)^{-1} (\mu_1 - \mu_2)$ in the mean separation condition we have $\left((\mu_1 - \mu_2)^{\top}(\Sigma_1+ \Sigma_2)^{-1} (\mu_1 - \mu_2)\right)^2 \leq \Delta_1 \log(1/\alpha)(\mu_1 - \mu_2)^{\top}(\Sigma_1+ \Sigma_2)^{-1} (\mu_1 - \mu_2)$. Rearranging the terms, we get $(\mu_1 - \mu_2)^{\top}(\Sigma_1+ \Sigma_2)^{-1} (\mu_1 - \mu_2)\leq \Delta_1\log(1/\alpha)$. Combining the two terms, we have
\begin{equation*}
\begin{split}
\dtv \left(\cN(\mu_1,\Sigma_1), \cN(\mu_2,\Sigma_2)\right)^2 \leq 1 - \exp(-c\log(1/\alpha)/\alpha)
\end{split}
\end{equation*}
for a fixed constant $c$. 

\end{proof}


==> content/old/pruning.tex <==
%!TEX root = ../main.tex
\subsection{Analysis of Pruning}
\newcommand{\pr}{\mathsf{prune}}
\newcommand{\hw}{\hat{w}}
\newcommand{\param}{\mathsf{param}}


\begin{mdframed}[nobreak=true]
  \begin{algorithm} Pruning Lists %\Anote{The pruning algorithm is huge now and I am not sure we should fit it into a box? We also introduce the pruning constraints later on so it may not make much sense to say here what exactly they are. For this box, maybe we can just say that theres an algorithm that takes a large list and outputs a small list, details described in Subsection \ref{}.  } \Pnote{The algorithm should be described here. }
  \label[algorithm]{alg:pruning-general}
    \mbox{}
    \begin{description}
    \item[Given:]
    A list $\cL'$ of $d \times d$ Covariance matrices
      \item[Operation:] \textbf{} \\
      \vspace{-0.3in}
      \begin{enumerate}
          \item Let $d_{\param}$ be a metric on the parameter space (as defined in \ref{def:parameter_metric} ). Let $\eta = $\Anote{set $\eta$ to be radius that we use to cluster. } Greedily partition tuples $(\mu, \Sigma) \in \cL'$ into sets $\cS_1, \cS_2 \ldots \cS_{z}$ such that the pair-wise distance between all tuples in the same set is at most $2\eta$. For each $\ell \in [z]$, let $(\mu_{\ell}, \Sigma_{\ell})$ denote an arbitrary representative of $\cS_{\ell}$.
          \item For $\ell \in [z]$,
          \begin{enumerate}
          \item Consider the system of polynomial constraints given by $\cA_{\pr}(\mu_{\ell}, \Sigma_{\ell})$ (defined in Equations \eqref{eqn:prune_intersection},  \eqref{eqn:prune_parameter}, \eqref{eqn:prune_cert_anti_conc},\eqref{eqn:prune_cert_hypercontractive} and \eqref{eqn:prune_param_dist} below).
          \item If the system is feasible, append the tuple $(\mu_{\ell}, \Sigma_{\ell})$ to $\cL$. Else, discard the set $\cS_{\ell}$.
          \end{enumerate}
      \end{enumerate}
     \item[Output:]
      A $\cL \subseteq \R^d$ of size $O(1/\alpha)$  such that there exists a mean vector $\hat{mu}$ and Covariance matrix $\hat{\Sigma} \in \cL$ satisfying satisfying $\Norm{\Sigma_*^{-1/2}(\mu-\mu_*)}_2^2 \leq O(s^{2} \alpha^{-2} \alpha^{-2/s})$, $\Omega\Paren{\frac{\alpha}{s}}^2 \alpha^{2/s} I \preceq  \Sigma_*^{-1/2} \hat{\Sigma} \Sigma_*^{-1/2}$, and $\Norm{I - \Sigma_*^{-1/2} \Sigma \Sigma_*^{-1/2}}_F^2 \leq O(h^{4} \alpha^{-4} \alpha^{-6/h})$. \Anote{these are parameters from large list rounding, add real parameters here.}
    \end{description}
  \end{algorithm}
\end{mdframed}



Our TV to Parameter distance lemmas (Lemmas~\ref{lem:spectral-distance-LDC},~\ref{lem:mean-closeness-main},~\ref{lem:rel-frob-close-main}) immediately allow us to conclude (we formalize this in Corollary~ below) that whenever two nice distributions are non-trivially close in total variation distance, then their corressponding parameters $(\mu,\Sigma)$ must be close in appropriate notions of distances. Since we will repeatedly talk about the parameter distances in this section, we introduce the following compact notation:

% \begin{definition}[Parameter Distance]
% Let $P_1 = (\mu_1,\Sigma_1)$ and $P_2 = (\mu_2,\Sigma_2)$ be two parameter pairs such that $\mu_1, \mu_2 \in \R^d$ and $\Sigma_1, \Sigma_2 \in \R^{d\times d}$ are PSD. We say that $d_{\param}(P_1, P_2) \leq 1- \eta$ if
% \begin{enumerate}
% \item \[ \Norm{\hat{\Sigma}^{-1/2}(\hat{\mu}-\mu)}^2_2 \leq s(\eta/2)^2 \]
% \item \[ \Norm{\hat{\Sigma}^{-1/2} \Sigma \hat{\Sigma}^{-1/2}-I}_F^2 \leq s(\eta/2)^4/\eta^4 \]
% \item \[ \forall v \text{  } v^{\top} \hat{\Sigma}^{-1/2} \Sigma \hat{\Sigma}^{-1/2}v \geq \Paren{\frac{\eta}{s(\eta/2)}}^2 \]
% \end{enumerate}
% \end{definition}

\begin{definition}[Notation for Parameter Closeness]
\label{def:parameter_metric}
Let $P_1 = (\mu_1,\Sigma_1)$ and $P_2 = (\mu_2,\Sigma_2)$ be two parameter pairs such that $\mu_1, \mu_2 \in \R^d$ and $\Sigma_1, \Sigma_2 \in \R^{d\times d}$ are PSD. We say that $d_{\param}(P_1, P_2) \leq 1- \eta$ if $\Norm{\hat{\Sigma}^{-1/2}(\hat{\mu}-\mu)}^2_2 \leq s^{2} \eta^{-2} \eta^{-2/s}$, $\Norm{\hat{\Sigma}^{-1/2} \Sigma \hat{\Sigma}^{-1/2}-I}_F^2 \leq s^{4} \eta^{-4} \eta^{-6/s}$, $\forall v \text{  } v^{\top} \hat{\Sigma}^{-1/2} \Sigma \hat{\Sigma}^{-1/2}v \geq \Paren{\frac{\eta}{s}}^2 \eta^{2/s}$.
\end{definition}

The starting point for our  pruning algorithm is the following stand-alone corollary of our distance lemmas from the previous subsections stated using the above compact notation.

% In this compact notation, we can immediately conclude the following relationship between total variation distance and parameter distance from our distance lemmas in the previous subsections.
\Anote{this should be corollary of rounding lemmas }
\begin{corollary}[Corollary of Lemmas~\ref{lem:spectral-distance-LDC},\ref{lem:mean-closeness-main},~\ref{lem:rel-frob-close-main}] \label{cor:distilled-tv-to-param}
Fix $Y = \{y_1, y_2, \ldots, y_n\} \subseteq \R^d$. Let $\cB,\cB'$ be distributions supported on such that $\dtv(\cB,\cB') \leq 1-\eta$ such that the probability of any $y_i$ is at most $\frac{1}{\alpha n}$ under each. Suppose $\cB,\cB'$ are $s$-certifiably $(\delta,C\delta)$-anti-concentrated and $h$-certifiably $C$-hypercontractive. Then, $d_{\param}(\paren{\mu(\cB),\Sigma(\cB)}, \paren{\mu(\cB'),\Sigma(\cB')}) \leq 1-\eta$.
\end{corollary}
\begin{proof}
By using multiple copies of each points in $Y$ if needed (and thus increasing $n$), we can assume that $\cB,\cB'$ are uniform over (multi)-subset $Z,Z'$ of $Y$ with size $\geq \alpha n$. Set $Z = \cI$ and and let $w$ be the indicate of $Z'$. Then, $\dtv(\cB,\cB') \leq 1-\eta$ implies that $w(\cI) = 1-\eta$. Applying Lemmas~\ref{lem:spectral-distance-LDC},\ref{lem:mean-closeness-main},~\ref{lem:rel-frob-close-main} completes the proof.  \Anote{these are not the right lemmas. }
\end{proof}


\paragraph{Discussion}
We first explain the high-level idea of our pruning algorithm that relies on the corollary above.

The heart of the algorithm is a \emph{verification} subroutine that, given a set of parameters $(\hat{\mu},\hat{\Sigma})$, finds, whenever feasible, a weighting of the input sample $Y$ with close (in $d_{\param}$ distance) to them while being certifiably anti-concentrated and hypercontractive distribution with parameters close to them. We implement this subroutine via a sum-of-squares relaxation of verification constraint system $\cV$.

We use this subroutine as follows: we group the parameters in $\cL$ greedily with respect to the $d_{\param}$ distance. For each group so created, we pick a representative set of parameters $(\mu,\Sigma)$ and run the verification subroutine with them. If the  subroutine returns infeasible, we discard the whole group otherwise, we add the representative to the pruned list.

We show that subroutine is always feasible when run on any member of a group that contains a $(\hat{\mu},\hat{\Sigma})$ that are close to $\mu_*, \Sigma_*$. Further, since the subroutine is run with parameters that are pairwise far (in $d_{\param}$) from each other, Corollary~\ref{cor:distilled-tv-to-param} implies that the weights returned by the subroutine define distributions that are pairwise separated in total variation distance. Moreover, the distributions returned by the subroutine cannot give too much weight to any single sample (i.e. have high min-entropy). In Lemma~\ref{lem:TV-packing} we prove a ``packing lemma'' for distributions supported on the same set that are high min entropy which implies that there cannot be more than $O(1/\alpha)$ such distributions. Thus, in the above process, the rounded sets of parameters are a set of size at most $O(1/\alpha)$.

\paragraph{Constraint System}

The heart of our pruning algorithm is a subroutine that takes input a pair of parameters $\hat{\mu}, \hat{\Sigma}$ and tests if there's  a nice distribution (Definition~\ref{def:nice_distribution}) can be supported on a subsample of the input with mean and covariance close to $\hat{\mu}, \hat{\Sigma}$. When the test accepts it outputs a certificate - in the form of weights on the input  sample that form  such a distribution.

This subroutine is based on finding a pseudo-distribution consistent with a constraint system $\cV(\hat{\mu},\hat{\Sigma})$ closely related to $\cA$ along with a new set of parameter distance constraints $\cV_1$.  %and modifying $\cA$ in terms of the input $\hat{\mu}$ and $\hat{\Sigma}$. $\cA_6(\hat{\mu},\hat{\Sigma})$ depends on a known set of parameters $\hat{\mu},\hat{\Sigma}$ and forces the indeterminate parameters $\mu,\Sigma$ in the system to be appropriately close to $\hat{\mu}$ and $\hat{\Sigma}$ respectively.

Next, we show how to modify the constraints in $\cV$ for our pruning algorithm.

Our constraints resemble $\cV$ in form - but unlike $\cV$, note that the only indeterminates in the formulation below are $w_i$s. The  other indeterminates such as $\mu,\Sigma$ present in $\cV$ before are instantiated by known constants $\hat{\Sigma}$ and $\hat{\mu}$ here.

% \begin{equation}
% \text{Covariance Constraints: $\cA_1$} = %  \cA_{w,\Pi}\colon
%   \left \{
%     \begin{aligned}
%       &
%       &\Theta, \Pi
%       &\succeq 0\\
%       &
%       &\Theta \Pi = \Pi \Theta
%       &= I\\
%       &
%       &\Pi^2
%       &=\hat{\Sigma}\\
%       &
%       &\Theta^2\Sigma  = \Sigma \Theta^2
%       &=\Theta\Sigma\Theta =I\\
%     \end{aligned}
%   \right \}
% \end{equation}

\begin{equation}
\text{Parameter Distance Constraints: $\cV_1$} = %  \cA_{w,\Pi}\colon
  \left \{
    \begin{aligned}
      &
      &\Norm{\hat{\Sigma}^{-1/2}(\hat{\mu}-\mu)}^2_2
      &\leq  \\
      &
      &\Norm{\hat{\Sigma}^{-1/2} \Sigma \hat{\Sigma}^{-1/2}-I}_F^2
      &\leq \\
      &\forall v
      &v^{\top} \hat{\Sigma}^{-1/2} \Sigma \hat{\Sigma}^{-1/2}v
      &\geq \\
    \end{aligned}
  \right \}
\end{equation}

\begin{equation}
\text{Intersection Constraints: $\cV_2$} = %  \cA_{w,\Pi}\colon
  \left \{
    \begin{aligned}
      &\forall i\in [n].
      & w_i^2
      & = w_i\\
      &&
      \textstyle\sum_{i\in[n]} w_i
      &= \alpha n\\
    \end{aligned}
  \right \}
\end{equation}


\begin{equation}
\text{Parameter Constraints: $\cV_3$} = %  \cA_{w,\Pi}\colon
  \left \{
    \begin{aligned}
      &
      &\Norm{\hat{\Sigma}^{-1/2} \mu-\frac{1}{\alpha n}\sum_{i = 1}^n w_i\hat{\Sigma}^{-1/2} y_i}_2^2
      & \leq  s(\eta/2)^2/\eta^2\\
      &\alpha^2/s(\eta/2) \hat{\Sigma}
      &\preceq \frac{1}{\alpha n}\sum_{i = 1}^n w_i \Paren{y_i-\hat{\mu}} \Paren{y_i-\hat{\mu}}^{\top}
      &\preceq s(\eta/2) \alpha^{-2} \hat{\Sigma}\\
      % &
      % &\lambda_u I - \Sigma
      % &\succeq 0\\
      % &
      % &\Sigma-\lambda_l I
      % &\succeq 0\\
      % &
      % &\lambda^{1/2}_u I - \Pi
      % &\succeq 0\\
      % &
      % &\Pi-\lambda^{1/2}_l I
      % &\succeq 0\\
      % &
      % &\lambda^{-1/2}_l I - \Theta
      % &\succeq 0\\
      % &
      % &\Theta-\lambda_u^{-1/2} I
      % &\succeq 0\\
    \end{aligned}
  \right \}
\end{equation}


\begin{equation}
 \text{Certifiable Anti-Concentration: }\cV_4 =% \cA_{w,\Pi}\colon
  \left \{
    \begin{aligned}
      &
      &\frac{1}{\alpha n}\sum_{i \leq [n]} w_i p_{\cD}^2 \Paren{\Iprod{\hat{\Sigma}^{-1/2}(x_i - \hat{\mu}),v}}
      &\leq C\delta \norm{v}_2^{2t}\\
     \end{aligned}
    \right\}
 \end{equation}


\begin{equation}
\label{eqn:prune_cert_hypercontractive}
 \text{Certifiable Hyper-contractivity :}\cA_5 = %\cA_{w,\Pi}\colon
  \left \{
    \begin{aligned}
     &
     &\frac{1}{\alpha n} \sum_{i \leq [n]} w_i \Paren{ \Iprod{\Paren{\hat{\Sigma}^{-1/2} (x_i-\hat{\mu})}\Paren{\hat{\Sigma}^{-1/2} {x_i - \hat{\mu}}^{\top}},Q }}^{2h}
     &\leq \Paren{Ch}^h \Norm{Q}_F^{2h}
    \end{aligned}
  \right \}
\end{equation}



\begin{equation}
\label{eqn:prune_param_dist}
\text{Parameter Distance Constraints: $\cA_6$} = %  \cA_{w,\Pi}\colon
  \left \{
    \begin{aligned}
      &
      &\Norm{\hat{\Sigma}^{-1/2}(\hat{\mu}-\mu)}^2_2
      &\leq  \\
      &
      &\Norm{\hat{\Sigma}^{-1/2} \Sigma \hat{\Sigma}^{-1/2}-I}_F^2
      &\leq \\
      &\forall v
      &v^{\top} \hat{\Sigma}^{-1/2} \Sigma \hat{\Sigma}^{-1/2}v
      &\geq \\
    \end{aligned}
  \right \}
\end{equation}

%\Pnote{Need all the other constraints in terms of $\hat{\mu}$ and $\hat{\Sigma}$ and need to be linear in $w$.}

% \begin{lemma}
% Let $\tzeta$ be a pseudo-distribution of degree $$ consistent with $\cA_{\pr}(\hat{\mu},\hat{\Sigma})$.
% Consider the distribution on
% \end{lemma}

% \begin{lemma}[TV Distance vs Parameter Distance via Moments] \label{lem:analysis-of-rounding-of-pruning-SDP}
% Let $X$ be a good sample of size $n$.
% Let $\tzeta$ be a pseudo-distribution consistent with $\cA_{\pr}(\hat{\mu},\hat{\Sigma})$.
% Let $\hw_i = \pE_{\tzeta}[w_i]$ for each $i$, $\mu_{out} = \pE_{\tzeta}[\mu]$ and $\Sigma_{out} = \pE_{\tzeta}[\Sigma]$.
% Then,
% \begin{enumerate}
%   \item $\frac{k}{n} \sum_{i \leq n} \hw_i x_i = \mu_{out}$.
%   \item $\frac{k}{n} \sum_{i \leq n} \hw_j (x_i-\mu_{out})(x_i - \mu_{out})^{\top} = \Sigma_{out}$.
%   \item $\frac{k}{n}\sum_{i \leq n} \hw_i p_{\cD}^2 (\Iprod{x_i-\mu_{out},v}) \leq C\delta$.
%   \item $\frac{k}{n} \sum_{i \leq n} \hw_i \Iprod{(x_i-\mu_{out})(x_i - \mu_{out})^{\top} ,Q}^{2h} \leq ??  \Trace(\hat{\Sigma} \cdot Q}$
%   \item $d_{\param}((\hat{\mu},\hat{\Sigma}), (\mu_{out}, \Sigma_{out})\leq 1-\alpha^{10}$.
% \end{enumerate}
% \end{lemma}

% \begin{proof}
% \[
% \frac{1}{\alpha n} \sum_{i = 1}^n  w_i w_i' \iprod{\Sigma^{-1/2} x_i,v}^2 \geq \delta^2 \norm{\Sigma^{1/2} v}^2 \Paren{\frac{1}{n} \sum_{i = 1}^n w_i - C\delta}
% \]
% \end{proof}
The following two claims analyze our testing algorithm based on pseudo-distributions satisfying $\cA_{\pr}$.


The following lemma follows by  direct computation and checks that $\cI$ satisfies $\cV$ if $d_{\param}( \paren{\hat{\mu}, \hat{\Sigma}}, \paren{\mu_*,\Sigma_*}) \leq 1-\eta$.

\begin{lemma}[Constraints are Feasible for Parameters Close to Inliers]
Suppose $d_{\param}( \paren{\hat{\mu}, \hat{\Sigma}}, \paren{\mu_*,\Sigma_*}) \leq 1-\eta$. Then, $X' = \cI$ satisfies $\cV$. \label{lem:close-to-inliers-means-feasible}
\end{lemma}

The next lemma shows that a pseudo-distribution $\tzeta$ satisfying $\cV$ can be rounded to give a nice distribution with parameters close to $\hat{\mu},\hat{\Sigma}$.

\begin{lemma}[Rounded Distributions are Nice]
Let $\tzeta$ be a pseudo-distribution of degree consistent with $\cV$.
Round $\tzeta$ to give: $\hw(i) = \pE_{\tzeta}[w_i]$ for each $i$.
Then, $\hw_i$ defines a probability distribution $\cB$ on the input sample with mean $\mu$ and covariance $\Sigma$ satisfying:
\begin{enumerate}
\item $d_{\param}( \paren{\hat{\mu},\hat{\Sigma}},\paren{\mu,\Sigma}) \leq 1-\eta$.
\item $\cB$ is certifiably anti-concentrated and has certifiably hypercontractive degree 2 polynomials.
\end{enumerate}  \label{lem:rounding-produces-nice-dist}
\end{lemma}
\begin{proof}
Observe that our rounding simply returns $\hw_i = \pE_{\tzeta}[w_i]$. The main observation underlying the proof is that the constraints in our formulation are linear in the variables $w_i$.
\end{proof}


The last ingredient in the analysis of our pruning algorithm is the following result that shows that our testing algorithm can only be feasible for an $O(1/\alpha)$ invocations in our pruning algorithm.

\begin{lemma}[Packing Distributions with High Pairwise TV-Distance] \label{lem:TV-packing}
Let $D_1, D_2, \ldots, D_k$ be probability distributions supported on $Y = \Set{y_1, y_2, \ldots, y_n}$ such that
\begin{enumerate}
\item $\Pr_{D_j}[ y_i] \leq \alpha$ for every $i,j$, and,
\item $\dtv(D_i,D_j)>1-\alpha^2/20$ for every $i \neq j$.
\end{enumerate}
Then, $k \leq 2/\alpha$.
\end{lemma}

Given the three claims above, it is easy to complete the analysis of our pruning algorithm.
\begin{proof}[Proof of Lemma~\ref{lem:analysis-of-rounding-of-pruning-SDP}]

\end{proof}



\begin{proof}[Proof of Lemma~\ref{lem:TV-packing}]
Observe that if in addition, each $D_i$ is uniform over a subset $S_i$ of $Y$, then, $\dtv(D_i,D_j)>1-\alpha^2/10$ implies that for each $i \neq j$,  $|S_i \cap S_j| \leq \alpha^2/10 \min\{|S_i|,|S_j|\}$. Applying Lemma~\ref{lem:set-packing} then finishes the proof. We will now use this special case to argue the lemma in its generality.

Suppose now, for the sake of contradiction, there exists $D_1, D_2, \ldots, D_k$ satisfying the two conditions in the lemma statement above and that further $k > 2/\alpha$. Choose $r= \lceil (100/\alpha^2)n\rceil$ and consider $Y'$, the multiset of $nr$ points obtained by taking $r$ copies of each point in $Y$. For each $D_i$, build a multi-subset $S_i$ as follows: for each element $y_j$, include $c_j = \lceil D_i(y_j)/(r\alpha) \rceil$ copies of $y_j$ in $S_i$. Consider the uniform distribution $D_i'$ on $S_i$. Then by direct computation $\dtv(D_i,D_i')<\alpha^2/20$. Furthere, for each $i$, $|S_i| > \alpha  nr$.

Now, consider the distributions $D_1',D_2',\ldots, D_k'$. For each $i \neq j$, we must have $\dtv(D_i',D_j') \geq \dtv(D_i,D_j) - \dtv(D_i',D_i) - \dtv(D_j',D_j)\geq 1-\alpha^2/10$ thus yielding a contradiction if $k > 2/\alpha$. This finishes the proof.
\end{proof}

\begin{lemma}[Packing Sets with Low Pairwise Intersection]
Let $S_1, S_2, \ldots, S_k \subseteq [n]$ be sets of size $\geq \alpha n$ for each $i$ satisfying $|S_i \cap S_j| \leq \frac{1}{4}\alpha^2 \min\{|S_i|,|S_j|\}$. Then, $k \leq 2/\alpha$. \label{lem:set-packing}
\end{lemma}

\begin{proof}
%Since each set is of size at least $\alpha n$ and at most $n$, for any $i,j$, $\alpha |S_i| \leq |S_j| \leq \frac{1}{\alpha} |S_i|$.
The hypothesis implies that for every $i,j$, $|S_j \cap S_i| \leq \frac{1}{10}\alpha^2 n$.
Suppose $k>2/\alpha$. Take the first $k'=2/\alpha$ sets and observe that $n \geq |S_1 \cup S_2 \cup \cdots S_{k'}| \geq \sum_{j = 1}^{k'} |S_j| - \Paren{\sum_{i < j} |S_j\cap S_i|} \geq k'\alpha n- k'^2 \alpha^2n = 2n-(4/\alpha^2) \frac{\alpha^2}{10}n>1.5n$ yielding a contradiction.
\end{proof}



% \begin{lemma}[General Packing]
% Let $D_1, D_2, \ldots, D_k$ be probability distributions and let $Y = \Set{y_1, y_2, \ldots, y_n}$ be a fixed set of points such that $\Pr_{x \sim D_i}[ x \in Y] = \alpha$ for each $i$. Suppose  further that:
% \begin{enumerate}
% \item $\Pr_{D_j}[ y_i] \leq \frac{1}{\alpha n}$ for every $i,j$, and,
% \item $\dtv(D_i,D_j)>1-\alpha^4/400$ for every $i \neq j$.
% \end{enumerate}
% Then, $k \leq 2/\alpha^2$.
% \end{lemma}

% \begin{proof}
% By definition of Total Variation Distance,
% \[\dtv(D_i,D_j) = \frac{1}{2} \sum_{x \in Y} |D_i(x) - D_j(x)| + \frac{1}{2} \sum_{x \not \in Y} |D_i(x) - D_i(y)|
% \]
% Observe, the second term above can be bounded as follows:
% \[
% \frac{1}{2} \sum_{x \not \in Y} |D_i(x) - D_i(y)| \leq \frac{1}{2} \sum_{x \not \in Y} D_i(x) + D_i(y) = 1-\alpha
% \]
% Thus, for every $i \neq j$,
% \begin{equation}
% \frac{1}{2} \sum_{x \in Y} |D_i(x) - D_j(x)| \geq 1-\alpha^4/400 - (1-\alpha) = \alpha(1- \alpha^{2}/20) \mper\label {eq:TV-bound-conditional}
% \end{equation}
% Let $D_i'$ be the distribution obtained by conditioning $D_i$ to output a sample in $Y$.
% Then, from \eqref{eq:TV-bound-conditional},
% \[
% \dtv(D_i',D_j') = \frac{1}{2} \sum_{x \in Y} |D_i(x)/\alpha - D_j(x)/\alpha| \geq 1-\alpha^2/20 \mper
% \]
% We can now apply Lemma~\ref{lem:TV-packing} to conclude that $k \leq 2/\alpha$. This completes the proof.

% \end{proof}
% \Pnote{check bound here. Weird that it's $2/\alpha$ and not $2/\alpha^2$ somehow.}


==> content/setup.tex <==
%!TEX root = ../main.tex

%\section{Our Results} 


==> preamble/macros-custom.tex <==
% algorithm packages


%\usepackage{algorithmic}
%\usepackage{algorithm}
%\usepackage{algpseudocode}

%\algnewcommand\algorithmicinput{\textbf{Input:}}
%\algnewcommand\INPUT{\item[\algorithmicinput]}
%\algnewcommand\algorithmicoutput{\textbf{Output:}}
%\algnewcommand\OUTPUT{\item[\algorithmicoutput]}

% paper-specific packages
\usepackage{relsize}
\usepackage[font=footnotesize]{caption}
\usepackage{appendix}


% abbreviations and paper-specific macros

% math
\newcommand{\D}{\mathcal{D}}
\newcommand{\zo}{\{0,1\}}
\newcommand{\on}{\{-1,1\}}
\newcommand{\sphere}{\bbS^{n-1}}
\DeclareMathOperator{\Span}{Span}
\DeclareMathOperator{\im}{im}
\DeclareMathOperator{\lamax}{\lambda_{\mathrm{max}}}
\newcommand{\Sn}{\mathbb{S}^{n-1}}
\DeclareMathOperator{\Id}{\mathrm{Id}}
\DeclareMathOperator{\F}{\mathbb{F}}
\DeclareMathOperator{\codim}{codim}


% not math
\DeclareUrlCommand\email{}
\newcommand{\whp}{\text{w.h.p.}}
\newcommand{\wovp}{\text{w.ov.p.}\xspace}
\newcommand{\YES}{\textsc{yes}\xspace}
\newcommand{\NO}{\textsc{no}\xspace}

\newcommand{\wovple}{\hspace{-3mm}\stackrel{\text{\wovp}}{\le}}
\newcommand{\wovpeq}{\hspace{-3mm}\stackrel{\text{\wovp}}{=}}
\newcommand{\wovpge}{\hspace{-3mm}\stackrel{\text{\wovp}}{\ge}}
\newcommand{\aasle}{\hspace{-1.5mm}\stackrel{\text{a.a.s.}}\le}

\newcommand{\Pisymm}{\Pi_{\mathrm{symm}}}
\newcommand{\Pisym}{\Pi_{\mathrm{sym}}}

%added by TM
\newcommand{\inner}[1]{\langle #1 \rangle}
\newcommand{\sosle}{\preceq}
\newcommand{\sosge}{\succeq}

\DeclareMathOperator{\tE}{\tilde{\mathbb E}}
\DeclareMathOperator{\tO}{\tilde{O}}
\newcommand{\ta}{\tilde{a}}
\newcommand{\tA}{\tilde{A}}


\DeclareMathOperator*{\pE}{\tilde{\mathbb E}}

\newcommand{\bT}{\mathbf{T}}
\newcommand{\ot}{\otimes}
\newcommand{\tr}{\textup{tr}}
\newcommand{\diag}{\textup{diag}}

\let\pref=\prettyref

% transpose
% http://tex.stackexchange.com/questions/204892/visually-appealing-subscripts-with-intercal
% http://tex.stackexchange.com/questions/30619/what-is-the-best-symbol-for-vector-matrix-transpose
\newcommand*{\transpose}[1]{{#1}{}^{\mkern-4mu\intercal}}
\newcommand*{\vardyad}[1]{#1^{\vphantom{\intercal}}#1^{\intercal}}
\newcommand*{\dyad}[1]{#1#1{}^{\mkern-4mu\intercal}}

% \let\Id\undefined
% \newcommand*{\Id}{I}

% span of subspace -- temporary

\newcommand{\sspan}{\textup{span}}
\newcommand{\1}{\bm{1}}

\newcommand{\Cov}{\mathop{\mathrm{Cov}}}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../planted"
%%% End:


==> preamble/macros.tex <==
% {{{ etex }}}

\usepackage{etex}

% {{{ nag }}}

\usepackage[l2tabu, orthodox]{nag}

% {{{ common }}}

\usepackage{xspace,enumerate}

\usepackage[dvipsnames]{xcolor}

\usepackage[T1]{fontenc}
\usepackage[full]{textcomp}

% {{{ babelamerican }}}
\usepackage[american]{babel}

% {{{ mathtools }}}

\usepackage{mathtools}


% {{{ boldmath }}}

% fix for "too many math alphabets" problem
\newcommand\hmmax{0} % default 3
% \usepackage{bm}

% \usepackage{stmaryrd}


% {{{ amsthm }}}
\usepackage{amsthm}

\newtheorem{theorem}{Theorem}[section]
\newtheorem*{theorem*}{Theorem}

\newtheorem{subclaim}{Claim}[theorem]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem*{proposition*}{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem*{lemma*}{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem*{conjecture*}{Conjecture}
\newtheorem{fact}[theorem]{Fact}
\newtheorem*{fact*}{Fact}
\newtheorem{hypothesis}[theorem]{Hypothesis}
\newtheorem*{hypothesis*}{Hypothesis}
\newtheorem{conjecture}[theorem]{Conjecture}


\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{construction}[theorem]{Construction}
\newtheorem{example}[theorem]{Example}
\newtheorem{question}[theorem]{Question}
\newtheorem{openquestion}[theorem]{Open Question}
\newtheorem{algorithm}[theorem]{Algorithm}
\newtheorem{problem}[theorem]{Problem}
\newtheorem{protocol}[theorem]{Protocol}
\newtheorem{assumption}[theorem]{Assumption}

\theoremstyle{remark}
\newtheorem{claim}[theorem]{Claim}
\newtheorem*{claim*}{Claim}
\newtheorem{remark}[theorem]{Remark}
\newtheorem*{remark*}{Remark}
\newtheorem{observation}[theorem]{Observation}
\newtheorem*{observation*}{Observation}



% {{{ geometry-nice }}}


\ifnum\writemode=1
\usepackage[
letterpaper,
top=1.2in,
bottom=1.2in,
left=1in,
right=1in]{geometry}

\pagestyle{empty}
\fi

\ifnum\writemode=0
\usepackage[
letterpaper,
top=0.7in,
bottom=0.9in,
left=1in,
right=1in]{geometry}
\fi

% {{{ fonts }}}

\usepackage{newpxtext} % T1, lining figures in math, osf in text
\usepackage{textcomp} % required for special glyphs
\usepackage[varg,bigdelims]{newpxmath}
\usepackage[scr=rsfso]{mathalfa}% \mathscr is fancier than \mathcal
\usepackage{bm} % load after all math to give access to bold math
% \useosf %no longer needed
\linespread{1.1}% Give Palatino more leading (space between lines)
\let\mathbb\varmathbb

% {{{ showkeys }}}

\ifnum\showkeys=1
\usepackage[color]{showkeys}
\fi

% {{{ hyperref-option2 }}}

\ifnum\showcolorlinks=1
\usepackage[
pagebackref,
% letterpaper=true,
colorlinks=true,
urlcolor=blue,
linkcolor=blue,
citecolor=OliveGreen,
]{hyperref}
\fi

\ifnum\showcolorlinks=0
\usepackage[
pagebackref,
% letterpaper=true,
colorlinks=false,
pdfborder={0 0 0}
]{hyperref}
\fi


\usepackage[capitalise,nameinlink]{cleveref}
\crefname{lemma}{Lemma}{Lemmas}
\crefname{definition}{Definition}{Definitions}

% {{{ prettyref }}}

% \usepackage{prettyref}

% % From manual:
% % \newrefformat{eq}{\textup{(\ref{#1})}}
% % \newrefformat{lem}{Lemma~\ref{#1}}
% % \newrefformat{thm}{Theorem~\ref{#1}}
% % \newrefformat{cha}{Chapter~\ref{#1}}
% % \newrefformat{sec}{Section~\ref{#1}}
% % \newrefformat{tab}{Table~\ref{#1} on page~\pageref{#1}}
% % \newrefformat{fig}{Figure~\ref{#1} on page~\pageref{#1}}

% \newcommand{\savehyperref}[2]{\texorpdfstring{\hyperref[#1]{#2}}{#2}}

% \newrefformat{eq}{\savehyperref{#1}{\textup{(\ref*{#1})}}}
% \newrefformat{eqn}{\savehyperref{#1}{\textup{(\ref*{#1})}}}
% \newrefformat{lem}{\savehyperref{#1}{Lemma~\ref*{#1}}}
% \newrefformat{def}{\savehyperref{#1}{Definition~\ref*{#1}}}
% \newrefformat{thm}{\savehyperref{#1}{Theorem~\ref*{#1}}}
% \newrefformat{cor}{\savehyperref{#1}{Corollary~\ref*{#1}}}
% \newrefformat{cha}{\savehyperref{#1}{Chapter~\ref*{#1}}}
% \newrefformat{sec}{\savehyperref{#1}{Section~\ref*{#1}}}
% \newrefformat{app}{\savehyperref{#1}{Appendix~\ref*{#1}}}
% \newrefformat{tab}{\savehyperref{#1}{Table~\ref*{#1}}}
% \newrefformat{fig}{\savehyperref{#1}{Figure~\ref*{#1}}}
% \newrefformat{hyp}{\savehyperref{#1}{Hypothesis~\ref*{#1}}}
% \newrefformat{alg}{\savehyperref{#1}{Algorithm~\ref*{#1}}}
% \newrefformat{rem}{\savehyperref{#1}{Remark~\ref*{#1}}}
% \newrefformat{item}{\savehyperref{#1}{Item~\ref*{#1}}}
% \newrefformat{step}{\savehyperref{#1}{step~\ref*{#1}}}
% \newrefformat{conj}{\savehyperref{#1}{Conjecture~\ref*{#1}}}
% \newrefformat{fact}{\savehyperref{#1}{Fact~\ref*{#1}}}
% \newrefformat{prop}{\savehyperref{#1}{Proposition~\ref*{#1}}}
% \newrefformat{prob}{\savehyperref{#1}{Problem~\ref*{#1}}}
% \newrefformat{claim}{\savehyperref{#1}{Claim~\ref*{#1}}}
% \newrefformat{relax}{\savehyperref{#1}{Relaxation~\ref*{#1}}}
% \newrefformat{red}{\savehyperref{#1}{Reduction~\ref*{#1}}}
% \newrefformat{part}{\savehyperref{#1}{Part~\ref*{#1}}}



% {{{ sref }}}

% short section reference
\newcommand{\Sref}[1]{\hyperref[#1]{\S\ref*{#1}}}

% {{{ nicefrac }}}
% commands for fractions
\usepackage{nicefrac}
% poor man's fraction
\newcommand{\flatfrac}[2]{#1/#2}
\newcommand{\varflatfrac}[2]{#1\textfractionsolidus#2}

\let\nfrac=\nicefrac
\let\ffrac=\flatfrac
% similar commands: tfrac,dfrac

\newcommand{\half}{\nicefrac12}
\newcommand{\onequarter}{\nicefrac14}
\newcommand{\threequarter}{\nicefrac34}

% {{{ microtype-option }}}

\ifnum\usemicrotype=1
\usepackage{microtype}
\fi

% {{{ authornotes }}}
\ifnum\showauthornotes=1
\newcommand{\Authornote}[2]{{\sffamily\small\color{red}{[#1: #2]}}}
\newcommand{\Authornotecolored}[3]{{\sffamily\small\color{#1}{[#2: #3]}}}
\newcommand{\Authorcomment}[2]{{\sffamily\small\color{gray}{[#1: #2]}}}
\newcommand{\Authorstartcomment}[1]{\sffamily\small\color{gray}[#1: }
\newcommand{\Authorendcomment}{]\rmfamily\normalsize\color{black}}
\newcommand{\Authorfnote}[2]{\footnote{\color{red}{#1: #2}}}
\newcommand{\Authorfixme}[1]{\Authornote{#1}{\textbf{??}}}
\newcommand{\Authormarginmark}[1]{\marginpar{\textcolor{red}{\fbox{\Large #1:!}}}}
\else
\newcommand{\Authornote}[2]{}
\newcommand{\Authornotecolored}[3]{}
\newcommand{\Authorcomment}[2]{}
\newcommand{\Authorstartcomment}[1]{}
\newcommand{\Authorendcomment}{}
\newcommand{\Authorfnote}[2]{}
\newcommand{\Authorfixme}[1]{}
\newcommand{\Authormarginmark}[1]{}
\fi

\newcommand{\Dnote}{\Authornote{D}}
%\newcommand{\Tnote}{\Authornotecolored{blue}{T}}
\newcommand{\TMnote}{\Authornotecolored{blue}{T}}
\newcommand{\Inote}{\Authornotecolored{ForestGreen}{I}}
\newcommand{\inote}{\Inote}
\newcommand{\Gnote}{\Authornote{G}}
\newcommand{\Jcomment}{\Authorcomment{J}}
\newcommand{\Dcomment}{\Authorcomment{D}}
\newcommand{\Dstartcomment}{\Authorstartcomment{D}}
\newcommand{\Dendcomment}{\Authorendcomment}
\newcommand{\Dfixme}{\Authorfixme{D}}
\newcommand{\Dmarginmark}{\Authormarginmark{D}}
\newcommand{\Dfnote}{\Authorfnote{D}}

\newcommand{\Pnote}{\Authornote{P}}
\newcommand{\Pfnote}{\Authorfnote{P}}

\newcommand{\PRnote}{\Authornote{PR}}
\newcommand{\PRfnote}{\Authorfnote{PR}}

\newcommand{\PTnote}{\Authornote{PT}}
\newcommand{\PTfnote}{\Authorfnote{PT}}

\newcommand{\PGnote}{\Authornote{PG}}
\newcommand{\PGfnote}{\Authorfnote{PG}}

\newcommand{\Bnote}{\Authornote{B}}
\newcommand{\Bfnote}{\Authorfnote{B}}

\definecolor{forestgreen(traditional)}{rgb}{0.0, 0.27, 0.13}
\newcommand{\Jnote}{\Authornotecolored{forestgreen(traditional)}{J}}
\newcommand{\Jfnote}{\Authorfnote{J}}


\newcommand{\Mnote}{\Authornote{M}}
\newcommand{\Mfnote}{\Authorfnote{M}}

\newcommand{\Rnote}{\Authornote{M}}
\newcommand{\Rfnote}{\Authorfnote{M}}

\newcommand{\Nnote}{\Authornote{N}}
\newcommand{\Nfnote}{\Authorfnote{N}}

\newcommand{\Snote}{\Authornote{S}}
\newcommand{\Sfnote}{\Authorfnote{S}}


% {{{ fixme }}}

% place red exclamation mark in margin
%\newcommand{\redmarginmarker}{\marginpar{\textcolor{red}{\fbox{\Large !}}}}
\newcommand{\redmarginmarker}{}

% short indicator for places that need fixing
\newcommand{\FIXME}{\textbf{\textcolor{red}{??}}\redmarginmarker}

\ifnum\showfixme=0
\renewcommand{\FIXME}{}
\fi


% {{{ boxedminipage }}}
\usepackage{boxedminipage}

\newenvironment{mybox}
{\center \noindent\begin{boxedminipage}{1.0\linewidth}}
{\end{boxedminipage}
\noindent
}


% {{{ parentheses }}}
% various bracket-like commands
% round parentheses
\newcommand{\paren}[1]{(#1)}
\newcommand{\Paren}[1]{\left(#1\right)}
\newcommand{\bigparen}[1]{\big(#1\big)}
\newcommand{\Bigparen}[1]{\Big(#1\Big)}
% square brackets
\newcommand{\brac}[1]{[#1]}
\newcommand{\Brac}[1]{\left[#1\right]}
\newcommand{\bigbrac}[1]{\big[#1\big]}
\newcommand{\Bigbrac}[1]{\Big[#1\Big]}
\newcommand{\Biggbrac}[1]{\Bigg[#1\Bigg]}
% absolute value
\newcommand{\abs}[1]{\lvert#1\rvert}
\newcommand{\Abs}[1]{\left\lvert#1\right\rvert}
\newcommand{\bigabs}[1]{\big\lvert#1\big\rvert}
\newcommand{\Bigabs}[1]{\Big\lvert#1\Big\rvert}
% cardinality
\newcommand{\card}[1]{\lvert#1\rvert}
\newcommand{\Card}[1]{\left\lvert#1\right\rvert}
\newcommand{\bigcard}[1]{\big\lvert#1\big\rvert}
\newcommand{\Bigcard}[1]{\Big\lvert#1\Big\rvert}
% set
\newcommand{\set}[1]{\{#1\}}
\newcommand{\Set}[1]{\left\{#1\right\}}
\newcommand{\bigset}[1]{\big\{#1\big\}}
\newcommand{\Bigset}[1]{\Big\{#1\Big\}}
% norm
\newcommand{\norm}[1]{\lVert#1\rVert}
\newcommand{\Norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\bignorm}[1]{\big\lVert#1\big\rVert}
\newcommand{\Bignorm}[1]{\Big\lVert#1\Big\rVert}
\newcommand{\Biggnorm}[1]{\Bigg\lVert#1\Bigg\rVert}
% 2-norm
\newcommand{\normt}[1]{\norm{#1}_2}
\newcommand{\Normt}[1]{\Norm{#1}_2}
\newcommand{\bignormt}[1]{\bignorm{#1}_2}
\newcommand{\Bignormt}[1]{\Bignorm{#1}_2}
% 2-norm squared
\newcommand{\snormt}[1]{\norm{#1}^2_2}
\newcommand{\Snormt}[1]{\Norm{#1}^2_2}
\newcommand{\bigsnormt}[1]{\bignorm{#1}^2_2}
\newcommand{\Bigsnormt}[1]{\Bignorm{#1}^2_2}
% norm squared
\newcommand{\snorm}[1]{\norm{#1}^2}
\newcommand{\Snorm}[1]{\Norm{#1}^2}
\newcommand{\bigsnorm}[1]{\bignorm{#1}^2}
\newcommand{\Bigsnorm}[1]{\Bignorm{#1}^2}
% 1-norm
\newcommand{\normo}[1]{\norm{#1}_1}
\newcommand{\Normo}[1]{\Norm{#1}_1}
\newcommand{\bignormo}[1]{\bignorm{#1}_1}
\newcommand{\Bignormo}[1]{\Bignorm{#1}_1}
% infty-norm
\newcommand{\normi}[1]{\norm{#1}_\infty}
\newcommand{\Normi}[1]{\Norm{#1}_\infty}
\newcommand{\bignormi}[1]{\bignorm{#1}_\infty}
\newcommand{\Bignormi}[1]{\Bignorm{#1}_\infty}
% inner product
\newcommand{\iprod}[1]{\langle#1\rangle}
\newcommand{\Iprod}[1]{\left\langle#1\right\rangle}
\newcommand{\bigiprod}[1]{\big\langle#1\big\rangle}
\newcommand{\Bigiprod}[1]{\Big\langle#1\Big\rangle}


% {{{ probability }}}
% expectation, probability, variance
\newcommand{\Esymb}{\mathbb{E}}
\newcommand{\Psymb}{\mathbb{P}}
\newcommand{\Vsymb}{\mathbb{V}}

\DeclareMathOperator*{\E}{\Esymb}
\DeclareMathOperator*{\Var}{\Vsymb}
\DeclareMathOperator*{\ProbOp}{\Psymb}

\renewcommand{\Pr}{\ProbOp}

% TODO: make case distinction if optional argument is not set
\newcommand{\prob}[1]{\Pr\set{#1}}
\newcommand{\Prob}[2][]{\Pr_{{#1}}\Set{#2}}

\newcommand{\ex}[1]{\E\brac{#1}}
\newcommand{\Ex}[2][]{\E_{{#1}}\Brac{#2}}
\newcommand{\varex}[1]{\E\paren{#1}}
\newcommand{\varEx}[1]{\E\Paren{#1}}

%\newcommand{\given}{\;\middle\vert\;}
\newcommand{\given}{\mathrel{}\middle\vert\mathrel{}}
%\newcommand{\given}{\mathrel{}\middle|\mathrel{}}

% {{{ mathfonts }}}

% \usepackage{dsfont}
% \usepackage{yfonts}
% \usepackage{mathrsfs}


% {{{ miscmacros }}}

% middle delimiter in the definition of a set
\newcommand{\suchthat}{\;\middle\vert\;}

% tensor product
\newcommand{\tensor}{\otimes}

% add explanations to math displays
\newcommand{\where}{\text{where}}
\newcommand{\textparen}[1]{\text{(#1)}}
\newcommand{\using}[1]{\textparen{using #1}}
\newcommand{\smallusing}[1]{\text{(\small using #1)}}
\ifx\because\undefined
\newcommand{\because}[1]{\textparen{because #1}}
\else
\renewcommand{\because}[1]{\textparen{because #1}}
\fi
\newcommand{\by}[1]{\textparen{by #1}}


% spectral order (Loewner order)
\newcommand{\sge}{\succeq}
\newcommand{\sle}{\preceq}

% smallest and largest eigenvalue
\newcommand{\lmin}{\lambda_{\min}}
\newcommand{\lmax}{\lambda_{\max}}

\newcommand{\signs}{\set{1,-1}}
\newcommand{\varsigns}{\set{\pm 1}}
\newcommand{\maximize}{\mathop{\textrm{maximize}}}
\newcommand{\minimize}{\mathop{\textrm{minimize}}}
\newcommand{\subjectto}{\mathop{\textrm{subject to}}}

\renewcommand{\ij}{{ij}}

% symmetric difference
\newcommand{\symdiff}{\Delta}
\newcommand{\varsymdiff}{\bigtriangleup}

% set of bits
\newcommand{\bits}{\{0,1\}}
\newcommand{\sbits}{\{\pm1\}}

% no stupid bullets for itemize environmentx
% \renewcommand{\labelitemi}{--}

% control white space of list and display environments
\newcommand{\listoptions}{\labelsep0mm\topsep-0mm\itemindent-6mm\itemsep0mm}
\newcommand{\displayoptions}[1]{\abovedisplayshortskip#1mm\belowdisplayshortskip#1mm\abovedisplayskip#1mm\belowdisplayskip#1mm}

% short for emptyset
%\newcommand{\eset}{\emptyset}
% moved to mathabbreviations

% short for epsilon
%\newcommand{\e}{\epsilon}
% moved to mathabbreviations

% super index with parentheses
\newcommand{\super}[2]{#1^{\paren{#2}}}
\newcommand{\varsuper}[2]{#1^{\scriptscriptstyle\paren{#2}}}

% tensor power notation
\newcommand{\tensorpower}[2]{#1^{\tensor #2}}


% multiplicative inverse
\newcommand{\inv}[1]{{#1^{-1}}}

% dual element
\newcommand{\dual}[1]{{#1^*}}

% subset
%\newcommand{\sse}{\subseteq}
% moved to mathabbreviations

% vertical space in math formula
\newcommand{\vbig}{\vphantom{\bigoplus}}

% setminus
\newcommand{\sm}{\setminus}

% define something by an equation (display)
\newcommand{\defeq}{\stackrel{\mathrm{def}}=}


% define something by an equation (inline)
\newcommand{\seteq}{\mathrel{\mathop:}=}



% declare function f by $f \from X \to Y$
\newcommand{\from}{\colon}

% big middle separator (for conditioning probability spaces)
\newcommand{\bigmid}{~\big|~}
\newcommand{\Bigmid}{~\Big|~}
\newcommand{\Mid}{\;\middle\vert\;}

% better vector definition and some variations
%\renewcommand{\vec}[1]{{\bm{#1}}}
\newcommand{\bvec}[1]{\bar{\vec{#1}}}
\newcommand{\pvec}[1]{\vec{#1}'}
\newcommand{\tvec}[1]{{\tilde{\vec{#1}}}}

% punctuation at the end of a displayed formula
\newcommand{\mper}{\,.}
\newcommand{\mcom}{\,,}

% inner product for matrices
\newcommand\bdot\bullet

% transpose
\newcommand{\trsp}[1]{{#1}^\dagger}

% indicator function / vector
\ifx\mathds\undefined % use double stroke fonts if available
\DeclareMathOperator{\Ind}{\mathbb{I}}
\else
\DeclareMathOperator{\Ind}{\mathds 1}}
\fi

% place a qed symbol inside display formula
%\qedhere

% {{{ superscripts }}}

\renewcommand{\th}{\textsuperscript{th}\xspace}
\newcommand{\st}{\textsuperscript{st}\xspace}
\newcommand{\nd}{\textsuperscript{nd}\xspace}
\newcommand{\rd}{\textsuperscript{rd}\xspace}


% {{{ mathoperators }}}
\DeclareMathOperator{\Inf}{Inf}
\DeclareMathOperator{\Tr}{Tr}
%\newcommand{\Tr}{\mathrm{Tr}}
\DeclareMathOperator{\SDP}{SDP}
\DeclareMathOperator{\sdp}{sdp}
\DeclareMathOperator{\val}{val}
\DeclareMathOperator{\LP}{LP}
\DeclareMathOperator{\OPT}{OPT}
\DeclareMathOperator{\opt}{opt}
\DeclareMathOperator{\vol}{vol}
\DeclareMathOperator{\poly}{poly}
\DeclareMathOperator{\qpoly}{qpoly}
\DeclareMathOperator{\qpolylog}{qpolylog}
\DeclareMathOperator{\qqpoly}{qqpoly}
\DeclareMathOperator{\argmax}{argmax}
\DeclareMathOperator{\polylog}{polylog}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\dist}{dist}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\conv}{conv}
\DeclareMathOperator{\Conv}{Conv}

\DeclareMathOperator{\rank}{rank}

% operators with limits
\DeclareMathOperator*{\median}{median}
\DeclareMathOperator*{\Median}{Median}

% smaller summation/product symbols
\DeclareMathOperator*{\varsum}{{\textstyle \sum}}
\DeclareMathOperator{\tsum}{{\textstyle \sum}}

\let\varprod\undefined

\DeclareMathOperator*{\varprod}{{\textstyle \prod}}
\DeclareMathOperator{\tprod}{{\textstyle \prod}}




% {{{ differentials }}}

\newcommand{\diffmacro}[1]{\,\mathrm{d}#1}

\newcommand{\dmu}{\diffmacro{\mu}}
\newcommand{\dgamma}{\diffmacro{\gamma}}
\newcommand{\dlambda}{\diffmacro{\lambda}}
\newcommand{\dx}{\diffmacro{x}}
\newcommand{\dt}{\diffmacro{t}}



% {{{ textabbreviations }}}

% some abbreviations
\newcommand{\ie}{i.e.,\xspace}
\newcommand{\eg}{e.g.,\xspace}
\newcommand{\Eg}{E.g.,\xspace}
\newcommand{\phd}{Ph.\,D.\xspace}
\newcommand{\msc}{M.\,S.\xspace}
\newcommand{\bsc}{B.\,S.\xspace}

\newcommand{\etal}{et al.\xspace}

\newcommand{\iid}{i.i.d.\xspace}

% {{{ foreignwords }}}

\newcommand\naive{na\"{\i}ve\xspace}
\newcommand\Naive{Na\"{\i}ve\xspace}
\newcommand\naively{na\"{\i}vely\xspace}
\newcommand\Naively{Na\"{\i}vely\xspace}




% {{{ names }}}
% Hungarian/Polish/East European names
\newcommand{\Erdos}{Erd\H{o}s\xspace}
\newcommand{\Renyi}{R\'enyi\xspace}
\newcommand{\Lovasz}{Lov\'asz\xspace}
\newcommand{\Juhasz}{Juh\'asz\xspace}
\newcommand{\Bollobas}{Bollob\'as\xspace}
\newcommand{\Furedi}{F\"uredi\xspace}
\newcommand{\Komlos}{Koml\'os\xspace}
\newcommand{\Luczak}{\L uczak\xspace}
\newcommand{\Kucera}{Ku\v{c}era\xspace}
\newcommand{\Szemeredi}{Szemer\'edi\xspace}
\newcommand{\Hastad}{H{\aa}stad\xspace}
\newcommand{\Hoelder}{H\"{o}lder\xspace}
\newcommand{\Holder}{\Hoelder}
\newcommand{\Brandao}{Brand\~ao\xspace}


% {{{ numbersets }}}
% number sets
\newcommand{\Z}{\mathbb Z}
\newcommand{\N}{\mathbb N}
\newcommand{\R}{\mathbb R}
\newcommand{\C}{\mathbb C}
\newcommand{\Rnn}{\R_+}
\newcommand{\varR}{\Re}
\newcommand{\varRnn}{\varR_+}
\newcommand{\varvarRnn}{\R_{\ge 0}}


% {{{ problems }}}

% macros to denote computational problems

% use texorpdfstring to avoid problems with hyperref (can use problem
% macros also in headings
\newcommand{\problemmacro}[1]{\texorpdfstring{\textup{\textsc{#1}}}{#1}\xspace}

\newcommand{\pnum}[1]{{\footnotesize #1}}

% list of problems
\newcommand{\uniquegames}{\problemmacro{unique games}}
\newcommand{\maxcut}{\problemmacro{max cut}}
\newcommand{\multicut}{\problemmacro{multi cut}}
\newcommand{\vertexcover}{\problemmacro{vertex cover}}
\newcommand{\balancedseparator}{\problemmacro{balanced separator}}
\newcommand{\maxtwosat}{\problemmacro{max \pnum{3}-sat}}
\newcommand{\maxthreesat}{\problemmacro{max \pnum{3}-sat}}
\newcommand{\maxthreelin}{\problemmacro{max \pnum{3}-lin}}
\newcommand{\threesat}{\problemmacro{\pnum{3}-sat}}
\newcommand{\labelcover}{\problemmacro{label cover}}
\newcommand{\setcover}{\problemmacro{set cover}}
\newcommand{\maxksat}{\problemmacro{max $k$-sat}}
\newcommand{\mas}{\problemmacro{maximum acyclic subgraph}}
\newcommand{\kwaycut}{\problemmacro{$k$-way cut}}
\newcommand{\sparsestcut}{\problemmacro{sparsest cut}}
\newcommand{\betweenness}{\problemmacro{betweenness}}
\newcommand{\uniformsparsestcut}{\problemmacro{uniform sparsest cut}}
\newcommand{\grothendieckproblem}{\problemmacro{Grothendieck problem}}
\newcommand{\maxfoursat}{\problemmacro{max \pnum{4}-sat}}
\newcommand{\maxkcsp}{\problemmacro{max $k$-csp}}
\newcommand{\maxdicut}{\problemmacro{max dicut}}
\newcommand{\maxcutgain}{\problemmacro{max cut gain}}
\newcommand{\smallsetexpansion}{\problemmacro{small-set expansion}}
\newcommand{\minbisection}{\problemmacro{min bisection}}
\newcommand{\minimumlineararrangement}{\problemmacro{minimum linear arrangement}}
\newcommand{\maxtwolin}{\problemmacro{max \pnum{2}-lin}}
\newcommand{\gammamaxlin}{\problemmacro{$\Gamma$-max \pnum{2}-lin}}
\newcommand{\basicsdp}{\problemmacro{basic sdp}}
\newcommand{\dgames}{\problemmacro{$d$-to-1 games}}
\newcommand{\maxclique}{\problemmacro{max clique}}
\newcommand{\densestksubgraph}{\problemmacro{densest $k$-subgraph}}


% {{{ alphabet }}}

\newcommand{\cA}{\mathcal A}
\newcommand{\cB}{\mathcal B}
\newcommand{\cC}{\mathcal C}
\newcommand{\cD}{\mathcal D}
\newcommand{\cE}{\mathcal E}
\newcommand{\cF}{\mathcal F}
\newcommand{\cG}{\mathcal G}
\newcommand{\cH}{\mathcal H}
\newcommand{\cI}{\mathcal I}
\newcommand{\cJ}{\mathcal J}
\newcommand{\cK}{\mathcal K}
\newcommand{\cL}{\mathcal L}
\newcommand{\cM}{\mathcal M}
\newcommand{\cN}{\mathcal N}
\newcommand{\cO}{\mathcal O}
\newcommand{\cP}{\mathcal P}
\newcommand{\cQ}{\mathcal Q}
\newcommand{\cR}{\mathcal R}
\newcommand{\cS}{\mathcal S}
\newcommand{\cT}{\mathcal T}
\newcommand{\cU}{\mathcal U}
\newcommand{\cV}{\mathcal V}
\newcommand{\cW}{\mathcal W}
\newcommand{\cX}{\mathcal X}
\newcommand{\cY}{\mathcal Y}
\newcommand{\cZ}{\mathcal Z}

\newcommand{\scrA}{\mathscr A}
\newcommand{\scrB}{\mathscr B}
\newcommand{\scrC}{\mathscr C}
\newcommand{\scrD}{\mathscr D}
\newcommand{\scrE}{\mathscr E}
\newcommand{\scrF}{\mathscr F}
\newcommand{\scrG}{\mathscr G}
\newcommand{\scrH}{\mathscr H}
\newcommand{\scrI}{\mathscr I}
\newcommand{\scrJ}{\mathscr J}
\newcommand{\scrK}{\mathscr K}
\newcommand{\scrL}{\mathscr L}
\newcommand{\scrM}{\mathscr M}
\newcommand{\scrN}{\mathscr N}
\newcommand{\scrO}{\mathscr O}
\newcommand{\scrP}{\mathscr P}
\newcommand{\scrQ}{\mathscr Q}
\newcommand{\scrR}{\mathscr R}
\newcommand{\scrS}{\mathscr S}
\newcommand{\scrT}{\mathscr T}
\newcommand{\scrU}{\mathscr U}
\newcommand{\scrV}{\mathscr V}
\newcommand{\scrW}{\mathscr W}
\newcommand{\scrX}{\mathscr X}
\newcommand{\scrY}{\mathscr Y}
\newcommand{\scrZ}{\mathscr Z}

\newcommand{\bbB}{\mathbb B}
\newcommand{\bbS}{\mathbb S}
\newcommand{\bbR}{\mathbb R}
\newcommand{\bbZ}{\mathbb Z}
\newcommand{\bbI}{\mathbb I}
\newcommand{\bbQ}{\mathbb Q}
\newcommand{\bbP}{\mathbb P}
\newcommand{\bbE}{\mathbb E}
\newcommand{\bbN}{\mathbb N}

\newcommand{\sfE}{\mathsf E}


% {{{ leqslant }}}
% slanted lower/greater equal signs
\renewcommand{\leq}{\leqslant}
\renewcommand{\le}{\leqslant}
\renewcommand{\geq}{\geqslant}
\renewcommand{\ge}{\geqslant}


% {{{ draftbox }}}
\ifnum\showdraftbox=1
\newcommand{\draftbox}{\begin{center}
  \fbox{%
    \begin{minipage}{2in}%
      \begin{center}%
%        \begin{Large}%
          \Large\textsc{Working Draft}\\%
%        \end{Large}\\
        Please do not distribute%
      \end{center}%
    \end{minipage}%
  }%
\end{center}
\vspace{0.2cm}}
\else
\newcommand{\draftbox}{}
\fi


% {{{ varepsilon }}}

\let\epsilon=\varepsilon

% {{{ numberequationwithinsection }}}
\numberwithin{equation}{section}


% {{{ restate }}}
% set of macros to deal with restating theorem environments (or anything
% else with a label)

% stolen from Boaz's latex macros

\newcommand\MYcurrentlabel{xxx}

% \MYstore{A}{B} assigns variable A value B
\newcommand{\MYstore}[2]{%
  \global\expandafter \def \csname MYMEMORY #1 \endcsname{#2}%
}

% \MYload{A} outputs value stored for variable A
\newcommand{\MYload}[1]{%
  \csname MYMEMORY #1 \endcsname%
}

% new label command, stores current label in \MYcurrentlabel
\newcommand{\MYnewlabel}[1]{%
  \renewcommand\MYcurrentlabel{#1}%
  \MYoldlabel{#1}%
}

% new label command that doesn't do anything
\newcommand{\MYdummylabel}[1]{}

\newcommand{\torestate}[1]{%
  % overwrite label command
  \let\MYoldlabel\label%
  \let\label\MYnewlabel%
  #1%
  \MYstore{\MYcurrentlabel}{#1}%
  % restore old label command
  \let\label\MYoldlabel%
}

\newcommand{\restatetheorem}[1]{%
  % overwrite label command with dummy
  \let\MYoldlabel\label
  \let\label\MYdummylabel
  \begin{theorem*}[Restatement of \prettyref{#1}]
    \MYload{#1}
  \end{theorem*}
  \let\label\MYoldlabel
}

\newcommand{\restatelemma}[1]{%
  % overwrite label command with dummy
  \let\MYoldlabel\label
  \let\label\MYdummylabel
  \begin{lemma*}[Restatement of \prettyref{#1}]
    \MYload{#1}
  \end{lemma*}
  \let\label\MYoldlabel
}

\newcommand{\restateprop}[1]{%
  % overwrite label command with dummy
  \let\MYoldlabel\label
  \let\label\MYdummylabel
  \begin{proposition*}[Restatement of \prettyref{#1}]
    \MYload{#1}
  \end{proposition*}
  \let\label\MYoldlabel
}

\newcommand{\restatefact}[1]{%
  % overwrite label command with dummy
  \let\MYoldlabel\label
  \let\label\MYdummylabel
  \begin{fact*}[Restatement of \prettyref{#1}]
    \MYload{#1}
  \end{fact*}
  \let\label\MYoldlabel
}

\newcommand{\restate}[1]{%
  % overwrite label command with dummy
  \let\MYoldlabel\label
  \let\label\MYdummylabel
  \MYload{#1}
  \let\label\MYoldlabel
}


% {{{ bibliography }}}

% add section for references to table of contents
\newcommand{\addreferencesection}{
  \phantomsection
  \addcontentsline{toc}{section}{References}
}


% {{{ mathabbreviations }}}

\newcommand{\la}{\leftarrow}
\newcommand{\sse}{\subseteq}
\newcommand{\ra}{\rightarrow}
\newcommand{\e}{\epsilon}
\newcommand{\eps}{\epsilon}
\newcommand{\eset}{\emptyset}


% {{{ paragraphperiod }}}


\let\origparagraph\paragraph
\renewcommand{\paragraph}[1]{\origparagraph{#1.}}


% {{{ allowdisplaybreaks }}}
% allows page breaks in large display math formulas

\allowdisplaybreaks


% {{{ sloppy }}}
% avoid math spilling on margin

\sloppy

% {{{ complexityclasses }}}

\newcommand{\cclassmacro}[1]{\texorpdfstring{\textbf{#1}}{#1}\xspace}
\newcommand{\p}{\cclassmacro{P}}
\newcommand{\np}{\cclassmacro{NP}}
\newcommand{\subexp}{\cclassmacro{SUBEXP}}

% {{{ paralist }}}

\usepackage{paralist}

% {{{ comment }}}

\usepackage{comment}


%{{{Bra Ket Notation}}}
\usepackage{braket}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../planted"
%%% End:

